Assured Mission Adaptation of UAVs

The design of systems that can change their behaviour to account for scenarios that were not foreseen at design time remains an open challenge. In this paper we propose an approach for adaptation of mobile robot missions that is not constrained to a predefined set of mission evolutions. We propose applying the MORPH adaptive software architecture to UAVs and show how controller synthesis can be used both to guarantee correct transitioning from the old to the new mission goals while architectural reconfiguration to include new software actuators and sensors if necessary. The architecture brings together architectural concepts that are commonplace in robotics such as temporal planning, discrete, hybrid and continuous control layers together with architectural concepts from adaptive systems such as runtime models and runtime synthesis. We validate the architecture flying several missions taken from the robotic literature for different real and simulated UAVs.

==> VCPref-main.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  This files contains initial values
%  of Vaucanson's parameter
%  Modify it to create your own style
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
% State aspect
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetStateLabelColor{black}      %% color
\SetStateLabelScale{1.7}        %% float
\SetStateLineStyle{solid}       %% aspect (other values: none, dashed, dotted)
\SetStateLineWidth{1.8pt}       %% length
\SetStateLineColor{black}       %% color
\SetStateFillStatus{solid}      %% aspect
\SetStateFillColor{white}       %% color
\FixDimState{solid}{gray}{1}{gray}{white}  %% LineStyle,LineColor,LineCoef (*\StateLineWidth),LabelColor,FillColor
\FixStateLineDouble{0.6}{0.4}               %% Double style: \StateLineDblCoef, \StateLineDblSep, coeffs applied to \StateLineWidth
%%%%%%%%%%%%%%
% Edge aspect
%%%%%%%%%%%%%%
\SetEdgeLabelColor{black}       %% color
\SetEdgeLabelScale{1.3}         %% float
\SetEdgeLineStyle{solid}        %% aspect
\SetEdgeLineWidth{1pt}          %% length
\SetEdgeLineColor{black}        %% color
\SetArcAngle{15}            %% int (degree)
\SetLArcAngle{30}           %% int (degree)
\SetArcCurvature{0.8}           %% float
\SetEdgeOffset{0pt}                     %% length
\SetArcOffset{1pt}          %% length
\SetLoopOffset{0pt}         %% length
\renewcommand{\ForthBackEdgeOffset}{5}  %% float : coef*\EdgeLineWidth -> offset
\FixDimEdge{solid}{1.2}{gray}{gray}     %% LineStyle,LineCoef,LineColor,LabelColor
\FixEdgeBorder{2}{white}        %% int,color : coef*\EdgeLineWidth -> width of border
\FixEdgeLineDouble{0.5}{0.6}        %% float : coefs*\EdgeLineWidth -> (width of lines, distance)
%%%%%%%%%%%%%%
% ZZ aspect
%%%%%%%%%%%%%%
\setlength{\ZZSize}{.9cm}       % length : apparent diameter
\renewcommand{\ZZShape}{0.5}        % coef: opening of the ZZ
\SetZZLineWidth{1.7}            % float
\renewcommand{\TransLabelZZCoef}{0.6}   % float : coef*\ZZSize -> distance added for labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scales  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\LargeScale}{0.85}        %float : argument of a \scalebox
\renewcommand{\MediumScale}{0.6}        %float
\renewcommand{\SmallScale}{0.5}     %float
\renewcommand{\TinyScale}{0.42}     %float
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% State parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\MediumStateDiameter}{.9cm}      %length
\setlength{\SmallStateDiameter}{.6cm}       %length
\setlength{\LargeStateDiameter}{1.2cm}      %length
\setlength{\VerySmallStateDiameter}{.3cm}   %length
\renewcommand{\VSStateLineCoef}{.6}         %float : coef *\StateLineWidth
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\ArrowOnMediumState}{1.5}     %float : coef *\StateDiameter for size of initial and final arrows
\renewcommand{\ArrowOnSmallState}{1.7}      %float
\renewcommand{\ArrowOnLargeState}{1.3}      %float
\renewcommand{\ArrowOnVerySmallState}{5}    %float
\renewcommand{\LoopOnMediumState}{7}        %float : curvature
\renewcommand{\LoopOnSmallState}{9.6}       %float
\renewcommand{\LoopOnLargeState}{5.8}       %float
\renewcommand{\LoopOnVariableState}{5.1}        %float
\renewcommand{\CLoopOnMediumState}{8}       %float
\renewcommand{\CLoopOnSmallState}{12}       %float
\renewcommand{\CLoopOnLargeState}{6}        %float
\renewcommand{\CLoopOnVariableState}{5.2}       %float
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\EdgeLabelPosit}{.45}   %per cent (use \Fix..LabelPosit with values in [10;90])
\renewcommand{\EdgeLabelRevPosit}{.55}
\renewcommand{\ArcLabelPosit}{.40}
\renewcommand{\ArcLabelRevPosit}{.60}
\renewcommand{\LArcLabelPosit}{.40}
\renewcommand{\LArcLabelRevPosit}{.60}
\renewcommand{\LoopLabelPosit}{.25}
\renewcommand{\LoopLabelRevPosit}{.75}
\renewcommand{\CLoopLabelPosit}{.25}
\renewcommand{\CLoopLabelRevPosit}{.75}
\renewcommand{\InitStateLabelPosit}{.10}
\renewcommand{\InitStateLabelRevPosit}{.90}
\renewcommand{\FinalStateLabelPosit}{.90}
\renewcommand{\FinalStateLabelRevPosit}{.10}
\SetEdgeArrowWidth{5pt}     %length of the edge arrow
\SetEdgeArrowLengthCoef{1.4}        %float : coef*\EdgeArrowSizeDim width of EA
\setlength{\EdgeDblArrowWidth}{5.5pt}       %length : size of EA for double transitions
\renewcommand{\EdgeDblArrowLengthCoef}{1.7} %int
\SetEdgeArrowInsetCoef{0.1}         %float : coef*\EdgeArrowSizeDim
\SetEdgeArrowStyle{->}              %style (other styles : <-, |-|, -|,...)
\renewcommand{\EdgeRevArrowStyle}{<-}           %style for reverse transitions
\renewcommand{\StateDimen}{outer}       %side of the boundary of states that corresponds to the diameter
\renewcommand{\StateDblDimen}{middle}       %idem for states with double line (values: outer, middle or inner)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initialization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetVCDirectory{}        %default dir=current dir
\HideFrame
\HideGrid
\MediumPicture
\HideName
\RigidLabel
\FullState              %% PlainState
\MediumState


==> VCpatch-pstricks-1-10.tex <==
\renewenvironment{VCPicture}[2][0]%
  {\settoheight{\VertShiftH}{$\{$}%
   \settodepth{\VertShiftD}{$\{$}%
   \setlength{\VertShift}{.5\VertShiftD-.5\VertShiftH}%
   \begin{pspicture}[shift=#1]#2%
   \ifVCFrame \FrameStyle \psframe#2\fi%
   \ifVCGrid \FrameStyle\GridStyle \psgrid#2\fi}%
  {\RstState\RstEdge%
   \end{pspicture}}


==> Vaucanson-G.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                           
%                  Vaucanson_v4.tex                      
%                                                           
%       Automata drawer based on Pstricks
%                       
%                V 0.2 - 03/05/09
%  modification of StateVar
%  Chg*LabelScale is relative w.r.t Set*LabelScale
%  Chg Vaucanson to Vaucanson-G
%                V 0.3 - 03/09/10
%  VCPref-main is no more required to initialize VC-G
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Commands for geometric constructions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% constants 
\newcommand{\SQRTwo}{0.717}
\newcommand{\SQRThree}{1.732}
\newcommand{\GoldMean}{0.618}
\newcommand{\GoldMeanI}{1.618}
\newcommand{\SQRGoldMeanI}{1.272}
\newcommand{\Vaucanson}{\textsc{V$\overline{\text{au}}$C%
\raisebox{.3ex}{$\underline{\text{an}}$}S$\overline{\text{on}}$-G}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Edge label drawing macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Separator in compound labels (eg \IOL{input}{output})
\newcommand{\IOL}[2]{#1\!\mid\! #2}
%%% Stacked labels
\newcommand{\StackTwoLabels}[2]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{c}#1\\ #2 \end{array}%
   \renewcommand{\arraystretch}{1.333}}
\newcommand{\StackThreeLabels}[3]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{c}#1\\ #2 \\ #3 \end{array}%
   \renewcommand{\arraystretch}{1.333}}
%%% Stacked labels with +
\newcommand{\StackTwoLabelsP}[2]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{c}#1\\ + \\ #2 \end{array}%
   \renewcommand{\arraystretch}{1.333}}
\newcommand{\StackThreeLabelsP}[3]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{c}#1\\ + \\ #2 \\ + \\ #3 \end{array}% 
   \renewcommand{\arraystretch}{1.333}}
%%% Lined up labels (with +)
\newcommand{\LineTwoLabelsP}[2]{#1 + #2} 
\newcommand{\LineThreeLabelsP}[3]{#1 + #2 + #3}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scales  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\LargeScale}{0.85}
\newcommand{\MediumScale}{0.6}
\newcommand{\SmallScale}{0.5}
\newcommand{\TinyScale}{0.42}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% State parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Size = StateDiameter
%%% The preset sizes are given in cm, and not in "psunits".
%%% This allows to use different scales for the whole figure 
%%% and for the "drawing grid".
\newlength{\MediumStateDiameter}
\newlength{\SmallStateDiameter}
\newlength{\LargeStateDiameter}
\newlength{\VerySmallStateDiameter}
\setlength{\MediumStateDiameter}{.9cm}
\setlength{\SmallStateDiameter}{.6cm}
\setlength{\LargeStateDiameter}{1.2cm}
\setlength{\VerySmallStateDiameter}{.3cm}
%%% Border line = StateLine
\newlength{\StateLineWidth}        % width
\setlength{\StateLineWidth}{1.8pt}
\newcommand{\StateLineStyle}{solid} % style
\newcommand{\StateLineColor}{black}
\newif\ifStateLineDbl \StateLineDblfalse 
\newcommand{\StateLineDblCoef}{0.6} 
\newcommand{\StateLineDblSep}{0.4} 
\newcommand{\VSStateLineCoef}{.6} % coef. for very small state
%%% State background and label
\newcommand{\StateFillStatus}{solid} 
\newcommand{\StateFillColor}{white}
\newcommand{\StateLabelColor}{black}
\newcommand{\StateLabelScale}{1.7}
\newcommand{\SmallStateFillStatus}{solid} %
\newcommand{\SmallStateFillColor}{white} %
   % As they have usually no labels it useful
   % to have a coloring facility for the "SmallState"
%%%  Dimmed states (e.g. for non accessible states)
\newcommand{\DimStateLineStyle}{solid} 
\newcommand{\DimStateLineCoef}{1} % 
\newcommand{\DimStateLineColor}{gray}
\newcommand{\DimStateLabelColor}{gray}
\newcommand{\DimStateFillColor}{white}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge drawing parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% line
\newlength{\EdgeLineWidth}
\setlength{\EdgeLineWidth}{1pt}
\newcommand{\EdgeLineStyle}{solid}
\newif\ifEdgeLineDbl \EdgeLineDblfalse 
%\newcommand{\EdgeLineDblStatus}{false} 
\newcommand{\EdgeLineDblCoef}{0.5} 
\newcommand{\EdgeLineDblSep}{0.6} 
\newcommand{\EdgeLineColor}{black}
% arrow
\newlength{\EdgeArrowWidth}\setlength{\EdgeArrowWidth}{5pt}
\newlength{\EdgeDblArrowWidth}\setlength{\EdgeDblArrowWidth}{5.5pt}
\newcommand{\EdgeArrowLengthCoef}{1.4}
\newcommand{\EdgeDblArrowLengthCoef}{1.7}
\newcommand{\EdgeArrowInset}{0.1}
\newcommand{\EdgeArrowStyle}{->}
\newcommand{\EdgeRevArrowStyle}{<-}
% border
\newcommand{\EdgeLineBorderCoef}{2}
\newcommand{\EdgeLineBorderColor}{white}
% label
\newcommand{\EdgeLabelColor}{black}
\newcommand{\EdgeLabelScale}{1.7}
%%% Dimmed edges 
\newcommand{\DimEdgeLineCoef}{1.2} 
\newcommand{\DimEdgeLineStyle}{solid} 
\newcommand{\DimEdgeLineColor}{gray}
\newcommand{\DimEdgeLabelColor}{gray}
%%% Zigzag edges parameter
\newlength{\ZZSize}
\setlength{\ZZSize}{.9cm}%\MediumStateDiameter
\newcommand{\ZZShape}{0.5}
\newcommand{\ZZLineWidth}{1.7}% coefficient multiplicateur
\newcommand{\TransLabelZZCoef}{0.6}% coefficient multiplicateur
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge geometric parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Edge 
\newlength{\EdgeOffset}
\setlength{\EdgeOffset}{0pt}
\newcommand{\ForthBackEdgeOffset}{5}% coef
% Arc parameters
\newcommand{\VaucArcAngle}{15}
\newcommand{\VaucArcCurvature}{0.8}
\newlength{\VaucArcOffset}
\setlength{\VaucArcOffset}{1pt}
% Large Arc parameters
\newcommand{\VaucLArcAngle}{30}
\newcommand{\VaucLArcCurvature}{0.8}
\newlength{\LoopOffset}\setlength{\LoopOffset}{0pt}
\newlength{\LoopVarOffset}\setlength{\LoopVarOffset}{.7pt}
\newcommand{\LoopAngle}{30}
\newcommand{\CLoopAngle}{22}
\newcommand{\LoopVarAngle}{28}
% Size of loops (depending on the size of the state)
\newcommand{\LoopOnMediumState}{7}
\newcommand{\LoopOnSmallState}{9.6} 
\newcommand{\LoopOnLargeState}{5.8} 
\newcommand{\LoopOnVariableState}{5.1} 
\newcommand{\LoopOnVerySmallState}{15} 
\newcommand{\CLoopOnMediumState}{8}
\newcommand{\CLoopOnSmallState}{12}
\newcommand{\CLoopOnLargeState}{6}
\newcommand{\CLoopOnVariableState}{5.2}
%\newcommand{\CLoopOnVerySmallState}{14} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Edge label parameters --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% label distance from transition
\newlength{\TransLabelSep}\setlength{\TransLabelSep}{3.5pt}
% label position on transitions
\newcommand{\EdgeLabelPosit}{.45}\newcommand{\EdgeLabelRevPosit}{.55}
\newcommand{\ArcLabelPosit}{.4}\newcommand{\ArcLabelRevPosit}{.6}
\newcommand{\LArcLabelPosit}{.4}\newcommand{\LArcLabelRevPosit}{.6}
\newcommand{\LoopLabelPosit}{.25}\newcommand{\LoopLabelRevPosit}{.75}
\newcommand{\CLoopLabelPosit}{.25}\newcommand{\CLoopLabelRevPosit}{.75}
% label position on initial-final arrow
\newcommand{\InitStateLabelPosit}{.1}\newcommand{\InitStateLabelRevPosit}{.9}
\newcommand{\FinalStateLabelPosit}{.9}\newcommand{\FinalStateLabelRevPosit}{.1}
%%% Size of initial and final arrow
% the size is relative to the diameter
% and the coefficient varies with the diameter
\newcommand{\ArrowOnStateCoef}{}
\newcommand{\ArrowOnMediumState}{1.5}
\newcommand{\ArrowOnSmallState}{1.7} 
\newcommand{\ArrowOnLargeState}{1.3}
\newcommand{\ArrowOnVerySmallState}{5} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Shift for aligned labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\VertShiftH} \settoheight{\VertShiftH}{$\{$}
\newlength{\VertShiftD} \settodepth{\VertShiftD}{$\{$}
\newlength{\VertShift}
\setlength{\VertShift}{.5\VertShiftD-.5\VertShiftH}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% flags 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\ifVCFrame
\newcommand{\HideFrame}{\VCFramefalse}
\newcommand{\ShowFrame}{\VCFrametrue}
\newif\ifVCGrid
\newcommand{\HideGrid}{\VCGridfalse}
\newcommand{\ShowGrid}{\VCGridtrue}
\newif\ifVCRigidLabel
\newcommand{\RigidLabel}{\VCRigidLabeltrue}
\newcommand{\SwivelLabel}{\VCRigidLabelfalse}
\newif\ifVCStateLabelBaseLine
\newcommand{\AlignedLabel}{\VCStateLabelBaseLinetrue}
\newcommand{\FloatingLabel}{\VCStateLabelBaseLinefalse}
\HideFrame
\HideGrid
\RigidLabel
\FloatingLabel
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   style for the frame around the picture
\psset{unit=1cm}
\newpsstyle{VaucFrameStyle}{arrows=-,framesep=0pt,%                   
                     linewidth=0.6pt,linecolor=black,%
                                         linestyle=solid,%
                                         doubleline=false,%
                                         fillcolor=white,fillstyle=none,%
                                         cornersize=relative,framearc=0}
\newcommand{\FrameStyle}{\psset{style=VaucFrameStyle}}
\newpsstyle{VaucGridStyle}{%
      gridwidth=0.6pt,griddots=10,subgriddiv=1,%
          gridlabels=7pt}
\newcommand{\GridStyle}{\psset{style=VaucGridStyle}}
% figure, vertically centered by default
% draw frame according to VCFrame flag
% Set the shift for aligned label w.r.t the current size of characters
\newenvironment{VCPicture}[2][.5]%
  {\settoheight{\VertShiftH}{$\{$}%
   \settodepth{\VertShiftD}{$\{$}%
   \setlength{\VertShift}{.5\VertShiftD-.5\VertShiftH}%
   \begin{pspicture}[#1]#2%
   \ifVCFrame \FrameStyle \psframe#2\fi%
   \ifVCGrid \FrameStyle\GridStyle \psgrid#2\fi}%
  {\RstState\RstEdge%
   \end{pspicture}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scaling matters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% The "sizes" (for states) and the "line widths" are given 
%%% as "lengthes" in a fixed unit (cm or pt), whereas the positions 
%%% are supposed to be given in "psunits".
%%% This allows to use different scaling parameters 
%%% for the whole figure and for the "drawing grid".
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scaling commands
\newcommand{\VCScale}{0.6}% Global scale parameter
\newcommand{\VCGridScale}{1}% Global scale parameter
% 
\newcommand{\FixVCScale}[1]{\renewcommand{\VCScale}{#1}}% v4 pour 
%                                              % cause de syntaxe
\newcommand{\LargePicture}{\FixVCScale{\LargeScale}}
\newcommand{\MediumPicture}{\FixVCScale{\MediumScale}}
\newcommand{\SmallPicture}{\FixVCScale{\SmallScale}}
\newcommand{\TinyPicture}{\FixVCScale{\TinyScale}}
%%% Grid scale commands
% \newcommand{\VCGridScale}{}% Grid scale parameter
% 
\newcommand{\FixVCGridScale}[1]{\renewcommand{\VCGridScale}{#1}}% v4 pour 
% "grid unit"
%%%%% Typical figure would look like
%   \scalebox{\VCScale}{%
%     \begin{VCPicture}{(x0,y0)(x1,y1)}
%     %  figure description
%     \end{VCPicture}%
%    }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Using a special directory for the figure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\VCDirectory}{}
\newcommand{\SetVCDirectory}[1]{\renewcommand{\VCDirectory}{#1}}
% flag for printing the name of the figure file
\newif\ifVCName
\newcommand{\HideName}{\VCNamefalse}
\newcommand{\ShowName}{\VCNametrue}
\newcommand{\VCDraw}[2][\VCGridScale]{%
\psset{unit=#1cm}%
\ifVCName\makebox[0pt][r]{\fbox{{\scriptsize #2}}}\fi%
\scalebox{\VCScale}{#2}%
\psset{unit=1cm}}
\newcommand{\VCCall}[2][\VCGridScale]{%
\psset{unit=#1cm}%
\ifVCName\makebox[0pt][r]{\fbox{{\scriptsize #2}}}\fi%
\scalebox{\VCScale}{\input{\VCDirectory #2}}%
\psset{unit=1cm}}
%%% commands
\newcommand{\VCPut}[3][0]{\rput{#1}#2{#3}}% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% State internal parameters  --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\StateLineWid}
\setlength{\StateLineWid}{\StateLineWidth}
\newcommand{\StateLineSty}{\StateLineStyle} 
\newcommand{\StateLineCol}{\StateLineColor}
%\newcommand{\StateLineDblSta}{\StateLineDblStatus}
\newcommand{\StateLineDblWid}{\StateLineDblWidth}
\newcommand{\StateLineDblSp}{\StateLineDblSep}
\newcommand{\StateFillCol}{\StateFillColor}
\newcommand{\StateFillSta}{\StateFillStatus} 
\newcommand{\StateLabelSca}{1}
\newcommand{\StateLabelCol}{\StateLabelColor}
\newcommand{\StateDimen}{outer}
\newcommand{\StateDblDimen}{middle}
%%%  Initial-final quality
\newcommand{\VCIFflag}{2}\newcommand{\VCIFflagtemp}{2}
\newcommand{\PlainState}%
  {\renewcommand{\VCIFflag}{0}\renewcommand{\VCIFflagtemp}{0}}
\newcommand{\FullState}%
  {\renewcommand{\VCIFflag}{2}\renewcommand{\VCIFflagtemp}{2}}
\newcommand{\IFState}{\renewcommand{\VCIFflag}{1}}
\newcommand{\IFXState}{\renewcommand{\VCIFflag}{2}}
\newcommand{\RstVCIF}{\renewcommand{\VCIFflag}{\VCIFflagtemp}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  State drawing style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% flag for hiding -- showing states (used for overlays in slides)
% the trick is to have two different styles and instead of 
% saving\restoring parameters
\newif\ifVCShowState
\newcommand{\HideState}{\VCShowStatefalse}
\newcommand{\ShowState}{\VCShowStatetrue}
\ShowState % initialisation
% the only difference between the two styles is the linestyle
\newpsstyle{VaucStateStyle}{framesep=0pt,%                   
         linewidth=\StateLineWid,linecolor=\StateLineCol,%
         linestyle=\StateLineSty,doubleline=false,%
         fillcolor=\StateFillCol,fillstyle=\StateFillSta,% 
         border=0pt,dimen=\StateDimen,%
         cornersize=relative,framearc=1,framesep=0pt}
\newpsstyle{VaucStateDblStyle}{framesep=0pt,%                   
         linewidth=\StateLineDblCoef\StateLineWid,linecolor=\StateLineCol,%
         linestyle=\StateLineSty,doubleline=true,doublesep=\StateLineDblSep\StateLineWid,%
         fillcolor=\StateFillCol,fillstyle=\StateFillSta,% 
         border=0pt,dimen=\StateDblDimen,%
         cornersize=relative,framearc=1,framesep=0pt}
\newpsstyle{VaucHiddenStateStyle}{framesep=0pt,%                   
         linewidth=\StateLineWid,linecolor=\StateLineCol,%
         linestyle=none,%
         fillcolor=\StateFillCol,fillstyle=none,% 
         border=0pt,dimen=outer,%
         cornersize=relative,framearc=1,framesep=0pt}
\newcommand{\StateStyle}{%
   \ifVCShowState%
         \ifStateLineDbl\psset{style=VaucStateDblStyle}\else\psset{style=VaucStateStyle}\fi%
   \else\psset{style=VaucHiddenStateStyle}\fi}
\newcommand{\VaucStateRBLabel}[1]{%
    \textcolor{\StateLabelCol}{\scalebox{\StateLabelSca}{\scalebox{\StateLabelScale}{\rput[B]{0}(0,\VertShift){$ #1 $}}}}}%
\newcommand{\VaucStateLabel}[1]%
    {\ifVCShowState%
        \ifVCRigidLabel%
           \ifVCStateLabelBaseLine%
                 \textcolor{\StateLabelCol}{\scalebox{\StateLabelSca}{\scalebox{\StateLabelScale}{\rput[B]{*0}(0,\VertShift){$ #1 $}}}}%
           \else
                 \textcolor{\StateLabelCol}{\scalebox{\StateLabelSca}{\scalebox{\StateLabelScale}{\rput{*0}(0,0){$ #1 $}}}}%
           \fi
        \else
                 \textcolor{\StateLabelCol}{\scalebox{\StateLabelSca}{\scalebox{\StateLabelScale}{$ #1 $}}}%
        \fi
     \else%
                 \textcolor{white}{\scalebox{\StateLabelSca}{\scalebox{\StateLabelScale}{$ #1 $}}}%
     \fi}
\newcommand{\VCPutStateLabel}[2]%
    {\rput#1{\scalebox{\StateLabelSca}{$ #2 $}}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  State parameter changing and setting macros 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% line style
\newcommand{\ChgStateLineStyle}[1]{\renewcommand{\StateLineSty}{#1}}
\newcommand{\RstStateLineStyle}{\ChgStateLineStyle{\StateLineStyle}}
\newcommand{\SetStateLineStyle}[1]%
   {\renewcommand{\StateLineStyle}{#1}\RstStateLineStyle}%
%%% doubleline status
\newcommand{\StateLineDouble}{\StateLineDbltrue}
\newcommand{\StateLineSimple}{\StateLineDblfalse}
%%% line width
\newcommand{\ChgStateLineWidth}[1]{\setlength{\StateLineWid}{#1\StateLineWidth}}%  
\newcommand{\RstStateLineWidth}{\ChgStateLineWidth{1}}%
\newcommand{\SetStateLineWidth}[1]% ATTN the parameter is a length
   {\setlength{\StateLineWidth}{#1}\RstStateLineWidth}
%%% line color
\newcommand{\ChgStateLineColor}[1]{\renewcommand{\StateLineCol}{#1}}
\newcommand{\RstStateLineColor}{\ChgStateLineColor{\StateLineColor}}
\newcommand{\SetStateLineColor}[1]%
   {\renewcommand{\StateLineColor}{#1}\RstStateLineColor}
%%% background fill status
\newcommand{\ChgStateFillStatus}[1]{\renewcommand{\StateFillSta}{#1}}
\newcommand{\RstStateFillStatus}{\ChgStateFillStatus{\StateFillStatus}}
\newcommand{\SetStateFillStatus}[1]% 
    {\renewcommand{\StateFillStatus}{#1}\RstStateFillStatus}
%%% backgroud color
\newcommand{\ChgStateFillColor}[1]{\renewcommand{\StateFillCol}{#1}}
\newcommand{\RstStateFillColor}{\ChgStateFillColor{\StateFillColor}}
\newcommand{\SetStateFillColor}[1]% 
    {\renewcommand{\StateFillColor}{#1}\RstStateFillColor}%
%%% label color
\newcommand{\ChgStateLabelColor}[1]{\renewcommand{\StateLabelCol}{#1}}
\newcommand{\RstStateLabelColor}{\ChgStateLabelColor{\StateLabelColor}}
\newcommand{\SetStateLabelColor}[1]%
    {\renewcommand{\StateLabelCol}{#1}\RstStateLabelColor}
%%% label scale
\newcommand{\ChgStateLabelScale}[1]{\renewcommand{\StateLabelSca}{#1}}
\newcommand{\RstStateLabelScale}{\ChgStateLabelScale{1}}
\newcommand{\SetStateLabelScale}[1]%
   {\renewcommand{\StateLabelScale}{#1}\RstStateLabelScale}
\newcommand{\FixStateLineDouble}[2]{%
    \renewcommand{\StateLineDblCoef}{#1}%
    \renewcommand{\StateLineDblSep}{#2}}
\newcommand{\FixDimState}[5]{%
    \renewcommand{\DimStateLineStyle}{#1}%
    \renewcommand{\DimStateLineCoef}{#3}%
    \renewcommand{\DimStateLineColor}{#2}%
    \renewcommand{\DimStateLabelColor}{#4}%
    \renewcommand{\DimStateFillColor}{#5}}%
%%% restoring state parameters
\newcommand{\RstState}{%
   \RstStateLineStyle\RstStateLineWidth%
   \RstStateLineColor%
   \RstStateFillStatus\RstStateFillColor%
   \RstStateLabelColor\RstStateLabelScale}%
%%% establishing the dimmed style
\newcommand{\DimState}{%
    \ChgStateLineStyle{\DimStateLineStyle}%
    \ChgStateLineWidth{\DimStateLineCoef}%
    \ChgStateLineColor{\DimStateLineColor}%
        \ChgStateFillColor{\DimStateFillColor}%
    \ChgStateLabelColor{\DimStateLabelColor}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% State drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% preparation
\newlength{\StateDiam}
\newlength{\VaucAOS}\newlength{\VaucAOSdiag}
%%%  A flag to remember the current size of state
\newcommand{\StateSizeFlag}{}
%
\newcommand{\SetAOS}{%
   \setlength{\VaucAOS}{\ArrowOnStateCoef\StateDiam}%
   \setlength{\VaucAOSdiag}{\SQRTwo\VaucAOS}}
%% parameter for variable width states
\newlength{\VariableStateIntDiam}
\newlength{\VariableStateWidth}
\newlength{\VariableStateITPos}
\newcommand{\SetStateIntDiam}{%
   \setlength{\VariableStateIntDiam}{\StateDiam}%
   \addtolength{\VariableStateIntDiam}{-2\StateLineWid}%
}%
% Loop parameters
\newcommand{\LoopSize}{}\newcommand{\LoopSi}{}
\newcommand{\LoopVarSize}{}\newcommand{\LoopVarSi}{}
\newcommand{\CLoopSize}{}\newcommand{\CLoopSi}{}
%
\newcommand{\ChgLoopSize}[1]{\renewcommand{\LoopSi}{#1}}
\newcommand{\RstLoopSize}{\ChgLoopSize{\LoopSize}}
\newcommand{\SetLoopSize}[1]%
   {\renewcommand{\LoopSize}{#1}\RstLoopSize}
%
\newcommand{\ChgCLoopSize}[1]{\renewcommand{\CLoopSi}{#1}}
\newcommand{\RstCLoopSize}{\ChgCLoopSize{\CLoopSize}}
\newcommand{\SetCLoopSize}[1]%
   {\renewcommand{\CLoopSize}{#1}\RstCLoopSize}
%
\newcommand{\ChgLoopVarSize}[1]{\renewcommand{\LoopVarSi}{#1}}
\newcommand{\RstLoopVarSize}{\ChgLoopVarSize{\LoopVarSize}}
\newcommand{\SetLoopVarSize}[1]%
   {\renewcommand{\LoopVarSize}{#1}\RstLoopVarSize}
%
%%% setting state diameter -- internal command
\newcommand{\SetStateDiam}[4]{%
   \setlength{\StateDiam}{#1}%
   \renewcommand{\ArrowOnStateCoef}{#2}%
   \SetLoopSize{#3}%
   \SetLoopVarSize{#3}%
   \SetCLoopSize{#4}%
   \SetAOS\SetStateIntDiam}
%%% setting state diameter -- external command
\newcommand{\FixStateDiameter}[1]%  v4 pour cause de syntaxe
   {\setlength{\StateDiam}{#1}\SetStateIntDiam \SetAOS}
%%%
\newcommand{\MediumState}%
   {\SetStateDiam{\MediumStateDiameter}{\ArrowOnMediumState}%
         {\LoopOnMediumState}{\CLoopOnMediumState}%
                  \renewcommand{\StateSizeFlag}{0}}
\newcommand{\SmallState}%
   {\SetStateDiam{\SmallStateDiameter}{\ArrowOnSmallState}%
         {\LoopOnSmallState}{\CLoopOnSmallState}%
                  \renewcommand{\StateSizeFlag}{1}}
\newcommand{\LargeState}%
   {\SetStateDiam{\LargeStateDiameter}{\ArrowOnLargeState}%
         {\LoopOnLargeState}{\CLoopOnLargeState}%
                  \renewcommand{\StateSizeFlag}{2}}
%
\newcommand{\RstStateSize}%
  {\ifthenelse{\equal{\StateSizeFlag}{0}}%
              {\MediumState}%
              {\ifthenelse{\equal{\StateSizeFlag}{1}}%
                              {\SmallState}{\LargeState}}}%
%%% Initialization
\MediumState
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\VaucState}[3][{}]%
   {\rput#2{%
      \Cnode[radius=.5\StateDiam](0,0){#3}%
          \ifVCShowState%
      \nput[labelsep=-.5\StateDiam]{0}{#3}%
        {\makebox[0pt]{\VaucStateLabel{#1}}}%
      \fi
      \ifthenelse{\equal{\VCIFflag}{0}}{}{%
        \pnode(-\VaucAOS,0){#3w}\pnode(\VaucAOS,0){#3e}%
        \pnode(0,\VaucAOS){#3n}\pnode(0,-\VaucAOS){#3s}%
           \ifthenelse{\equal{\VCIFflag}{1}}{}{%
          \pnode(-\VaucAOSdiag,\VaucAOSdiag){#3nw}%
           \pnode(\VaucAOSdiag,\VaucAOSdiag){#3ne}%
           \pnode(-\VaucAOSdiag,-\VaucAOSdiag){#3sw}%
           \pnode(\VaucAOSdiag,-\VaucAOSdiag){#3se}%
                   }%
            }%
     }%
}
%
\newcommand{\State}[3][{}]{\StateStyle\VaucState[#1]{#2}{#3}}
%
\newcommand{\FinalState}[3][{}]%
   {\psset{style=VaucStateDblStyle}\VaucState[#1]{#2}{#3}}
%%% ecological commands   
\newcommand{\StateIF}[3][{}]{\IFState\State[#1]{#2}{#3}\RstVCIF}%
\newcommand{\StateIFX}[3][{}]{\IFXState\State[#1]{#2}{#3}\RstVCIF}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Very Small State   
\newcommand{\VSState}[2]%
    {\renewcommand{\ArrowOnStateCoef}{\ArrowOnVerySmallState}%
         \FixStateDiameter{\VerySmallStateDiameter}%
     \ChgStateLineWidth{\VSStateLineCoef}%
         \State{#1}{#2}%
         \RstStateLineWidth\RstStateSize}% mod 020201
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% white brace, of no width, used to place the label vertically
%\newlength{\BraceLength}
\newcommand{\WB}{%
   \textcolor{white}{\{\!\!\!}}%
\newcommand{\HS}{}
\newlength{\ExtraSpace}
\setlength{\ExtraSpace}{1em}
%
\newcommand{\StateVar}[3][]%
 {\StateStyle %
  \settowidth{\VariableStateWidth}{\scalebox{\StateLabelSca}{\scalebox{\StateLabelScale}{$#1$}}}%
  \addtolength{\VariableStateWidth}{\ExtraSpace}
  \ifthenelse{\lengthtest{\VariableStateWidth < \VariableStateIntDiam}}%
        {\setlength{\VariableStateWidth}{\VariableStateIntDiam}}{}%
  \setlength{\VariableStateITPos}{\ArrowOnStateCoef\StateDiam}%
  \addtolength{\VariableStateITPos}{0.5\VariableStateWidth}%
  \addtolength{\VariableStateITPos}{-0.5\StateDiam}%
  \rput#2{\pnode(\VariableStateITPos,0){#3e}%
          \pnode(-\VariableStateITPos,0){#3w}%
          \pnode(0,\ArrowOnStateCoef\StateDiam){#3n}%
          \pnode(0,-\ArrowOnStateCoef\StateDiam){#3s}}%
  \rput#2{\rnode{#3}{\psframebox{\protect\rule[-.5\VariableStateIntDiam]{0pt}{\VariableStateIntDiam}\protect\rule{\VariableStateWidth}{0pt}}}}
  \rput#2{\VaucStateRBLabel{#1}}%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\VarLoopOn}{\ChgLoopOffset{\LoopVarOff}%
   \ChgLoopSize{\LoopVarSi}%
   \ChgLoopAngle{\LoopVarAng}}
\newcommand{\VarLoopOff}{\RstLoopOffset \RstLoopSize \RstLoopAngle}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge drawing parameters  --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\EdgeLineWid}
\setlength{\EdgeLineWid}{\EdgeLineWidth}
\newcommand{\EdgeLineSty}{\EdgeLineStyle}
\newcommand{\EdgeLineCol}{\EdgeLineColor}
% label
\newcommand{\EdgeLabelSca}{1}
\newcommand{\EdgeLabelCol}{\EdgeLabelColor}
% arrow
\newlength{\EdgeArrowSZDim}
\setlength{\EdgeArrowSZDim}{\EdgeArrowWidth}
\newcommand{\EdgeArrowSZNum}{\EdgeArrowLengthCoef}
\newcommand{\EdgeArrowSty}{\EdgeArrowStyle}
\newcommand{\EdgeArrowIns}{\EdgeArrowInset}
% border 
\newlength{\EdgeLineBord}\setlength{\EdgeLineBord}{0pt}
%%% Zigzag edge parameter
\newlength{\ZZSiZ}
\setlength{\ZZSiZ}{\ZZSize}%
\newcommand{\ZZLineWid}{\ZZLineWidth}% coefficient multiplicateur
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge geometric parameters  --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Edge 
\newlength{\EdgeOff}
\setlength{\EdgeOff}{\EdgeOffset}
% Arc
\newcommand{\VaucArcAng}{\VaucArcAngle}
\newcommand{\VaucLArcAng}{\VaucLArcAngle}
\newlength{\VaucArcOff}\setlength{\VaucArcOff}{\VaucArcOffset}
% Loop
\newcommand{\VaucArcCurv}{\VaucArcCurvature}
\newcommand{\VaucLArcCurv}{\VaucLArcCurvature}
\newcommand{\LoopAng}{\LoopAngle}
\newcommand{\CLoopAng}{\CLoopAngle}
\newcommand{\LoopVarAng}{\LoopVarAngle}
\newlength{\LoopOff}\setlength{\LoopOff}{\LoopOffset}
\newlength{\LoopVarOff}\setlength{\LoopVarOff}{\LoopVarOffset}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Edge label parameters --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% label distance from transition
\newlength{\TransLabelSP}\setlength{\TransLabelSP}{\TransLabelSep}
% label position on transitions
\newcommand{\EdgeLabelPos}{\EdgeLabelPosit}
\newcommand{\ArcLabelPos}{\ArcLabelPosit}
\newcommand{\LArcLabelPos}{\LArcLabelPosit}
\newcommand{\LoopLabelPos}{\LoopLabelPosit}
\newcommand{\CLoopLabelPos}{\CLoopLabelPosit}
% label position on initial-final arrow
\newcommand{\InitStateLabelPos}{\InitStateLabelPosit}
\newcommand{\FinalStateLabelPos}{\FinalStateLabelPosit}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Transition styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpsstyle{VaucEdgeStyle}%
    {arrows=\EdgeArrowSty,arrowsize=\EdgeArrowSZDim,arrowlength=\EdgeArrowSZNum,%
         arrowinset=\EdgeArrowIns,%
     linewidth=\EdgeLineWid,linecolor=\EdgeLineCol,linestyle=\EdgeLineSty,%
     doubleline=false,%
         bordercolor=\EdgeLineBorderColor,border=\EdgeLineBord,%
     fillstyle=none,offset=\EdgeOff,%
     labelsep=\TransLabelSP,nodesep=0pt}
\newpsstyle{VaucEdgeDblStyle}%
    {arrows=\EdgeArrowSty,arrowsize=\EdgeArrowSZDim,arrowlength=\EdgeArrowSZNum,%
         arrowinset=\EdgeArrowIns,%
     linewidth=\EdgeLineDblCoef\EdgeLineWid,linecolor=\EdgeLineCol,linestyle=\EdgeLineSty,%
     doubleline=true,doublesep=\EdgeLineDblSep\EdgeLineWid,%
         bordercolor=\EdgeLineBorderColor,border=\EdgeLineBord,%
     fillstyle=none,offset=\EdgeOff,%
     labelsep=\TransLabelSP,nodesep=0pt}
%%% Arc
\newpsstyle{VaucArcR}{ncurv=\VaucArcCurv,arcangle=-\VaucArcAng,%
     labelsep=\TransLabelSP,offset=-\VaucArcOff}
\newpsstyle{VaucArcL}{ncurv=\VaucArcCurv,arcangle=\VaucArcAng,%
     labelsep=\TransLabelSP,offset=\VaucArcOff}
\newpsstyle{VaucLArcR}{ncurv=\VaucLArcCurv,arcangle=-\VaucLArcAng,%
     labelsep=\TransLabelSP,offset=-\VaucArcOff}
\newpsstyle{VaucLArcL}{ncurv=\VaucLArcCurv,arcangle=\VaucLArcAng,%
     labelsep=\TransLabelSP,offset=\VaucArcOff}
%%% zig-zag
\newpsstyle{VaucZigzagStyle}%
   {linewidth=\ZZLineWid\EdgeLineWid,%
    labelsep=\TransLabelSP,nodesep=0pt,%
    coilwidth=1.2\ZZSiZ,coilarmA=0.1\ZZSiZ,%
    coilarmB=0.3\ZZSiZ,coilheight=\ZZShape,linearc=1.6pt}
%%%
\newcommand{\EdgeStyle}{\ifEdgeLineDbl\psset{style=VaucEdgeDblStyle}%
        \else\psset{style=VaucEdgeStyle}\fi}
\newcommand{\ZigzagStyle}%
   {\addtolength{\TransLabelSP}{\TransLabelZZCoef\ZZSiZ}%
    \psset{style=VaucZigzagStyle}%
        \addtolength{\TransLabelSP}{-\TransLabelZZCoef\ZZSiZ}%
        }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Transition parameter changing and setting macros 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% geometric parameters
\newcommand{\ChgEdgeOffset}[1]{\setlength{\EdgeOff}{#1}}
\newcommand{\RstEdgeOffset}{\ChgEdgeOffset{\EdgeOffset}}
\newcommand{\SetEdgeOffset}[1]%
   {\setlength{\EdgeOffset}{#1}\RstEdgeOffset}
\newcommand{\ForthBackOffset}{%
   \setlength{\EdgeOff}{\ForthBackEdgeOffset\EdgeLineWid}}
%
\newcommand{\ChgArcAngle}[1]{\renewcommand{\VaucArcAng}{#1}}
\newcommand{\RstArcAngle}{\ChgArcAngle{\VaucArcAngle}}
\newcommand{\SetArcAngle}[1]%
   {\renewcommand{\VaucArcAngle}{#1}\RstArcAngle}
%
\newcommand{\ChgLArcAngle}[1]{\renewcommand{\VaucLArcAng}{#1}}
\newcommand{\RstLArcAngle}{\ChgLArcAngle{\VaucLArcAngle}}
\newcommand{\SetLArcAngle}[1]%
   {\renewcommand{\VaucLArcAngle}{#1}\RstLArcAngle}
%
\newcommand{\ChgArcCurvature}[1]{\renewcommand{\VaucArcCurv}{#1}}
\newcommand{\RstArcCurvature}{\ChgArcCurvature{\VaucArcCurvature}}
\newcommand{\SetArcCurvature}[1]%
   {\renewcommand{\VaucArcCurvature}{#1}\RstArcCurvature}
%
\newcommand{\ChgLArcCurvature}[1]{\renewcommand{\VaucLArcCurv}{#1}}
\newcommand{\RstLArcCurvature}{\ChgLArcCurvature{\VaucLArcCurvature}}
\newcommand{\SetLArcCurvature}[1]%
   {\renewcommand{\VaucLArcCurvature}{#1}\RstLArcCurvature}
%
\newcommand{\ChgArcOffset}[1]{\setlength{\VaucArcOff}{#1}}
\newcommand{\RstArcOffset}{\setlength{\VaucArcOff}{\VaucArcOffset}}
\newcommand{\SetArcOffset}[1]%
   {\renewcommand{\VaucArcOffset}{#1}\RstArcOffset}
%
\newcommand{\ChgLoopOffset}[1]{\setlength{\LoopOff}{#1}}
\newcommand{\RstLoopOffset}{\setlength{\LoopOff}{\LoopOffset}}
\newcommand{\SetLoopOffset}[1]%
   {\renewcommand{\LoopOffset}{#1}\RstLoopOffset}
%
\newcommand{\ChgLoopAngle}[1]{\renewcommand{\LoopAng}{#1}}
\newcommand{\RstLoopAngle}{\ChgLoopAngle{\LoopAngle}}
\newcommand{\SetLoopAngle}[1]%
   {\renewcommand{\LoopAngle}{#1}\RstLoopAngle}
%
\newcommand{\ChgCLoopAngle}[1]{\renewcommand{\CLoopAng}{#1}}
\newcommand{\RstCLoopAngle}{\ChgCLoopAngle{\CLoopAngle}}
\newcommand{\SetCLoopAngle}[1]%
   {\renewcommand{\CLoopAngle}{#1}\RstCLoopAngle}
%
%%% drawing parameters
\newcommand{\ChgEdgeLineColor}[1]{\renewcommand{\EdgeLineCol}{#1}}
\newcommand{\RstEdgeLineColor}{\ChgEdgeLineColor{\EdgeLineColor}}
\newcommand{\SetEdgeLineColor}[1]%
   {\renewcommand{\EdgeLineColor}{#1}\RstEdgeLineColor}
%
\newcommand{\ChgEdgeLineStyle}[1]{\renewcommand{\EdgeLineSty}{#1}}  
\newcommand{\RstEdgeLineStyle}{\ChgEdgeLineStyle{\EdgeLineStyle}}
\newcommand{\SetEdgeLineStyle}[1]%
   {\renewcommand{\EdgeLineStyle}{#1}\RstEdgeLineStyle}
%
\newcommand{\ChgEdgeLineWidth}[1]% coefficient !
   {\setlength{\EdgeLineWid}{#1\EdgeLineWidth}}
\newcommand{\RstEdgeLineWidth}{\ChgEdgeLineWidth{1}}
\newcommand{\SetEdgeLineWidth}[1]% length !
   {\setlength{\EdgeLineWidth}{#1}\RstEdgeLineWidth}
%
\newcommand{\EdgeLineDouble}%
        {\EdgeLineDbltrue%
    \ChgEdgeArrowWidth{\EdgeDblArrowWidth}
    \ChgEdgeArrowLengthCoef{\EdgeDblArrowLengthCoef}}
\newcommand{\EdgeLineSimple}%
   {\EdgeLineDblfalse \RstEdgeArrowWidth \RstEdgeArrowLengthCoef}
%
\newcommand{\ChgEdgeLabelColor}[1]{\renewcommand{\EdgeLabelCol}{#1}}
\newcommand{\RstEdgeLabelColor}{\ChgEdgeLabelColor{\EdgeLabelColor}}
\newcommand{\SetEdgeLabelColor}[1]%
   {\renewcommand{\EdgeLabelColor}{#1}\RstEdgeLabelColor}
%
\newcommand{\ChgEdgeLabelScale}[1]{\renewcommand{\EdgeLabelSca}{#1}}
\newcommand{\RstEdgeLabelScale}{\ChgEdgeLabelScale{1}}
\newcommand{\SetEdgeLabelScale}[1]%
   {\renewcommand{\EdgeLabelScale}{#1}\RstEdgeLabelScale}
\newcommand{\FixDimEdge}[4]{%
    \renewcommand{\DimEdgeLineStyle}{#1}%
    \renewcommand{\DimEdgeLineCoef}{#2}%
    \renewcommand{\DimEdgeLineColor}{#3}%
    \renewcommand{\DimEdgeLabelColor}{#4}}%
%
\newcommand{\ChgEdgeArrowStyle}[1]{\renewcommand{\EdgeArrowSty}{#1}}
\newcommand{\RstEdgeArrowStyle}{\ChgEdgeArrowStyle{\EdgeArrowStyle}}
\newcommand{\SetEdgeArrowStyle}[1]%
   {\renewcommand{\EdgeArrowStyle}{#1}\RstEdgeArrowStyle}
%
\newcommand{\ChgEdgeArrowWidth}[1]%
   {\setlength{\EdgeArrowSZDim}{#1}} % !! length !!
\newcommand{\RstEdgeArrowWidth}{\ChgEdgeArrowWidth{\EdgeArrowWidth}}
\newcommand{\SetEdgeArrowWidth}[1]%
   {\setlength{\EdgeArrowWidth}{#1} \RstEdgeArrowWidth}
%
\newcommand{\ChgEdgeArrowLengthCoef}[1]{\renewcommand{\EdgeArrowSZNum}{#1}}
\newcommand{\RstEdgeArrowLengthCoef}{\ChgEdgeArrowLengthCoef{\EdgeArrowLengthCoef}}
\newcommand{\SetEdgeArrowLengthCoef}[1]%
   {\renewcommand{\EdgeArrowLengthCoef}{#1}\RstEdgeArrowLengthCoef}
%
\newcommand{\ChgEdgeArrowInsetCoef}[1]{\renewcommand{\EdgeArrowIns}{#1}}
\newcommand{\RstEdgeArrowInsetCoef}{\ChgEdgeArrowInsetCoef{\EdgeArrowInset}}
\newcommand{\SetEdgeArrowInsetCoef}[1]%
   {\renewcommand{\EdgeArrowInset}{#1}\RstEdgeArrowInsetCoef}
%
\newcommand{\ReverseArrow}%
   {\ChgEdgeArrowStyle{\EdgeRevArrowStyle}%
    \renewcommand{\EdgeLabelPos}{\EdgeLabelRevPosit}%
    \renewcommand{\ArcLabelPos}{\ArcLabelRevPosit}%
    \renewcommand{\LArcLabelPos}{\LArcLabelRevPosit}%
    \renewcommand{\LoopLabelPos}{\LoopLabelRevPosit}%
    \renewcommand{\CLoopLabelPos}{\CLoopLabelRevPosit}%
    \renewcommand{\InitStateLabelPos}{\InitStateLabelRevPosit}%
    \renewcommand{\FinalStateLabelPos}{\FinalStateLabelRevPosit}}
\newcommand{\StraightArrow}%
   {\ChgEdgeArrowStyle{\EdgeArrowStyle}%
    \renewcommand{\EdgeLabelPos}{\EdgeLabelPosit}%
    \renewcommand{\ArcLabelPos}{\ArcLabelPosit}%
    \renewcommand{\LArcLabelPos}{\LArcLabelPosit}%
    \renewcommand{\LoopLabelPos}{\LoopLabelPosit}%
    \renewcommand{\CLoopLabelPos}{\CLoopLabelPosit}%
    \renewcommand{\InitStateLabelPos}{\InitStateLabelPosit}%
    \renewcommand{\FinalStateLabelPos}{\FinalStateLabelPosit}}
% Double
\newcommand{\FixEdgeLineDouble}[2]{%
    \renewcommand{\EdgeLineDblCoef}{#1}%
    \renewcommand{\EdgeLineDblSep}{#2}}
% border
\newcommand{\FixEdgeBorder}[2]{%
    \renewcommand{\EdgeLineBorderCoef}{#1}%
    \renewcommand{\EdgeLineBorderColor}{#2}}
\newcommand{\EdgeBorder}%
  {\setlength{\EdgeLineBord}{\EdgeLineBorderCoef\EdgeLineWid}}
\newcommand{\EdgeBorderOff}{\setlength{\EdgeLineBord}{0pt}}
%%%
\newcommand{\DimEdge}{%
    \ChgEdgeLineStyle{\DimEdgeLineStyle}%
    \ChgEdgeLineWidth{\DimEdgeLineCoef}%
    \ChgEdgeLineColor{\DimEdgeLineColor}%
        \ChgEdgeLabelColor{\DimEdgeLabelColor}}
%%%
\newcommand{\ChgZZSize}[1]{\setlength{\ZZSiZ}{#1}}
\newcommand{\RstZZSize}{\setlength{\ZZSiZ}{\ZZSize}}
\newcommand{\SetZZSize}[1]{\setlength{\ZZSiZe}{#1}\RstZZSize}
%%%\ZZLineWidth
\newcommand{\ChgZZLineWidth}[1]{\renewcommand{\ZZLineWid}{#1}}
\newcommand{\RstZZLineWidth}{\ChgZZLineWidth{\ZZLineWidth}}
\newcommand{\SetZZLineWidth}[1]%
   {\renewcommand{\ZZLineWidth}{#1}\RstZZLineWidth}
%
%%% label of transitions
\newcommand{\VaucEdgeLabel}[1]{%
        \textcolor{\EdgeLabelCol}{\scalebox{\EdgeLabelSca}{\scalebox{\EdgeLabelScale}{$ #1 $}}}}
%%%
\newcommand{\RstEdge}{%
   \RstEdgeOffset\RstArcAngle\RstLArcAngle%
   \RstArcCurvature\RstLArcCurvature%
   \RstArcOffset\RstLoopOffset\RstLoopSize%
   \RstEdgeLineColor\RstEdgeLineStyle\RstEdgeLineWidth\EdgeLineSimple%
   \StraightArrow%\EdgeBorderOff%
   \RstEdgeLabelScale\RstEdgeLabelColor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Initial-final arrow drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% implicit parameter
\newcommand{\InitialDir}{w}\newcommand{\FinalDir}{e}
% without label
\newcommand{\Initial}[2][\InitialDir]{\EdgeStyle\ncline{#2#1}{#2}}
\newcommand{\Final}[2][\FinalDir]{\EdgeStyle\ncline{#2}{#2#1}}
% with label
%  NB modified syntax eg \InitialL[pos]{dir}{statename}{label}
\newcommand{\InitialL}[4][{\InitStateLabelPos}]%
   {\EdgeStyle\ncline{#3#2}{#3}\naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\InitialR}[4][{\InitStateLabelPos}]%
   {\EdgeStyle\ncline{#3#2}{#3}\nbput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\FinalL}[4][{\FinalStateLabelPos}]%
   {\EdgeStyle\ncline{#3}{#3#2}\naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\FinalR}[4][{\FinalStateLabelPos}]%
   {\EdgeStyle\ncline{#3}{#3#2}\nbput[npos=#1]{\VaucEdgeLabel{#4}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Transition drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EdgeL}[4][{\EdgeLabelPos}]%
   {\EdgeStyle \ncline{#2}{#3} \naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\EdgeR}[4][{\EdgeLabelPos}]%
   {\EdgeStyle \ncline{#2}{#3} \nbput[npos=#1]{\VaucEdgeLabel{#4}}}
%
\newcommand{\ArcL}[4][{\ArcLabelPos}]%
   {\EdgeStyle \psset{style=VaucArcL}% 
    \ncarc{#2}{#3} \naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\ArcR}[4][{\ArcLabelPos}]%
   {\EdgeStyle \psset{style=VaucArcR}% 
    \ncarc{#2}{#3} \nbput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\LArcL}[4][{\LArcLabelPos}]%
   {\EdgeStyle \psset{style=VaucLArcL}% 
    \ncarc{#2}{#3} \naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\LArcR}[4][{\LArcLabelPos}]%
   {\EdgeStyle \psset{style=VaucLArcR}% 
    \ncarc{#2}{#3} \nbput[npos=#1]{\VaucEdgeLabel{#4}}}
%
\newcounter{anglea}\newcounter{angleb}
\newcommand{\LoopXR}[7]%
   {{\setcounter{anglea}{#2-#4}}%
    {\setcounter{angleb}{#2+#4}}%
    {\EdgeStyle \psset{angleA=\theanglea,angleB=\theangleb,offset=#5,ncurv=#6}% 
    \nccurve{#3}{#3} \nbput[npos=#1]{\VaucEdgeLabel{#7}}}}
\newcommand{\LoopXL}[7]%
   {{\setcounter{anglea}{#2+#4}}%
    {\setcounter{angleb}{#2-#4}}%
    {\EdgeStyle \psset{angleA=\theanglea,angleB=\theangleb,offset=-#5,ncurv=#6}% 
    \nccurve{#3}{#3} \naput[npos=#1]{\VaucEdgeLabel{#7}}}}
\newcommand{\LoopR}[4][{\LoopLabelPos}]%
   {\LoopXR{#1}{#2}{#3}{\LoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\LoopL}[4][{\LoopLabelPos}]%
   {\LoopXL{#1}{#2}{#3}{\LoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\CLoopR}[4][{\CLoopLabelPos}]%
   {\LoopXR{#1}{#2}{#3}{\CLoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\CLoopL}[4][{\CLoopLabelPos}]%
   {\LoopXL{#1}{#2}{#3}{\CLoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\LoopVarR}[4][{\LoopLabelPos}]%
   {\LoopXR{#1}{#2}{#3}{\LoopVarAng}{\LoopVarOff}{\LoopVarSi}{#4}}
\newcommand{\LoopVarL}[4][{\LoopLabelPos}]%
   {\LoopXL{#1}{#2}{#3}{\LoopVarAng}{\LoopVarOff}{\LoopVarSi}{#4}}
\newcommand{\LoopW}[3][{\LoopLabelPos}]{\LoopR[#1]{180}{#2}{#3}}
\newcommand{\LoopE}[3][{\LoopLabelPos}]{\LoopL[#1]{0}{#2}{#3}}
\newcommand{\LoopN}[3][{\LoopLabelPos}]{\LoopL[#1]{90}{#2}{#3}}
\newcommand{\LoopS}[3][{\LoopLabelPos}]{\LoopR[#1]{-90}{#2}{#3}}
\newcommand{\LoopNW}[3][{\LoopLabelPos}]{\LoopR[#1]{135}{#2}{#3}}
\newcommand{\LoopNE}[3][{\LoopLabelPos}]{\LoopL[#1]{45}{#2}{#3}}
\newcommand{\LoopSW}[3][{\LoopLabelPos}]{\LoopL[#1]{-135}{#2}{#3}}
\newcommand{\LoopSE}[3][{\LoopLabelPos}]{\LoopR[#1]{-45}{#2}{#3}}
\newcommand{\CLoopW}[3][{\CLoopLabelPos}]{\CLoopR[#1]{180}{#2}{#3}}
\newcommand{\CLoopE}[3][{\CLoopLabelPos}]{\CLoopL[#1]{0}{#2}{#3}}
\newcommand{\CLoopN}[3][{\CLoopLabelPos}]{\CLoopL[#1]{90}{#2}{#3}}
\newcommand{\CLoopS}[3][{\CLoopLabelPos}]{\CLoopR[#1]{-90}{#2}{#3}}
\newcommand{\CLoopNW}[3][{\CLoopLabelPos}]{\CLoopR[#1]{135}{#2}{#3}}
\newcommand{\CLoopNE}[3][{\CLoopLabelPos}]{\CLoopL[#1]{45}{#2}{#3}}
\newcommand{\CLoopSW}[3][{\CLoopLabelPos}]{\CLoopL[#1]{-135}{#2}{#3}}
\newcommand{\CLoopSE}[3][{\CLoopLabelPos}]{\CLoopR[#1]{-45}{#2}{#3}}
\newcommand{\LoopVarN}[3][{\CLoopLabelPos}]{\LoopVarL[#1]{90}{#2}{#3}}
\newcommand{\LoopVarS}[3][{\CLoopLabelPos}]{\LoopVarR[#1]{-90}{#2}{#3}}
%
\newcommand{\ZZEdge}[2]%
   {\EdgeStyle\ZigzagStyle\nczigzag{#1}{#2}}%
\newcommand{\ZZEdgeL}[4][{\EdgeLabelRevPosit}]%
   {\EdgeStyle\ZigzagStyle\nczigzag{#2}{#3}%
    \naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\ZZEdgeR}[4][{\EdgeLabelRevPosit}]%
   {\EdgeStyle\ZigzagStyle\nczigzag{#2}{#3}%
    \nbput[npos=#1]{\VaucEdgeLabel{#4}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Reprise des macros pstricks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Point}[2]{\pnode#1{#2}}
\newcommand{\Edge}[2]{\EdgeStyle\ncline{#1}{#2}}
%
\newcommand{\VArcL}[5][{\ArcLabelPos}]%
   {\EdgeStyle \psset{style=VaucLArcL}% 
    \ncarc[#2]{#3}{#4} \naput[npos=#1]{\VaucEdgeLabel{#5}}}
\newcommand{\VArcR}[5][{\ArcLabelPos}]%
   {\EdgeStyle \psset{style=VaucLArcR}% 
    \ncarc[#2]{#3}{#4} \nbput[npos=#1]{\VaucEdgeLabel{#5}}}
%
\newcommand{\VCurveL}[5][{\ArcLabelPos}]%
   {\EdgeStyle \psset{angleA=0,angleB=180,ncurv=1}% 
    \nccurve[#2]{#3}{#4} \naput[npos=#1]{\VaucEdgeLabel{#5}}}
\newcommand{\VCurveR}[5][{\ArcLabelPos}]%
   {\EdgeStyle \psset{angleA=0,angleB=0,ncurv=1}% 
    \nccurve[#2]{#3}{#4} \nbput[npos=#1]{\VaucEdgeLabel{#5}}}
%
\newcommand{\LabelL}[2][{\EdgeLabelPos}]%
   {\naput[npos=#1]{\VaucEdgeLabel{#2}}}
\newcommand{\LabelR}[2][{\EdgeLabelPos}]%
   {\nbput[npos=#1]{\VaucEdgeLabel{#2}}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> src/adaptationreqs.tex <==
\section{Mission Adaptation at Runtime}
\begin{itemize}
\item Los requerimientos son:
\begin{itemize}
\item Poder definir una adaptación mientras vuela el robot. Que no sea una opción 
predefinida al momento de haberlo puesto a volar
\item Necesitamos poder especificar la nueva misión de manera independiente de la 
vieja.
\item Necesitamos poder controlar cuando se realizan una reconfiguracion del robnot
\item NEcesitamos poder especificar cuando sucede una el cambio de misión y 
reglas de contorno
\item necesitamos una arquitectura que pueda recibir un controlador nuevo y hacer 
el hotswap. 
\item necesitamos poder dar garantías sobre el comportamiento global del sistema. 
\end{itemize}
\item el related work no lo hace
\item La solución que identificamos combina y extiende estos elementos
\begin{itemize}
\item DCU que lo extendemos con liveness
\item Control hibrido que lo extendemos con capacidad de hotswap y elementos de 
morph
\end{itemize}

\end{itemize}


==> src/arquitectura.tex <==
% !TeX encoding = UTF-8
\section{Hardware and Software Packages}  \label{sec:hwarch}


%\begin{figure}
%\centering
%\includegraphics[width=1.0\linewidth]{src/img/hwarch.eps}
%\caption{Deployment architecture.}
%\label{fig:hwarch}
%\end{figure}


In this section we discuss the main architectural hardware components and a key 
robotics software packages we used: MAVProxy. 


The system (see Figure~\ref{fig:archoverview}) 
comprises of three main hardware components: An \morphOfftheshelf, an 
\morphComputer that runs the adaptation software, and a general 
purpose computer that acts as a 
\morphGCS. 



%\begin{tabular}{|l|l|l|}
%\hline 
%Architectural Component & HW Component &  SW Packages 
%\\
%\hline 
%\morph{Control Panel} &   \hwarch{Ground Control Station}  & [Blinded], MAVProxy\\
%\morph{Synthesiser} & \hwarch{Ground Control Station} & [Blinded] \\ 
%\morph{Controller Management} & \hwarch{Onboard Computer} & MAVProxy 
%Custom 
%Module\\ 
%\morph{Enactor} & \hwarch{Onboard Computer} & MAVProxy Custom Module\\ 
%\morph{Hybrid Control} & \hwarch{Onboard Computer} & MAVProxy Custom 
%Modules\\ 
%\morph{Cont. Var. Control} &\hwarch{Off-the-shelf Vehicle} & Off-the-shelf Flight 
%Controllers \\ 
%\morph{Actuators} & \hwarch{Off-the-shelf UAV} & Off-the-shelf Flight Controllers 
%\\  
%\morph{Vehicle} & \hwarch{Off-the-shelf UAV} & Off-the shelf drivers\\ 
%\hline
%\end{tabular}
%We use an \hwarch{alternative 
%font} to refer to
%Figure~\ref{fig:hwarch}.



The \morphOfftheshelf includes hardware required for flying 
(propellers, rudders, batteries, motors, etc.)  and an embedded processor that runs 
communications software supporting MAVLink~\cite{MAVLink}, a 
lightweight messaging protocol for receiving commands and sending 
telemetry. The processor also runs software for its sensors and actuators including 
various feedback-control loops (often referred as Autopilot or Flight 
Controllers) that implements MAVLink commands such as commanding the 
vehicle to navigate to a specified waypoint, calibrating sensors,  return-to-launch 
emergency commands, and arming and disarming the vehicle. 

% log  - Log management, 
% signing - Packet signing (security)
% wp - waypoint management 
% rally - failsafe
% fence 
% param
% relay - Control of relays
% tuneopt
% arm
% mode
% calibration - calibration
% rc
% auxopt
% misc
% cmdlong
% battery - battery alerts
% terrain
% output
% adsb

In our experimentation we  used a Parrot Ar.Drone 2.0~\cite{Parrot,Parrot2}, a simple 
quadcopter, that has proprietary communication with basic MAVLink capabilities. We 
also used the ArduPilot Software-In-The-Loop (SITL) UAV simulator as 
in~\cite{Baidya18,Barros16}. The SITL simulator allows us to test UAV systems loaded with 
ArduPilot firmware (e.g., custom made as in~\cite{Rokhmana16} or commercial as the 3DR 
Solo Drone~\cite{Baidya18}) without the UAV hardware. This simulator 
(see~\cite{Iterator}) has been used
to seamlessly go from testing to actually flying a custom made 
fixed-wing vehicle (e.g.,~\cite{Mapping}) 
based on a Pixhawk (e.g.,~\cite{Sinisterra17,MAVProxy3}).

Similarly to~\cite{MAVProxy1, Yamazaki19, Rasp2} we expand the computing 
capabilities on 
the 
vehicle by physically fixing on top a general purpose \morphComputer
that runs 
most of the adaptive software architecture. We use a Raspberry Pi 3B+ single board 
computer when simulating with the ArduPilot SITL (to emulate realistic computing 
capabilities for an onboard computer), and a lighter Raspberry Pi Zero 
W mounted on the vehicle when flying the Parrot Ar.Drone 2.0.
  
Finally, for the \morphGCS, a reasonably spec'ed computer is 
needed to run the discrete event controller synthesis software \cite{MTSA}.
 We used a Linux laptop with an Intel i7 3.5GHz processor and 12GB of RAM.
  
  
A key element of the architecture is the MAVProxy software 
package~\cite{MAVProxyGit}. This is a widely used 
(e.g.,~\cite{MAVProxyGit, MAVProxy1,  MAVProxy2,  MAVProxy3}) GNU GPL Python 
  package for UAVs that implements the MAVLink protocol. The package includes 
many standard modules, from firmware management to a camera viewer and a 
moving map, that allow configuring a MAVProxy process to support different vehicle 
setups and mission tasks.

MAVProxy is designed 
to be used as ground control software (e.g.,\cite{MAVProxy3}). That is, MAVProxy 
running on a computer on the ground and providing a 
series of modules that provide mission monitoring capabilities and high-level commands for 
setting up and running missions. However, since MAVProxy provides a simple 
mechanism using custom modules for ad-hoc extensions, 
%with custom code
 it has also been used onboard the vehicle (e.g.,~\cite{MAVProxy1}) to provide new 
functionality.

The architecture runs a lean MAVProxy instance on the \morphComputer
including 
only default standard modules that connect via WIFI or serial communication 
with the embedded processor on the \morphOfftheshelf. However, we 
add a number of custom modules to implement \morphCtrlManagment, 
\morphEnactor and \morphHybridControl layers. 
We discuss these in Section~\ref{sec:swarch}.

Note that the system conformed by the \morphComputer running the 
MAVProxy instance and the \morphVehicle running the flight controllers is a fully 
autonomous vehicle that does not need communication to a ground computer to 
fly its mission.

%We use a Linux laptop with an Intel i7 3.5GHz processor and 12GB of RAM as a 
%\hwarch{Ground Control Station}. This computer 
%plays two roles. The first is to host the \morph{Knowledge Repository} and the 
%\morph{Goal 
%Management} layer. The second is to have direct access to the vehicle for regulatory 
%purposes and contingency management.  

The \morphGCS runs a separate MAVProxy instance, 
configured similarly to most MAVProxy uses. It communicates 
directly with the vehicle to perform the initial mission setup, to receive telemetry and to 
allow taking control over the vehicle if necessary. Telemetry data is shown on a GUI to 
users using standard modules. This ground MAVProxy instance communicates 
with the airborne MAVProxy instance using a custom protocol over TCP/IP via WIFI to 
support the interactions between the \morphCtrlManagment layer and 
the\morphSynthesiser.

Note that although MAVProxy only supports natively MAVLink there are 
MAVLink  
wrappers for alternative protocols such as~\cite{RosettaDrone} for DJI 
speaking drones (e.g., the DJI Phantom 2~\cite{DJI}). Thus, the architecture can be 
used with a broad variety of vehicles.

 
The other software package that we use is~\cite{MTSA} 
which provides functionality for specifying discrete event control problems as 
described in Section~\ref{sec:Preliminaries} and provides a backend 
\morphSynthesiser layer.



\section{UAV Software Architecture} \label{sec:swarch}
\begin{figure}
\centering
\includegraphics[width=1.0\linewidth]{src/img/swarch.eps}
\caption{Software architecture.}
\label{fig:swarch}
\end{figure}

In Figure~\ref{fig:swarch} we depict the software architecture of the Adaptive UAV 
system.
%that implements the MORPH reference architecture described in 
%Section~\ref{sec:morph}.
 We use an \swarch{alternative font} when referring to software components in
Figure~\ref{fig:swarch} and structure the section based on the main deployment 
components  described in 
Section~\ref{sec:hwarch} and architectural elements of Figure~\ref{fig:archoverview}. 
% \hwarch{Ground Control Station} and \hwarch{UAV 
%Platform}.

%For each component we provide an overview of how the software architecture 
%components in 
%Figure~\ref{fig:swarch} relate to MORPH (Section~\ref{sec:morph}) and to the 
%hardware 
%(Section~\ref{sec:hwarch}). We then describe each component in more detail. 
%Note that Figure~\ref{fig:swarch} also illustrates which components we developed 
%(\swarch{MTSA Java Packages} and \swarch{Python Modules}).

\subsection{Ground Control Station}
%The right hand side of Figure~\ref{fig:swarch} corresponds the \morph{Knowledge 
%Repository} layer of MORPH. The component group \swarch{Control Panel} 
%corresponds to 
%MORPH's \morph{Goal Model}  (i.e., \swarch{Model Editor}, \swarch{Discretizer}, 
%\swarch{Code Editor}, and \swarch{Mission Viewer}). Bellow are components that 
%map directly to MORPH's \morph{Inference} and \morph{Log} elements. They all 
%execute on 
%the 
%\hwarch{Ground 
%Control Station}. There are also a number of back-end components, 
%% The \swarch{Hybrid Module TX} manages the transmission of code modules 
%%for dynamic reconfiguration of the UAV's software. 
%the ones on the top-left part correspond to MORPH's \morph{Goal Management} 
%layer. 
%Component \swarch{Goal Model Manager} maps directly to MORPH while the 
%\swarch{GR(1) 
%Synthesiser} implements MORPH's \morph{Control Problem Solver}. 
%
%%As 
%%both execute on 
%%the \hwarch{Ground Control Station} there is a component (\swarch{Controller TX}) 
%%that 
%%manages transmission of controllers to the UAV.
%
%%On the right we can identify two main sub-components: the \swarch{Control 
%%Panel} 
%%that allows a 
%%user to interact with the adaptive system and the rest of the modules we will refer 
%%to as 
%%\emph{Back-end} since its operation is invisible to the user. 
%%\su{El diagrama no tiene "back end". Creo que hay que agregarlo}
%
%We first discuss the components in the \swarch{Control Panel} which which users 
%interact directly, and then discuss the rest of the components running back-end on 
%the \hwarch{Ground 
%Control Station}.

\subsubsection{\morphControlPanel} \label{sec:controlpanel}
A typical view of the \morphControlPanel can be seen in 
Figure~\ref{fig:controlpanel}.

The \swarch{\textbf{Mission Viewer}} is a collection of MAVProxy standard modules 
that include a \textit{Horizon module} that creates a horizon window, showing common 
real-time flight information such as speed, attitude, and 
heading. A \textit{GUI Console module} displays additional information about the UAV's 
current state including flight mode and arming state, GPS status, system voltage, 
telemetry radio link quality, and availability of different sensors (e.g., inertial 
system, magnetometer, airspeed), amongst other sensor readings.  A \textit{Moving Map 
module} is used to show the UAV's current position, waypoints and allows users to 
define regions of interest. 
Finally, there is a \textit{Command line} window for the user to run various 
commands that MAVProxy modules introduce when loaded (e.g., \textit{arm throttle, takeoff, 
land,} etc.).


\begin{figure}
\centering
\includegraphics[width=1.0\linewidth]{src/img/control-panel.eps}
\caption{\swarch{Control Panel}  during 
Section~\ref{sec:unexgoalchange} mission. 
%Note that some modules/components may not be loaded 
%(e.g., 
%\swarch{Code Editor}).
}
\label{fig:controlpanel}
\end{figure}

To start a mission, a user will typically start by interacting with the UAV to reset and 
calibrate its various sensors through the \textit{Command Line} and then 
define using the \textit{Moving Map} the discretization region and other areas of 
interest such as no-fly zones and areas to visit or cover. If the UAV is already flying a 
mission, new areas of interest can be defined.

The \swarch{\textbf{Discretizer}} component produces a discretized version of the areas 
defined using the \textit{Moving Map} (see Figure~\ref{fig:controlpanel}). 
Discretization 
is in form of a grid where the user can determine the size of the square grid cells and 
the angle in which the grid is built. Cell size is critical as it must be larger than the 
error in estimation of the actual location of the UAV and also larger than the expected 
drift the UAV may have while following waypoints. 

The \swarch{Discretizer} produces two different discrete representations. The first, 
in  the input language used to define and solve control problems (c.f., 
\swarch{Goal Model Manager}). It creates fluent definitions for locations and regions 
(e.g., \arrivedfl{2}, \arrivedfl{\nfold}, see Section~\ref{sec:fltl}).  It also encodes a 
cell adjacency matrix modelled as an LTS (see Figure~\ref{fig:discretization}).
The criteria to decide if a cell belongs to a 
user defined region is that the centre of this cell is included in the region. These 
expressions are passed on to the \swarch{Model Editor} to support specification of 
UAV missions.  

The second discrete representation is a mapping from $(x, y)$ coordinates to 
discrete 
locations and vice-versa.  This map is uploaded to the UAV via the \swarch{Hybrid 
Module TX} and used by the \swarch{Hybrid Layer} to convert discrete events 
such as \goN{5} into $(x, y)$ coordinates and vice-versa. 

The \swarch{\textbf{Code Editor}} is for writing Python code that will be uploaded onto 
the UAV. The code is intended to implement new sensor or actuator behaviour. Such as, for 
instance, a sensor that when commanded \photo, interacts with the 
onboard camera, takes a picture, processes it to detect if there is in view a feature 
than may be a lost person using a red jacket, and returns a 
\formatAction{found}/\formatAction{not.found} event accordingly (see code sample 
in supplementary material).

To integrate into the existing architecture, we require the code to extend a Python class 
\textit{HybridModule} (which in turn is a subclass of the MAVProxy standard 
\textit{Module} class).
% , see the example Person Sensor code in Listing~\ref{lst:personsensor}. 
The \swarch{Hybrid Module} can then subscribe to controllable actions from the discrete 
controller and publish uncontrollable discrete events to it.
% (see \emph{controllables} list) 
%from the \swarch{Enactor} and to 
% and publish events.
%to the \emph{event_queue} of the \swarch{Enactor}
%  It can also contain an internal process 
% (see \emph{_process_type} flag) to process complex computations (e.g., 
% \emph{_image_process} method).
% 
% \begin{lstlisting}[caption={Person Sensor. Between 
% brackets we indicate fragments of missing code.},label={lst:personsensor},language=Python]
% from MAVProxy.modules.hybrid_mod import HybridModule
% # { other imports }
% class PersonSensor(HybridModule):
%     def init(self):
% 	# Hybrid module has a internal process
% 	self._process_type = 1
% 	# Controllable actions implemented
%         self.controllables = ['sense_person']
% 
%     def sense_person(self):
% 	# call the "image_process" method in the
% 	# internal process
% 	self._add_to_command_queue('image_process')
% 
%     def _image_process(self):
% 	# called by the internal process
%         # { capture and filter image }
%         if (person):
% 	    # add to Enactor event queue
%             self._add_to_event_queue('found')
%             # { send to the GCS a FOUND message }
%         else:
% 	    # add to Enactor event queue
%             self._add_to_event_queue('not_found')
%         
% \end{lstlisting}

The \swarch{\textbf{Model Editor}} component is an editor that is intended for writing 
discrete event controller synthesis problems. These problems can be written as a 
combination of  LTS and LTL as described in Section~\ref{sec:Preliminaries}. The 
specification of LTS models is done using the process algebraic notation 
in~\cite{magee06} 
and typically includes descriptions of the sensors and robot 
capabilities  (e.g., Figure~\ref{fig:LTS}).

A number of different styles of control problems can be defined, including 
non-deterministic and partial-observability 
problems~\cite{DBLP:journals/tse/CiolekBDPU17} 
 for safety, reachability, 
non-blocking reachability~\cite{ramadge89}, and GR(1) \cite{piterman06} 
properties. It also 
supports specification of controller update problems as described in 
Section~\ref{sec:DCU}.


\subsubsection{\morphSynthesiser} \label{sec:backend}
It is comprised by two components of a synthesiser tool  %MTSA, 
a \swarch{Goal Model Manager} and a \swarch{GR(1) 
Synthesiser}, and the MAVProxy 
components that do not interact directly 
with users, including \swarch{Hybrid Module TX}, \swarch{Controller TX}, 
\swarch{Log}, and \swarch{Inference} 
components.

The \swarch{\textbf{Goal Model Manager}} inputs the specification of a control problem 
defined by the user and performs the necessary pre- and post-processing to solve it 
with 
the \swarch{GR(1) Synthesiser}. For example, for partial-observability and 
non-determinism this involves a modified~\cite{DBLP:journals/tse/CiolekBDPU17} 
subset construction~\cite{aho1985compilers}. For 
controller updates, post-processing is required to extract the update controller from the 
solution that the \swarch{GR(1) Synthesiser} returns~\cite{Nahabedian-TSE}. 
The \swarch{\textbf{GR(1) Synthesiser}} implements a basic rank-based algorithm for 
solving GR(1) games as originally described in~\cite{piterman06} but adapted to 
event-based 
descriptions. %~\cite{dippolito13}. 

The \swarch{\textbf{Hybrid Module TX}} uploads Python code to the UAV, be it the 
automated result of the \swarch{Discretizer}  component (i.e., the mapping between 
real coordinates and discrete cells) or the user's manually coded sensors and 
actuators. Similarly, the \swarch{\textbf{Controller TX}} component manages the 
transmission 
of controllers from the \swarch{Ground Control Station} to the \swarch{Off-the-shelf 
UAV}. 
The \swarch{\textbf{Log}} and \swarch{\textbf{Inference}} components are integrated in 
the default behaviour of MAVProxy standard modules. For instance, all received 
telemetry is stored in a log file. This file can be used to analyse in- and post- flight 
the vehicle performance and trajectory. MAVProxy modules that provide graphical output 
typically include inference 
procedures that allow producing meaningful data from received telemetry. A typical 
example is the \swarch{Horizon} which must perform geometric operations over raw sensor 
data to provide a view of the UAV's attitude. Similarly, one could build a custom module 
that implements a runtime monitor to estimate the battery level using an energy 
consumption model as in~\cite{Wei18} and the raw position telemetry data.


\subsection{UAV Platform}
Mid-left components of Figure~\ref{fig:swarch}   (\swarch{Update Manager} and 
\swarch{Fallback Manager}) implement the \morphCtrlManagment layer described in 
Section~\ref{sec:morph}, while component \swarch{Discrete Control} maps directly to 
its counterpart, all of which run on the \morphComputer.

%The \swarch{Hybrid Control Layer}, comprises various components running on 
%the \hwarch{Onboard Computer}, implements MORPH's \morph{Effectors} and 
%\morph{Probes} in the \morph{Target 
%System} and interacts with the  
%software running on the \hwarch{Off-the-shelf Vehicle}.

%The main components of this part of the system can be divided in: \swarch{Control 
%Manager}, \swarch{Enactor}, \swarch{Hybrid Control Layer} and \swarch{Embedded 
%System}.

\subsubsection{\morphCtrlManagment} Comprised of two components.

The \swarch{\textbf{Update Manager}} receives controllers from the ground station and 
deploys them onto the \swarch{Discrete Control}. If there is no controller currently 
running, then deployment is trivial. If there is one, then the \swarch{Update Manager} 
must perform a hot-swap. For this, the initial state of the new controller $C'$ must be 
derived using the state mapping specified as part of the mission change (see 
Section~\ref{sec:DCU}).
%where $s_i$ is the current state of the controller being enacted  ($C$). This means 
%finding in $C'$ a state that is bisimilar to $s_i$ up to \hotSwap.  Once found 
%$H(s_i)$, 
%controller  $C_u$ is deployed in the \swarch{Enactor} setting its initial state to 
%$H(s_i)$. Note that there is one added technical difficulty: while $H(s_i)$ is being 
%computed, the current state of $C$ may change. Thus, while $H(s_i)$ is being 
%computed, the 
%trace that $C$ takes is recorded and replayed from $H(s_i)$ before hot-swapping.   


The \swarch{\textbf{Fallback Manager}} component can implement various goal 
degradation 
policies as described in~\cite{DIppolito:2014:HBP:2568225.2568264}
%MORPH's \morph{Strategy Management}. 
We have implemented a basic fallback plan which is triggered when the 
\swarch{Discrete Control} receives an event from the 
\swarch{Hybrid Control Layer} that according to the current state of the controller, 
the event should not have occurred. In this case, the fallback plan kicks in taking the 
UAV  to the point of launch and/or landing.

\subsubsection{Enactment} The \swarch{Discrete Control} component runs as an 
independent process and manages 
event queues to receive and process events from the hybrid architecture. It stores the 
current controller and changes its current state based on the events that occur. When 
there are 
no events to process, if the current state has at least one enabled controllable 
transition, one controlled transition is picked and the corresponding command is sent to 
the \swarch{Hybrid Control Layer}. If an unexpected event occurs, it raises an 
exception to the \swarch{Fallback Manager}.  

\subsubsection{Hybrid Control Layer} This layer is responsible for mediating between the 
\morphEnactor layer and the \morphOfftheshelf.
%Thus, on one hand it 
%receives high-level commands that must be implemented via lower level calls to 
%vehicle 
%functionality, including the mapping of discrete locations to coordinates in 
%$\reals^2$. 
%On the other hand, it generates high-level events based on low-level telemetry data 
%or as a 
%result of complex computation of sensor information. 
The layer's main components are custom \swarch{\textbf{Hybrid 
Modules}}. A simple \swarch{Hybrid Module} may process battery 
telemetry packets and produce \formatAction{low.battery} events when the voltage readings 
are 
bellow a certain threshold. A more complex \swarch{Hybrid Module} is the person sensor 
described in Section~\ref{sec:controlpanel}, as it involves image processing algorithms to 
be able to decide which discrete event to generate: \formatAction{found} or 
\formatAction{not.found}.
% shown in Listing~\ref{lst:personsensor}.

The \swarch{\textbf{Discrete/Continuous Conversion}} is used by 
\swarch{Hybrid Modules} that require reasoning about the physical space in which the UAV 
moves. For 
instance, the \swarch{Hybrid Module} that implements the \goN{i} commands 
first obtains the centre point of the discrete location with the help of this component 
and then calls the \swarch{Motion Planner} to actually move the vehicle to the location. 

The \swarch{\textbf{Motion Planner}} can vary significantly depending on the UAV being 
flown and the degree to which the off-the-shelf control of the UAV guarantees reaching 
the target location. Different algorithms can be implemented in this component to guide 
the UAV to the target location (e.g.,~\cite{Ji15,Livingston13}). We 
implemented a fairly simple planner that doesn't take into account obstacles (static or 
dynamic). For quadcopters, the \swarch{Motion Planner}  simply requests the UAV to fly to 
the target location, with the possibility of waiting some time at the location. In the 
case of the fixed-wing plane, which has turn-radius limitations, sending a target 
location that involves a sharp turn will simply make the plane miss its target. In these 
cases, the  \swarch{Motion Planner} computes a Dubins path~\cite{Song17} and discretizes 
it into a set of intermediate coordinates. This simple planner can be replaced modularly 
by more complex ones that implements standard motion planning algorithms (e.g, 
rapidly-exploring random tree~\cite{Carpin02}, probabilistic roadmaps~\cite{Kavraki96}, 
A*~\cite{Song17}).

%\begin{itemize}
%\item HModules: Called by MAVproxy regularly, can generate events. Publish 
%commands that they implement and are called by Enactor. Explicar que pueden 
%implementar varios sensores y actuadores. 
% Sensores que puede correr en paralelo si son procesamientos.Explicar c�mo se 
% registran eventos con c�digo y como una actuador recibe el procesador para poder 
% generar eventos 

The \swarch{\textbf{Module Loader}}  can receive Python code for \swarch{Hybrid 
Modules} 
from the \hwarch{Ground Control System} and stores them until a \reconfigure command is 
produced by the \swarch{Discrete Control}. At this point, it registers the new 
\swarch{Hybrid 
Modules} 
with the \swarch{Discrete Control} and deregisters any \swarch{Hybrid Modules} not in use 
any 
more. 

\subsubsection{\morphOfftheshelf}
Although this part of the system depends heavily on the \morphOfftheshelf being 
used, we can divide most of them in two components: 
the \swarch{\textbf{Flight Controllers}} that implement various \morphFeedback to 
maintain the vehicle in-flight, reading from the available \morphSensors (e.g., airspeed 
and GPS readings) and outputting to the different actuators (e.g., motors, servos), 
and the \swarch{\textbf{MAVLink Communications}} handler that provides an interface 
between external agents and the \swarch{Flight Controllers}, as well as other vehicle 
\morphSensors and \morphActuators (e.g., battery level, camera gimbal).








==> src/dcu.tex <==
\subsection{Dynamic Controller Update}
\label{sec:DCU}
%
%
%
%The relabelling operation defines an LTS by relabelling or removing transitions from 
%another LTS. 
%It does so by either removing a transition when its label is not defined in the 
%relabelling 
%function, or by changing the label according to the relabelling function.
%
%\begin{definition}\emph{(Relabelling operator)} \label{def:relabelling}
%Let $E = (S_E, A_E,$ $\Delta_E, e_0)$ be an LTS and $f:A_E \rightarrow \emph{Act}$ 
%be an injective partial function.
%The relabelling operation $[E]_f$ is an LTS $(S_E, A', \Delta_f, 
%e_0)$, where $\Delta_f$ is the smallest relation that satisfies the rule below:
%\begin{center} 
%	\begin{tabular}{lcl}
%	    $\!  \dfrac{(e,\ell,e') \; \in \; \Delta_E}
%	    {(e,f(\ell),e') \; \in \; \Delta_{f}} 
%	    \, {}$ %&
%%	    $\!  \frac{(e, \ell, e') \; \in \; \Delta_E} 
%%	    {(e,\ell,e') \; \not\in \; \Delta_{f}}
%%	    \, {\scriptstyle \ell \, \not\in \, Dom(f)}$
%	\end{tabular} 
%\end{center}
%\end{definition}

%\begin{property}\label{prop:relabel}
%Let $E, B$ be deterministic LTS, and $f: Act \rightarrow Act$ be a partial injective 
%function, 
%then, the 
%following equivalence holds: $[E\|B]_f \sim [E]_f \| [B]_f$ 
%\end{property}

%\begin{proof}[Proof of Property~\ref{prop:relabel}]
%We postulate the binary relation $=$ as a bisimulation. Then, for every state $(e,b)$ 
%the following 
%holds.
%
%\vspace{1em}
%\noindent
%\begin{tabular}{rclc}
%$(e,b) \xrightarrow[{[}E\|B{]}_f]{f(\ell)} (e',b')$ & iff & $(e,b) \xrightarrow[E\|B]{\ell} 
%(e',b')$ 
%& iff \\
%$e \xrightarrow[E]{\ell} e'$ or $b \xrightarrow[B]{\ell} b'$ & iff &
%$e \xrightarrow[{[}E{]}_f]{f(\ell)} e'$ or $b \xrightarrow[{[}B{]}_f]{f(\ell)} b'$ & iff \\ 
%\multicolumn{4}{c}{$(e,b) \xrightarrow[{[}E{]}_f\|{[}B{]}_f]{f(\ell)} (e',b')$}
%\end{tabular}
%
%As $f$ is an injective function, it is not possible to generate a non-deterministic 
%LTS from 
%relabelling.
%\end{proof}

%We introduce an interrupt handler operation that defines the sequential execution of 
%two LTS where 
%the switch from one LTS to the other is triggered by an event ($\alpha$).
%
%\begin{definition}\emph{(Interrupt handler)}  \label{def:lightning}
%Let $E$ $=$ $(S_E, A_E, \Delta_E, e_0)$ and $N$ $=$ $(S_N, A_N, \Delta_N, n_0)$ be 
%LTS, 
%$H$ be an interrupt handler relation such that $H \subseteq (S_E \times S_N)$, and
%$\alpha$ be an interrupt event such that $\alpha \not\in (A_E \cup A_N)$,.
%
%The interrupt handler $E \lig{H}{\alpha}N$ is an LTS 
%defined as $(S_E \cup S_N, A_E \cup A_N \cup \{\alpha\}, \Delta_{\lightning}, 
%e_0)$, where $\Delta_{\lightning}$ is the smallest relation that satisfies the 
%rules below:
%\\
%\begin{center} 
%	\begin{tabular}{lr}
%	    $\!  \dfrac{(e,\ell,e') \; \in \; \Delta_E}
%	    {(e,\ell,e') \; \in \; \Delta_{\lightning}}$
%	    &
%   	    $\! \dfrac{(n,\ell,n') \; \in \; \Delta_N}  
%        {(n,\ell,n') \; \in \; \Delta_{\lightning}}$ 
%\\
%\\		
%		\multicolumn{2}{c}{
%    	$\!  \dfrac{} 
%	    {(e,\alpha,n) \; \in \; \Delta_{\lightning}}
%	    \, {(e,n) \, \in \, H}$
%	    }
%	\end{tabular} 
%\end{center}
%\end{definition}

%\begin{property} \label{prop:lig}
%Let $A, B, C$ and $D$ be LTS,
%$H$ and $K$ be interrupt handlers relations defined for each state of $A$ and $K$ 
%respectively,
%$\ell$ be an interrupt event,
%then, the following equivalence holds:
%\begin{equation*}
%P = ( (A \;\lig{H}{\alpha}\; B) \;\|\; (C \;\lig{K}{\alpha}\; D) ) \;\;\; \sim \;\;\; (A\|C) 
%\;\lig{R}{\alpha} \; (B\|D) = Q
%\end{equation*}
%where $R$ is an interrupt handler such that $((a,c),(b,d)) \in R$ iff $(a,b) \in H$ and 
%$(c,d) 
%\in 
%K$. 
%\end{property}
%

%\begin{property} \label{prop:lig}
%Let $A, B, C$ and $D$ be LTS, 
%$H$ and $K$ be interrupt handlers relations and
%$\ell$ be an iterrupt event,
%then, the following equivalence holds:
%\begin{equation*}
%(A \;\lig{H}{\alpha}\; B) \;||\; (C \;\lig{K}{\alpha}\; D) \sim ( (A||C) \;\lig{H'}{\alpha}\; 
%B) 
%\;||\; (( A||C)\; \lig{K'}{\alpha}\; D)
%\end{equation*}
%where 
%$((a,c),b) \in H'$ iff $(a,b) \in H$, and,
%$((a,c),d) \in K'$ iff $(c,d) \in K$.
%\end{property}

%\begin{proof}[Proof of Property~\ref{prop:lig}]
%	We postulate the binary relation $\mathcal{R}$ such that for all $(a,c) \in A\|C$, 
%$(a,c) 
%	\mathcal{R} (ab,cd)$ where $(ab,cd)$ are states before $\alpha$ in $P$. 
%	For all $(b,d) \in B\|D$, $\mathcal{R}$ is the relation $=$.
%	
%	\noindent
%	\begin{tabular}{rcll}
%		%\multicolumn{2}{c}{$(ab_0,cd_0) \sim$ $(a_0,c_0)$} & 
%%\multicolumn{2}{c}{$(ab_0,cd_0)$, 
%		%$(a_0,c_0)$ 
%		%initial states.}\\
%		$a \xrightarrow{\ell} a'$ or $c \xrightarrow{\ell} c'$ & iff & $(a,c) 
%		\xrightarrow{\ell} (a',c')$ & $\ell \neq \alpha$\\
%		& & $(a,c) \xrightarrow{\ell} (a',c')$ &\\
%		$a \xrightarrow{\alpha} H(a)$ and $c \xrightarrow{\alpha} K(c)$ & iff & 
%		\multicolumn{2}{l}{$(a,c)  \xrightarrow{\alpha} H'(a,c)$}\\
%		& & \multicolumn{2}{l}{$(a,c)  \xrightarrow{\alpha} K'(a,c)$}\\
%	\end{tabular}
%When transitioning through $\alpha$ both LTS reach bisimilar states because 
%interrupt handler 
%relations $H'$ and $K'$ were defined to do so.
%\end{proof}




%In this section we precisely state the problem of dynamic update of discrete event 
%controllers. In 
%other words, 
%To  formalise what it means for a controller updated to be hot swapped into a 
%system at 
%runtime while guaranteeing that the resulting system will eventually transition 
%correctly to the 
%new system specification. We first formalise controller hot-swapping, then 
%environment 
%reconfiguration and finally a notion of correctness.

%\subsection{Dynamic Controller Update}
%We now formally define the behaviour of a system in which the current controller is 
%hot swapped by another one. 

Assume a controller $C$ is being enacted to achieve a goal $\varphi$ in a UAV system 
that is assumed to behave like $E$. Due to an unexpected change of goal, 
assumptions or capabilities (controlled and uncontrolled events), a new controller is 
required to be put in place to achieve $\varphi'$ under environment $E'$. 

Managing this change is not as simple as synthesising a controller $C'$ for $E'$ and 
$\varphi'$. There are various important subtleties. The first is how to set the initial 
state of 
$E'$ based on the current state of $E$. This can be easily addressed by simply providing a 
mapping of states of $E$ to $E'$. The second is that as synthesis takes time, the current 
state of $E$ may change and so will the intended initial state of $E'$.  
Thus a takeover strategy that works from any state of $E$ (or at least reachable states from 
$E$'s current state) must be synthesised.  The third is that there may be inconsistencies 
between the old and new mission goals; this requires more explanation.
%
%To start, note that the initial state of $E'$ depends on the current state of $C 
%\| E$ (or for simplicity $C$ because $C$ is legal w.r.t 
%$E$). For instance, at the time of 
%deciding to compute $C'$ the 
%UAV may be in position $1$ but by the time $C'$ has been computed (under the 
%assumption of a UAV starting at position $1$), the UAV may be at $5$. As the state in 
%which the system will be in by the time synthesis of $C'$ has finished is unknown. We 
%require having a $C'$ for every possible state in which $C$ may be in. 
%
%Another way of thinking about the problem of synthesising $C'$ is that there is a system 
%that behaves as $C\|E$ and when an event \hotSwap occurs, $C'$ must take 
%control (whatever the state of $C\|E$ is) and guarantee $\varphi'$ assuming $E'$ 
%where the initial state of $E'$ is inferred from that of $C$ via some relation $H$.
%We refer to the hot-swap composition of two LTS as $(A \; \lightning_H^{\hotSwap} \; 
%B)$ where $\lightning$ is an interrupt operator that sets the state $B$ via a 
%$\hotSwap$ transition according to the current state of $A$ and mapping $H$.

\example{
Consider a new mission in which the no-fly zone changes to the top locations 
($0-2$) and patrolling is to be between $3$ and $5$ (i.e. $\left(\Gl \F 
\arrivedfl{3} \wedge \Gl \F \arrivedfl{5} \right) \wedge \left( \Gl \neg 
\arrivedfl{\region{\nfnew}} \right) )$. 

% Although $E$ and $E'$ are structurally 
% equivalent, 
% the initial state of $E'$ when starting the new mission depends on the current state of 
% the mission $ \left(\Gl \F \arrivedfl{0} \wedge \Gl \F \arrivedfl{2} \right) \wedge \left( 
% \Gl \neg 
% \arrivedfl{\region{\nfold}} \right)$
% %The LTS to be considered for computing $C'$ is actually a hot-swap composition of 
% %Figure~\ref{fig:controller} ($C\|E$) and \ref{fig:composition} ($E'$) where states in the 
% %former are linked to states of the latter via \hotSwap transitions according to 
% %the 
% %relation 
% and can represented with relation $\set{(0 \rightarrow 0),$ $(1 \rightarrow 1),$ $(2 
% \rightarrow 2), $ 
% $(3 \rightarrow 4),$ $(4 \rightarrow 5),$ $(5 \rightarrow 8),$ $(6 \rightarrow 2),$ $(7 
% \rightarrow 3)$, $(11 \rightarrow 4),$ $\ldots}$. 

}


Note that in the running example, it is not possible switch from the old goal 
($\varphi$) to the new goal ($\varphi'$) without violating one of them. If the UAV is in 
locations $0-2$ then it cannot switch to achieving ($\varphi'$)  because $0-2$ 
are in the new no-fly area. If the UAV is moved to locations $3-5$ to comply to 
($\varphi'$) then it is violating ($\varphi$). This is an extreme example that motivates 
the need for specifying requirements that deal with \textit{transitioning behaviour} 
between missions. 

To aide specification of transition requirements we introduce two new controlled 
events \stopOld 
and \startNew which the new controller will signal when it stops guaranteeing 
$\varphi$ and starts guaranteeing $\varphi'$. 

The \emph{standard transition requirement} is one that states that the system is always 
either satisfying the old or the new specification. In other words that if the old 
specification has been dropped or the new one has been started: $T = \Gl (\neg 
\stopOldfl \vee \startNewfl)$, where \stopOldfl and \startNewfl are fluents initialised 
to false that become true when event \stopOld and \startNew occur, respectively. They 
never become false 
again.

\example{
To resolve the inconsistency between the old and new no-fly zones and the 
standard transition requirement, which forces one or the other to 
hold, we must allow a period in which neither $\varphi$ nor $\varphi'$ are being 
achieved. There is no single transition requirement for this, indeed it is domain 
dependent. One choice may be to restrict movement to the left side of the grid. That is, 
when the old specification is dropped, the UAV must be at locations $0$ 
or $3$ until the new one is adopted: 
\begin{equation} \label{eqn:T-arrived03}
T = \Gl \big(\stopOldfl \implies
\left((\arrivedfl{0} \vee \arrivedfl{3}) \W \startNewfl \right) \big)
\end{equation}

Assume the UAV is patrolling according to $\varphi$ between $0$ and $2$ avoiding 
\region{\nfold}. When the need to change mission occurs, it is in location $0$. By the 
time a controller $C'$ that manages the update to the new mission $\varphi'$ under 
transition requirement (\ref{eqn:T-arrived03}) is synthesised, the UAV is on its way to 
$1$. 
Thus, the last event to occur would be \goN{1}. At this point, $C$ would be replaced by 
$C'$ 
(\hotSwap) and then what $C'$ should do is the following: wait for \arrivedN{1} and 
then move back to location $0$ (\goN{0}, \arrivedN{0}) to be able to declare (consistently 
with $T$) that the old goal is being dropped (\stopOld). It would then have to move to 
$3$ (\goN{3}, 
\arrivedN{3}) which is still consistent with $T$ and then, being out of the new no-fly 
zone, declare \startNew. From then on it should visit $4$, $5$, $4$, $3$, $\ldots$
}



%
%Suppose that the controller $C$ is to be hot swapped with a new controller $C'$. In 
%some cases, the initial state of $C'$ at the time in which it is swapped in can be fixed 
%at design time. However, in general the initial state of $C'$ depends on the state of 
%the system at the instant at which  $C'$ takes control. Thus, a function $H$ for 
%setting 
%the initial state of $C'$ based on the current state of $C$ is required.
%
%\begin{definition}\emph{(Hot Swap)} \label{def:hotswap}
%Let $E$, $C$ and $C'$ be LTS where the states of the latter two are $S_C$ and 
%$S_{C'}$ and none of them have \hotSwap in their alphabet. Let $H \subseteq S_C 
%\times S_{C'}$
%% be a total function from $S_C$ to $\powerset{S_{C'}} \setminus \emptyset$.  NO 
%%HACE FALTA, LO PEDIMOS EN CORRECTITUD
%The behaviour 
%resulting from running 
%$C$ in 
%$E$ and 
%hot swapping it with $C'$ is defined by $(C \; \lightning_H^{\hotSwap} \; C') \| E$
%\end{definition}

%
%. Consequently, in $(C \; \lightning_H^{\hotSwap} \; C') \| E$ the event 
%$\hotSwap$ is 
%unconstrained and can occur only once but at any point. Indeed, this models that 
%\hotSwap will be 
%triggered by the underlying enactment infrastructure 
%which will use $H$ to set the current state of $C'$ according to that of $C$.
%

%At the top of Figure~\ref{fig:hotSwap} we depict a controller $C$ for a reduced (i.e, 
%two tool) version of the production cell with slightly modified objectives (reduced to 
%aid understandability of the diagram): after 
%receiving a raw element $x$ in the tray (\emph{in(x)}), the controller will 
%\emph{drill(x)} and 
%\emph{polish(x)} the element. 
%The \emph{out(x)} command will be executed by the controller when 
%both tools were applied to the element correctly.
%At the bottom of the same figure, we show a controller $C'$ that instead of 
%polishing elements, it will paint them (\emph{paint(x)}) instead.
%The combination of both controllers plus the dotted \hotSwap transitions is the 
%result of $(C \; 
%\lightning_H^{\hotSwap} \; C')$, where the \hotSwap transitions coincide with 
%relation $H$
%from states in $C$ to states in $C'$ (i.e $H =$ $ 
%\{(0,0),(1,1),(2,2),(3,3),(4,3),(5,3)\}$).


%It is important to note that the communicating alphabet of $C 
%\lightning_H^{\hotSwap} C'$ is a superset of the alphabets of $C$ and $C'$. Thus, 
%an 
%event $\ell$ that is in the alphabet of $C$ that is not in that of $C'$  will be 
%restricted from occurring after $\hotSwap$ in the composition $(C \; 
%\lightning_H^{\hotSwap} \; C')$ because there is no transition in $C'$ labelled with 
%$\ell$ (see parallel composition, Definition~\ref{def:parallelComposition}). The 
%same 
%holds for events in the alphabet of $C'$ that are not in the alphabet of $C$, where 
%such events will be constrained from occurring in $(C \; 
%\lightning_H^{\hotSwap} \; C')$ before $\hotSwap$. For instance, in the  example, 
%$C$ has in its alphabet \emph{polish(x)} but not \emph{paint(x)} which is in the 
%alphabet of $C'$. The term $C \lightning_H^{\hotSwap} C'$ will prohibit the 
%occurrence of \emph{paint(x)} before \hotSwap and the occurrence of 
%\emph{polish(x)} 
%after hotSwap. 


%Finally, we require the controller to be an LTKS with no propositions. This is akin to saying that the controller cannot sense nor modify propositions directly, it can only sense via event synchronisation. 



%\subsection{Controlling Reconfiguration}
%Controllers are updated in systems because the system goals or the environment 
%assumptions have changed. 
%The 
%latter may be due to adoption of unrealistic or invalid assumptions or because the 
%executing (software and/or 
%hardware) configuration environment of the controller has changed: an API that 
%provides services to the 
%controller needs to be changed, a sensor or actuator is not working with the desired 
%precision. In the case of 
%our example, 
%the required change in the configuration environment is that the Polishing tool is no 
%longer needed and 
%Paint tool is. This involves unloading the driver for the Polish tool and loading the 
%driver for the Paint 
%tool. 

When a controller needs to be updated it is quite common that the infrastructure that 
it is controlling must be changed too. For instance, a new software component may 
need to be loaded and bound to existing components.  This is often referred to as 
structural adaptation~\cite{MORPH15} or software architecture 
reconfiguration~\cite{Tajalli2010}.
%A change in the executing configuration environment typically needs to be managed 
%and coordinated with the 
%overall behaviour that is satisfying the system goals. Thus, the controller that 
%manages the dynamic update 
%needs to be able to control when reconfiguration should occur, and it must signal 
%the change at a point in 
%time where the whole update can be guaranteed to be correct. 
%Note that the latter setting guarantees planned environment changes where the 
%update controller chooses when to 
%reconfigure.
%
%We model a controller that is capable of changing its environment's configuration 
%dynamically with the term 
%$C' \| (E \lightning_R^{\reconfigure} E')$ assuming that \reconfigure is part of the 
%communicating 
%alphabet of $C'$. This means that, as opposed to \hotSwap, \reconfigure is 
%controlled by the 
%controller $C'$. 
For simplicity of presentation, here we assume atomic 
reconfiguration modelled by the event \reconfigure. More complex reconfigurations can be 
modelled in the spirit 
of~\cite{Tajalli2010, alvares2017domain}.



\example{
Assume that in addition to the changes in no-fly  and patrolling areas, the mission is 
required to take a picture at every location it enters and perform some image 
processing to identify a particular object (e.g., a lost person using a red jacket). For 
this, new image processing code needs to be uploaded onto the UAV and the 
mission requirements must also be updated. The new requirement might be 
formalised as in requirement (\ref{eqn:T-sense}), where $\photofl$ is a fluent turned on 
by the command \photo and turned off on arriving to any new location (\arrivedN{i}).
\begin{equation} \label{eqn:T-sense}
 \forall 0 \leq i, j \leq 5 \cdot \big[i \neq j 
\wedge 
\Gl \big(\arrivedfl{i} \rightarrow (\neg \arrivedfl{j} \W \photofl) \big)\big]
\end{equation}


For \photo to be interpretable by the controller, the label \photo must be bound to 
the code that takes the picture and processes the image. This binding may require 
the system to be in some form of quiescence that can be captured in the transition 
requirement. For instance, $T = \Gl \big(\reconfigure \implies (\stopOld 
\wedge \neg \goingfl) \big)$ together with requirement (\ref{eqn:T-arrived03}).

This transition requirement adds that reconfiguration cannot be done before 
dropping the old mission and it cannot be performed while moving to a location 
(assuming that fluent \goingfl is defined to be turned on with a \go command and 
switched off with 
an \arrived event).
}



In the example above we modelled constraints of the new command \photo in 
temporal logic. However, these can also be introduced with LTS (as in 
Figure~\ref{fig:capabilities}).
%In this case, the initial state of the LTS reeds to be set 
%at reconfiguration time. This can be modelled similarly to \hotSwap,  using the 
%interrupt operator and another state mapping $(E \; \lightning_R^{\reconfigure} E')$.



%\begin{definition}\emph{(Environment Reconfiguration)} \label{def:reconfigure}
%Let $C$ be an LTS and $E$, $E'$ be LTS with states $S_E$ and 
%$S_{E'}$. Let  \reconfigure be an event that is only in the alphabet of $C$. Let $R$ be 
%a total 
%function from $S_E$ to $\powerset{S_{E'}} \setminus \emptyset$. The behaviour 
%resulting from having a controller $C$ trigger the reconfiguration of its environment 
%is defined by $C' \| (E \lightning_R^{\reconfigure} E')$
%\end{definition}
%
%The relation $R$, sets the initial state of $E'$ according to the current state of $E$ 
%at 
%the time of \reconfigure. One possible choice for $R$ is to map all states of $E$ to 
%one fixed 
%initial state of $E'$ modelling fixed initialisation of the environment. 
%Note that we do not require $R$ to be defined for all states of $E$; this provides a 
%way of 
%restricting when $C'$ is allowed to reconfigure. 

%It is important to note that $R$ may introduce non-determinism by mapping one 
%state in $E$ to 
%several states in $E'$. This is an important feature that is required to model 
%scenarios such as 
%the RailCab case study from ~\cite{Ghezzi2012}. The RailCab, described in more 
%detail in the 
%Validation Section, discusses a scenario in which the railway infrastructure has been 
%enhanced with 
%additional sensors. The current RailCab system receives messages for various 
%milestones as it 
%approaches a crossing (\emph{endOfTrunkSection}, \emph{lastBrake} and then 
%\emph{noReturn}. Its 
%goals are stated in terms of actions it must perform between different milestones. 
%The new system 
%is to receive an additional message (\emph{approachingCrossing}) for a newly 
%introduced sensor that 
%sits halfway between the \emph{endOfTrunkSection} and the \emph{lastBrake} 
%milestones. 
%Figure~\ref{fig:reconfigure} (ignoring dashed transitions) depicts a portion of the 
%environment 
%model for the current (top) and new (bottom) RailCab specifications. 
%
%Non-determinism is introduced in the mapping from $E$ to $E'$ in the RailCab 
%setting between the 
%state in the current environment that models that the RailCab is between 
%\emph{endOfTrunkSection} 
%and \emph{lastBrake} and the two states in the new environment model that 
%describe the fact that 
%the RailCab is between \emph{endOfTrunkSection} and \emph{lastBrake}. Because 
%the event 
%\emph{approachingCrossing} is not monitored in $E$, the correct way to model the 
%transition to $E'$ 
%is to make no assumption on whether \emph{approachingCrossing} has occurred.
%Indeed, Figure~\ref{fig:reconfigure} describes the combination of both 
%environments via an interrupt action $\reconfigure$ and a relation ($R$ $=$ 
%$\{(0,0),$ $(1,1),$ $(1,2),$ $(2,3),$ $(3,4),$ $(4,5)\}$).
%
%%i.e., $(E \; \lightning_R^{\reconfigure} \; E')$ 
%
%\begin{figure}
%    \centering
%   \includegraphics[scale=.37]{src/img/reconfigureACM.pdf}
%    \caption{Environment assumptions $(E \lig{R}{reconfigure} E')$ for the Railcab 
%dynamic 
%    update case 
%    study~\cite{Ghezzi2012}. Dotted reconfigure transitions indicate how old 
%assumptions are mapped 
%    into new ones according to relation $R$. }
%    \label{fig:reconfigure}
%  \end{figure}

%This scenario can be specify in $R$ defining, for a pair of states 
%in $E$ and $E'$, to a fresh event representing the unsensed event.

%Thus, there's a need to specify that from some states of $E$, while reconfiguring, some particular 
%event was not tracked before but occur.
%For this reason, we let the user to augmentate the reconfigure process by adding a special fresh 
%event representing this untracked action (see Definition~\ref{def:lightning}).
%We want to add these fresh events into initiating or terminating actions of some fluents.
%To do so, we are going to change de image of the definition function to change these sets if 
%necessary.

%
%
%On a methodological note, as with \hotSwap, the alphabet of $(E 
%\lightning_R^{\reconfigure} E')$ is 
%the union of the alphabets of $E$ and $E'$. This entails that events in the 
%communicating alphabet 
%of $E$ and not in that of $E'$ (resp. in $E'$ and not in $E$) are restricted from 
%occurring after 
%(resp. before) $reconfigure$. 

%\subsection{Correctness Criteria for Dynamic Controller Update}

The problem of computing a controller that can be hot-swapped into a 
running 
system while satisfying transition and reconfiguration requirements no matter has been 
studied and addressed by many 
(e.g.,~\cite{Ghezzi2012,MAPEKTemplates,Baresi:2010:DBD:1882362.1882367}), we 
use the fully 
automated approach described in~\cite{Nahabedian-TSE} 
which is restricted to safety missions but can be trivially extended to \gr missions. 

%
%In~\cite{Nahabedian-TSE} we present an algorithm for solving the problem of updating a 
%controller to satisfy a new mission while satisfying transition and reconfiguration 
%requirements. The formulation in~\cite{Nahabedian-TSE} is restricted to safety missions, 
%but it can  be extended to \gr missions. The MTSA tool in~\cite{MTSAweb} supports the 
%update of controllers for \gr missions. The algorithm, given the current controller $C$, 
%computes a controller $C_u$  that is bisimilar to $(C \; \lightning_H^{\hotSwap} \; 
%C')$ for some $H$ and $C'$. Obtaining $H$ and $C'$ is straightforward: $C'$ is the 
%portion of $C_u$ that appears after $\hotSwap$, while $H$ maps states in $C$ to 
%bisimilar states in $C_u$ up to $\hotSwap$.  

%
%To adapt a system $C\|E$ at runtime one must produce a new controller $C'$, a 
%new 
%environment $E'$ and mappings $H$ and $R$ that describe how to set the initial 
%states of $C'$ and $E'$ respectively. 
%
%
%\begin{definition}\emph{(Dynamic Controller Update)} \label{def:adaptation}
%Let $C$, $C'$, $E$, $E'$ be LTS with states and alphabets $S_i$ and $A_i$ and $i \in 
%\{C, C', E, E'\}$. Assume that $\reconfigure \not\in A_C \ cup A_E \cup A_{E'}$ and 
%$\hotSwap \not\in A_S \cup A_{S'} \cup A_E \cup A_{E'}$.  Let $R$ be a total 
%function from $S_E$ to $\powerset{S_{E'}} \setminus \emptyset$, and  $H$ be a 
%total 
%function from $S_C$ to $\powerset{S_{C'}} \setminus \emptyset$. The behaviour of 
%updating dynamically system $C\|E$
%is defined by $(C 
%\lightning_H^{\hotSwap} C') \|$
% $(E $ $\lightning_R^{\reconfigure}$ $ E')$
%\end{definition}


%
% We now formalise what it means for an dynamic controller update to be correct. In 
%particular, what should the behaviour of a system be when a controller $C$ that is 
%guaranteeing a specification (in the form of current
%environment assumptions $E$, requirements $\Gl G$ with $G$ a propositional LTL 
%formula, $d$ a 
%fluent definition, and controllable actions $A$) is replaced with a new 
%controller that should satisfy a new specification (similarly, in the form 
%$E'$, $\Gl G'$, $d'$ and $A'$) under a transition requirement $T$?
%
%As an input to the correctness criteria, we require a specification of how the state 
%of $C'$ is to be set based on the state of $C$, (i.e. the relation $H$) and also how 
%the state of the 
%reconfigured environment $E'$ is influenced by the state of $E$ (i.e. the relation 
%$R$). 
%
%
%We use the following term to model the behavior of updating $C$ with $C'$ such 
%that the latter can 
%change its environment $E$ with $E'$ via \reconfigure: 
%$(C \lightning_H^{\hotSwap} C')$ $\|$ $(E \lightning_R^{\reconfigure} E')$. 
%$\stopOld$, $\startNew$ and $\reconfigure$ should only be in the alphabet of $C'$ 
%thus stating 
%that it is the new controller that will signal when the old specification is dropped, 
%from when the 
%new one is guaranteed and when the environment is to be reconfigured. 
%As explained previously in this section, $\hotSwap$ should not be in the alphabet 
%of $C$, $C'$, 
%$E$, nor $E'$. 
%$H$ should be defined for each state of $C$. 
%Also, $C \lig{H}{\hotSwap} C'$ should be legal for $E \lig{R}{\reconfigure} 
%E'$ with respect to $(A_u,\unc{A_u})$ where $A_u$ $=$  $A \cup A' \cup 
%\{\stopOld, 
%\startNew, \reconfigure\}$ is the set of controllable actions for update, and, 
%$\unc{A_u}$ $=$ 
%$\unc{A} \cup \unc{A}'$ is the set of uncontrollable actions for update.
%In other words, $C$ and $C'$ never block monitored events 
%($\ell \in \unc{A_u}$) neither do controllable events that $E$ and $E'$ prohibit.
%In addition, note that \hotSwap is an internal action of $C \lig{H}{\hotSwap} C'$ and 
%we do not 
%restrict the execution of this action (i.e. \hotSwap $\notin A_u \cup \unc{A_u}  $).
%


%In the following, we define the FLTL formula that models the expected behaviour of 
%system $(C 
%\lightning_H^{\hotSwap} C') \|$
% $(E $ $\lightning_R^{\reconfigure}$ $ E')$: 
%
%To reason about the correctness of an dynamic controller update we must specify 
%the 
%intended behaviour of the system before, during and after the update. We assume 
%$G$ and $G'$ to be specifications of the system before and after the update, while 
%$T$ to be a specification of the expected behaviour during the transition between 
%$G$ and $G'$. To facilitate specification of $T$ we use two additional events: 
%\stopOld, \startNew. We  require \stopOld to occur when $G$ is no longer 
%guaranteed to hold, and \startNew to occur when $G'$ can be guaranteed to hold.    
%
%\begin{definition} \label{def:Goal} \emph{(Goal for Dynamic Controller Update)}
%Let $G$ and $G'$ FLTL formulas describing the requirements for a system before 
%and 
%after it is updated. These goals do not include \stopOld, \startNew, \reconfigure, 
%nor 
%\hotSwap. 
%Let $T$ be an FLTL formula modelling the transition requirement that may refer to 
%\stopOld, \startNew, and \reconfigure, but not to \hotSwap.
%We define $G_u$, the goal for a dynamic controller update as the conjunction of the 
%following FLTL 
%formulae:
%
%\begin{compactenum}
%\item $G \; \mathbf{W} \; \stopOld$
%\item $T$
%\item $\Gl (\startNew \implies G')$
%\item $\Gl (\hotSwap \implies (\F \stopOld \;\; \wedge $
%
%\noindent $\qquad\qquad\qquad\qquad \F \reconfigure \wedge \F 
%\startNew))$
%\end{compactenum} 
%\end{definition}
%


%The first formula requires that the old goal $G$ holds until the controller signals 
%\stopOld. 
%Recall that if the moment in which the old goal is dropped needs to be restricted, 
%this must be specified in the transition requirement $T$.
%% as exemplified in the previous subsection. 
%The second formula states that the transition requirement $T$ must hold. 
%It is expected to predicate over
%\stopOld and \startNew as it must constrain these from occurring based on what is 
%considered a safe 
%update state by the user. 


%(as the $T$ for the production cell discussed in 
%Section~\ref{sec:motivation} that constrains \stopOld to happen before \startNew). 
%A more structured approach such as requiring $T$ to hold only between the two events (i.e., $\G \emph{inTransition} \Rightarrow T$ with $\emph{inTransition} = \langle \{\stopOld\},$ $\{\startNew\}, \bot \rangle$) is too restrictive as the transition requirements may need to refer to situations that happened before the old specification was dropped (e.g., a photograph taken before \stopOld that was not processed before \stopOld) or after \startNew (e.g, do not start new specification until all unprocessed photographs are processed). 
%In addition, the third formula simply requires the new specification to hold from the 
%point in 
%which the controller signals \startNew. 
%This will force the controller to only produce this signal only when it can ensure 
%$G'$. 
%The last formula requires the controller, once  \hotSwap occurs, to progress 
%towards the occurrence
%of events \stopOld, \startNew and \reconfigure.

%
%The correcness relation between a dynamic controller update the update goal is 
%defined as follows 
%
%\begin{definition} \label{def:Correctness} \emph{(Correctness Criteria for Dynamic 
%Controller Update)}
%Given a system in where the controller will be updated $\mathcal{S} = (C 
%\lightning_H^{\hotSwap} C') \| (E \lightning_R^{\reconfigure} E')$, an update goal 
%$G_u$, $A_u = A_C \cup A_{C'} \cup \{\stopOld, \startNew y \reconfigure\}$ and 
%$\unc{A_u} 
%= \unc{A_C} \cup \unc{A_{C'}} \cup \{\hotSwap\} $ 
%where $A_C$ ($A_{C'}$) and $\unc{A_C}$ ($\unc{A_{C'}}$) are the set of controlled 
%and 
% uncontrolled actions of C (C').
%. We say that $\mathcal{S}$ is a correct DCU with respect to 
%$G_u$, $A_u$ and $\unc{A_u}$ 
%if all the 
%following hold:
%\begin{enumerate}[label = {\small(\arabic*)}, leftmargin=0.75cm]
%\item  $\mathcal{S} \modelsF{d_u} G_u$.
%\item $\mathcal{S}$ is 
%deadlock-free.
%\item  Every state of $C$ is mapped by $H$ to at least one state in $C'$. 
%\item  $(C \lightning_H^{\hotSwap} C')$ is a legal LTS for $(E 
%\lightning_R^{\reconfigure} E')$ 
%with respect $(A_u,\unc{A_u})$.
%\end{enumerate} 
%
%\end{definition}


%
%\begin{definition} \label{def:Correctness} \emph{(Correctness Criteria for Dynamic 
%Controller Update)}
%Let $\mathcal{P}$ be a tuple $(\mathcal{E},$ $C,$ $\mathcal{E'},$ $C',$ $T,$ $H,$ 
%$R,$ $d_u)$ 
%where, $C$ and $C'$ are LTS that model respectively the current controller and the 
%new controller 
%such that the communicating alphabet of $C$ does not contain \stopOld, 
%\startNew, \reconfigure, nor 
%\hotSwap, and the communicating alphabet of $C'$ contains \stopOld, \startNew, 
%and \reconfigure but 
%not \hotSwap;
%$\mathcal{E}$ $=$ $(E,\Gl G,d,A,\unc{A})$ and $\mathcal{E'}$ $=$ $(E',\Gl 
%G',d',A',\unc{A'})$ are, respectively, the 
%old and the new specification of systems for a dynamic controller update, where 
%$G$ and $G'$ 
%are propositional FLTL formulae that neither refer to \stopOld, \startNew, 
%\reconfigure, nor 
%\hotSwap;
%$d_u$ is a fluent definition extension of $d$ and $d'$ as defined 
%in Definition~\ref{def:fluentDefinitionExtension}; 
%$T$ is a FLTL formula modelling the transition requirement, which may refer to 
%\stopOld, \startNew, 
%and \reconfigure, but not to \hotSwap;
%$H$ and $R$ are relations defining how $C$ and $E$ are interrupt to be replaced for 
%$C'$ 
%and $E'$ respectively;
%Let $G_u$ be defined as in Definition~\ref{def:Goal};
%
%We say that $\mathcal{P}$ is a correct DCU if all the following hold:
%\begin{enumerate}[label = {\small(\arabic*)}, leftmargin=0.75cm]
%\item  $(C \lightning_H^{\hotSwap} C') \| (E \lightning_R^{\reconfigure} E') 
%\modelsF{d_u} G_u$.
%\item $(C \lightning_H^{\hotSwap} C') \| (E \lightning_R^{\reconfigure} E')$ is 
%deadlock-free.
%\item  Every state of $C$ is mapped by $H$. 
%\item  $(C \lightning_H^{\hotSwap} C')$ is a legal LTS for $(E 
%\lightning_R^{\reconfigure} E')$ 
%with respect $(A_u,\unc{A_u})$.
%\end{enumerate} 
%
%\end{definition}

%
%The previous goal for the DCU problem must be evaluated with the fluent definition 
%extension of 
%$d$ and $d'$ (Definition~\ref{def:fluentDefinitionExtension}). We will call it $d_u$.
%Note that the union of $d$ and $d'$ guarantees that the interpretation of $G$ and 
%$G'$ does not 
%change over $E$ and $E'$ respectively.

%For the informal requirements for dynamic controller update discussed in 
%Section~\ref{sec:motivation}, rules \2
%through \5 are captured in rules 1 through 4 of Definition~\ref{def:Goal}. Rule \1 is 
%captured by the fact that \hotSwap is not part of the alphabet of $C$, $C'$, $E$ and 
%$E'$, and $H$ 
%is defined for every rechable state in $C$. 
%Thus, in the term $(C
%\lightning_H^{\hotSwap} C') \| (E \lightning_R^{\reconfigure} E')$, \hotSwap is 
%never constrained 
%from occurring once.


%\subsection{DCU Synthesis Problem}
%Rather than checking if an update is correct, it is desirable to automatically 
%synthesis 
%a controller that performs a correct update from the update goal. 
%
%\begin{definition} \label{def:Synthesis} \emph{(DCU Synthesis Problem)}
%Let $C$ be a controller that guarantees $G$ in an environment $E$ while controlling 
%actions $A$ and monitoring actions $\unc{A}$ (i.e., it is a solution to the control 
%problem $(E, G,\comments{d,}A,\unc{A})$ ). Let $G'$ be the goal to be achieved by 
%the new controller with environment $E'$ controlling actions $A'$ and monitoring 
%actions $\unc{A'}$, and $R \subseteq (S_E \times S_{E'})$ be a 
%relation that models the relation between the old and new environment. Let $G_u$ 
%be 
%the update goal built using $G$ and $G'$. 

%and $d_u$ be a fluent definition extension of $d$ and $d'$.
%
%A solution for the DCU Synthesis Problem is a pair $(C', H)$ such that $C 
%\lightning_H^{\hotSwap} C') \| (E \lightning_R^{\reconfigure} E')$ is a correct 
%dynamic update with respect to $G_u$, $A_u \cup A_u'$ and $\unc{A_u} \cup 
%\unc{A_u'}$ .
%\end{definition}
%
%
%The DCU synthesis problem, when $G$, $G'$ and $T$ are restricted to safety 
%properties, can be solved using traditional controller synthesis 
%algorithm that supports safety and reachability goals (the reachability is required to 
%ensure clause 4 of Definition~\ref{def:Goal}). The key element in mapping the DCU 
%synthesis 
%into a controller synthesis problem is building an appropriate  environment $E_u$ 
%for the 
%control $(E_u, G_u,\comments{d,}A,\unc{A})$. 
%
%\begin{definition} \label{def:EnvironmentU} \emph{(Environment For Update)}
%Given a DCU synthesis problem with $C$, $E$, $E'$, $R$, $G$, $G'$ 
%and $T$. Let $A$ and $\unc{A}$ be the set of controlled and monitored 
%events of $C$. 
%
%The \emph{Environment for the DCU Synthesis Problem} is an LTS defined $E_u$ 
%$\triangleq$ 
%$([E\|C]_f \lightning_I^{\hotSwap}  E \lightning_R^{\reconfigure} E') \|  O$ where 
%$I$ is a 
%partial 
%function such that $((e,c), e) \in I$ 
%iff $(e,c) \in S_{E\|C}$, 
%$O$ is the LTS depicted in figure~\ref{fig:observers} with alphabet $\{\hotSwap, 
%\stopOld, 
%\startNew\}$, and
%$f$ is the function that relabels all events $\ell \in A$ to fresh events 
%$\overline{\ell} \notin 
%A$. 
%\end{definition}
%
%
%The following theorem is a generalization of that of~\cite{update} where it is limited 
%to $G$, $G'$ and $T$ being safety properties. 
%
%\begin{theorem} \label{def:solution} \emph{(Solution to the DCU Synthesis 
%Problem)}
%Given a DCU synthesis problem with $C$, $E$, $E'$, $R$ and goals $G$, $G'$ 
%and $T$,
%\begin{itemize}
%\item if there is a solution $C'$ to the control problem $(E_u, 
%G_u,\comments{d,}A,\unc{A})$ then a mapping $H$ can be built from the states of 
%$C$ to those of $C'$ such that $(C \lightning_H^{\hotSwap} C') \| (E 
%\lightning_R^{\reconfigure} E')$ is a correct 
%dynamic update with respect to $G_u$, $A$, and $\unc{A}$.
%
%\item  if there is a controller $C'$ and a mapping $H$ such that  $(C 
%\lightning_H^{\hotSwap} C') $ $\|$  $(E \lightning_R^{\reconfigure} E')$ is a correct 
%dynamic update with respect to $G_u$, $A$, and $\unc{A}$, then there is a solution 
%to the control 
%problem $(E_u, G_u,\comments{d,}A,\unc{A})$.
%\end{itemize}
%
%\end{theorem}
%
%\begin{remark} \label{def:Safetysolution} \emph{(Implementation of the DCU 
%Safety Synthesis 
%Problem)}
%If $G$, $G'$ and $T$ are safety goals, the $G_u$ is the conjunction of a safety 
%property and a reachability propoerty. Thus, a  synthesis algorithm that is linear to 
%the size of $E_u$ can be applied to correctly and completely solve the DCU 
%synthesis 
%problem. In~\cite{update}, such an algorithm is presented. 
%\end{remark}
%
%


%
%
%
%
%Note that the DCU problem may or may not have a solution.
%The existence of a solution indicates that the controller resulting from solving the 
%problem will 
%guarantee $G_u$. 
%The validity of the assumptions $E$ and $E'$ is the engineer's responsibility.
%In general, the non-existence of a solution arises due to too stringent 
%combinations of 
%specifications ($E$, $G$, $E'$, $G'$ and $T$) and lack of controllability by the 
%controller of 
%environment events. 
%A controller that is a solution to the DCU problem will, informally, have the structure depicted in
%Figure~\ref{fig:controller}. 
%First it will maintain $G$ except that it will accept at any point the uncontrollable event 
%\hotSwap. 
%Then it will behave as a controller that is attempting to achieve \stopOld and \startNew while 
%satisfying $T$. 
%Finally, once \startNew and \stopOld have occurred it will behave as a controller that satisfies 
%$G'$.

  
%The non-existence of a solution to the control problem can arise in three different 
%situations. 
%The first is that the new goal under the new environment assumptions are not 
%achievable by a 
%controller. 
%For instance, there is no way to handle products to satisfy the new production 
%process 
%specification. 
%In this case, the new specification must be corrected.  
%
%The second reason is that it is not possible to guarantee that the transition will 
%satisfy $T$. 
%For instance, requiring in $T$ that the new specification be put in place immediately 
%is 
%impossible 
%as products that have been partially processed may have been done so in a way that 
%is inconsistent 
%with the new specification. 
%In this case, the transition requirement needs to be weakened. 
%
%Finally, non-existence of a solution may be due to the impossibility of 
%guaranteeing that 
%the 
%update will \emph{eventually} occur (even though it may actually occur). 
%For instance, requiring the production line be emptied before changing cannot be 
%guaranteed by the controller as it does not control the event \emph{in(x)}. 
%In this case the transition requirement needs to be changed to allow updates with a 
%non-empty 
%production line. 
%


==> src/gr1update.tex <==
\section{Dynamic Update of GR1 Controllers} \label{sec:gr1update}

\begin{itemize}
\item Motivate GR1 for UAV missions. Citations to Robotics, Pelliconi and us
\item Explain naif update. If we have an old and new GR1 spec and introduce it 
trivially to Gu, then the result is not encodable in GR1. Explain and introduce a GR1 
update goal.
\item Restate that the correctness criteria and control problem are the same as 
before but where Gu is not required to be safety
\item Explain how to solve the GR update problem. Essentially build Eu, synthesise 
and build H. 
\item Prove that this is a good solution. For this we need to build on two lemmas 
from the TOSEM paper, one for proving correctness of solutions and the other for 
completeness of the algorithm. Correctness relies on the fact that the GR1u implies 
GSafetyu. 
\end{itemize}

\sz{Yo utilizaria como motivacion el ejemplo \goalchange de motivacion. Como ya esta 
indroducida la especificacion de la mision original solo falta mencionar la nueva 
especificacion y contar porque el problema de update no es trivial}




\subsection{Solution to the DCU GR1 Synthesis Problem}


\begin{definition} \label{def:GR1Goal} \emph{(GR1 Goal for Dynamic Controller 
Update)}
Let  $G = G_S \wedge 
G_{gr1}$, $G'= G'_S \wedge G_{gr1}$ and $T$ where $G_S$ and 
$G'_S$ are safety 
goals, $G_S$ and $G'_S$ are GR1 goals, and none \stopOld, \startNew, \reconfigure, 
nor \hotSwap. 
Let $T$ be a safety goal modelling the transition requirement that may refer to 
\stopOld, \startNew, and \reconfigure, but not to \hotSwap.
We define $G^{gr1}_u$, the goal for a dynamic controller update as the conjunction 
of the 
following FLTL 
formulae:

\begin{compactenum}
\item $G_S \; \mathbf{W} \; \stopOld$
\item $T$
\item $\Gl (\startNew \implies G_S')$
\item $\Gl (\hotSwap \implies (\F \stopOld \; \wedge \F \reconfigure \; \wedge $

\noindent $\qquad\qquad\qquad\qquad \F 
\startNew))$
\item $\Gl (\startNew \implies G'_{gr1})$
\end{compactenum} 
\end{definition}



\begin{theorem} \label{def:solution} \emph{(Solution to the 
DCU GR1 Synthesis 
Problem)}
Given a DCU synthesis problem with $C$, $E$, $E'$, $R$ and 
goals $G = G_S \wedge 
G_{gr1}$, $G'= G'_S \wedge G_{gr1}$ and $T$ where $G_S$, 
$G'_S$ and $T$ are safety 
goals and $G_S$ and $G'_S$ are GR1 goals. Let $E_u$ be an 
LTS built as in Definition~\ref{def:EnvironmentU}, $G_u^{gr1}$ according to 
Definition~\ref{def:GR1Goal} and $G_u$ according to Definition~\ref{def:Goal} then:

\begin{itemize}
\item if there is a solution $C'$ to the control problem $(E_u, 
G_u^{gr1},\comments{d,}A,\unc{A})$ then a mapping $H$ can be 
built from the states of 
$C$ to those of $C'$ such that $(C \lightning_H^{\hotSwap} 
C') \| (E 
\lightning_R^{\reconfigure} E')$ is a correct 
dynamic update with respect to $G_u$, $A$, and $\unc{A}$.

\item  if there is a controller $C'$ and a mapping $H$ such 
that  $(C 
\lightning_H^{\hotSwap} C') $ $\|$  $(E 
\lightning_R^{\reconfigure} E')$ is a correct 
dynamic update with respect to $G_u$, $A$, and $\unc{A}$, 
then there is a solution 
to the control 
problem $(E_u, G_u^{gr1},\comments{d,}A,\unc{A})$.
\end{itemize}

\end{theorem}

\begin{proof}
For the first item of the theorem we first define  $G_u^{safe}$, as the conjunction of:

\begin{compactenum}
\item $G_S \; \mathbf{W} \; \stopOld$
\item $T$
\item $\Gl (\startNew \implies G_S')$
\item $\Gl (\hotSwap \implies (\F \stopOld \; \wedge \F \reconfigure \; \wedge $

\noindent $\qquad\qquad\qquad\qquad \F \startNew))$

\end{compactenum} 

Note that $G_u^{safe} \wedge 
\Gl (\startNew \implies G'_{gr1}) \wedge (G_{gr1} \W \stopOld)$ if and only if $G_u$.

Assume that there is a solution $C'$ to the control problem $(E_u, 
G_u^{gr1},\comments{d,}A,\unc{A})$.  As  $G_u^{gr1}$ implies $G_u^{safe}$  then 
$C'$ is a 
solution to  $(E_u, 
G_u^{safe},\comments{d,}A,\unc{A})$. Then (Theorem~\ref{def:solution}) a mapping 
$H$ can be 
built from the states of 
$C$ to those of $C'$ such that $(C \lightning_H^{\hotSwap} 
C') \| (E 
\lightning_R^{\reconfigure} E')$ is a correct 
dynamic update with respect to $G_u^{safe}$, $A$, and $\unc{A}$. 

To prove that it is 
also correct with respect to $G_u$, $A$, and $\unc{A}$ what remains is to show that 
$(C 
\lightning_H^{\hotSwap} 
C') \| (E 
\lightning_R^{\reconfigure} E') \modelsF{d_u} (\Gl (\startNew \implies 
G'_{gr1}))  \wedge 
 (G_{gr1} \W \stopOld)$. 
 
 Satisfaction of $\Gl (\startNew \implies  G'_{gr1}) $ follows from the fact that $C'$ is 
 a solution for $(E_u, 
 G_u^{gr1},\comments{d,}A,\unc{A})$.
 
 Satisfaction of   $G_{gr1} \W \stopOld$ follows from the fact that $C$ 
 is a solution to the control problem $(E, G_S \wedge G_{gr1})$. Plus the fact that if 
 $\hotSwap$ never occurs then $(C 
 \lightning_H^{\hotSwap} 
 C') \| (E 
 \lightning_R^{\reconfigure} E')$ behaves like $C\|E$. While if $\hotSwap$ does 
 occur, then $\stopOld$ is guaranteed, and $G_{gr1} \W \stopOld$ is trivially true as 
 now liveness goal need be guaranteed as an infinite number of assumptions cannot 
 occur before $\stopOld$.


The second item of the theorem can be proved as follows: If 
$(C 
\lightning_H^{\hotSwap} C') $ $\|$  $(E 
\lightning_R^{\reconfigure} E')$ is a correct 
dynamic update with respect to $G_u$, $A$, and $\unc{A}$, then by 
Theorem~\ref{def:solution} there is a is a solution 
to the control 
problem $(E_u, G_u,\comments{d,}A,\unc{A})$. As  $G_u$ implies $G_u^{gr1}$ then 
the solution is also a solution to  $(E_u, G_u^{gr1},\comments{d,}A,\unc{A})$.

\end{proof}


==> src/lts/capabilities.tex <==
\TinyPicture
%  \ShowFrame \ShowGrid
\VCDraw{ %
    \begin{VCPicture}{(-2.4,-3.8)(4.7,3.9)}
%    \SetEdgeLabelScale{1.2}
    \State[0]{(0,2)}{0}
    \State[1]{(0.5,0)}{1}
    \State[2]{(0,-2)}{2}
    \State[3]{(3,-2.7)}{3}
    \State[4]{(-0.5,0)}{4}
    \Initial[w]{0}


    \ChgEdgeLineStyle{dashed} %\EdgeLineDouble 
        \ArcL{0}{1}{\takeOff}
        \ArcL{2}{4}{\land}
        \ArcL[.7]{2}{3}{\set{\goN{i} : 0 \leq i \leq 5}}
    \RstEdgeLineStyle %\EdgeLineSimple 


%\SetArcAngle{45} %% int (degree)
%\SetLArcAngle{45} %% int (degree)
%\SetArcCurvature{0} %% float
%\SetArcOffset{1pt} %% length

    \ArcL[.2]{1}{2}{\takeOffEnd}
    \ArcL{4}{0}{\landEnd}
    \ArcL[.7]{3}{2}{\set{\arrivedN{i} : 0 \leq i \leq 5}}
         
        
    \end{VCPicture}
}% \MediumPicture 


%
%\TinyPicture
% %\ShowFrame \ShowGrid
%\VCDraw{ %
%    \begin{VCPicture}{(0,-1)(5,2)}
%%    \SetEdgeLabelScale{1.2}
%    \State[0]{(0,0)}{0}
%    \State[1]{(4.2,0)}{1}
%    \Initial[n]{0}
%
%    \ChgEdgeLineStyle{dashed} %\EdgeLineDouble 
%    \EdgeR[.5]{0}{1}{\inP}
%    \RstEdgeLineStyle %\EdgeLineSimple 
%
%  %  \LArcL{1}{0}{\yesNemoCurrent}
%   % \LArcR{1}{0}{\noNemoCurrent}
%    \LArcR[.6]{1}{0}{\yinP}
%    \LArcL{1}{0}{\ninP}
%    \end{VCPicture}
%}% \MediumPicture 

==> src/lts/composition.tex <==
\TinyPicture
%  \ShowFrame \ShowGrid
\VCDraw{ %
    \begin{VCPicture}{(-3.3,-3.8)(11,4.2)}
%    \SetEdgeLabelScale{1.2}
    \State[0]{(-1,3.5)}{0}
    \State[1]{(-1,1.75)}{1}
    \State[2]{(0,0)}{2}
    \State[3]{(-0.05,2)}{3}

    \State[4]{(2,0.5)}{4}
    \State[5]{(4,0)}{5}
    \State[6]{(6,0.5)}{6}
    \State[7]{(8,0)}{7}
    \State[8]{(2,-0.5)}{8}
    \State[9]{(6,-0.5)}{9}
    
   \HideState
    \State[A]{(0,-4)}{A}
    \State[B]{(2,-3.5)}{B}
    \State[C]{(4,-4)}{C}
    \State[D]{(6,-3.5)}{D}
    \State[E]{(8,-4)}{E}
    \State[F]{(2,-4.5)}{F}
    \State[G]{(6,-4.5)}{G}
    \ShowState
    
    \State[10]{(-0.5,-2)}{10}
    \State[11]{(0.5,-2)}{11}
    \State[12]{(3.5,-2)}{12}
    \State[13]{(4.5,-2)}{13}
    \State[14]{(7.5,-2)}{14}
    \State[15]{(8.5,-2)}{15}
   
    \State[16]{(4,3.5)}{16}
    \State[17]{(3.5,2)}{17}
    \State[18]{(4.5,2)}{18}
   
    \State[19]{(9,3.5)}{19}
    \State[20]{(8.05,2)}{20}
    \State[21]{(9,1.75)}{21}
    
    \Initial[w]{0}


    \ChgEdgeLineStyle{dashed} %\EdgeLineDouble 
        \ArcL[.8]{2}{4}{\goN{1}}
        \ArcL[.8]{5}{6}{\goN{2}}
        \ArcL[.7]{7}{9}{\goN{1}}
        \ArcL[.7]{5}{8}{\goN{0}}
        
        \ArcR{0}{1}{\takeOff}
        \ArcR[.9]{2}{3}{\land}
        
        \ArcR{16}{17}{\takeOff}
        \ArcR[.9]{5}{18}{\land}
        \ArcR{19}{20}{\takeOff}
        \ArcR[.9]{7}{21}{\land}
        
%         \ArcL[.7]{A}{B}{\goN{4}}
%         \ArcL[.7]{C}{D}{\goN{5}}
%         \ArcL{E}{G}{\goN{4}}
%         \ArcL{C}{F}{\goN{3}}
        
        \ArcR[.9]{A}{11}{\goN{0}}
        \ArcR[.9]{2}{10}{\goN{3}}
        \ArcR[.9]{C}{13}{\goN{1}}
        \ArcR[.9]{5}{12}{\goN{4}}
        \ArcR[.9]{E}{15}{\goN{2}}
        \ArcR[.9]{7}{14}{\goN{5}}
    \RstEdgeLineStyle %\EdgeLineSimple 


%\SetArcAngle{45} %% int (degree)
%\SetLArcAngle{45} %% int (degree)
%\SetArcCurvature{0} %% float
%\SetArcOffset{1pt} %% length

    \ArcL[.2]{4}{5}{\arrivedN{1}}
    \ArcL{6}{7}{\arrivedN{2}}
    \ArcL{9}{5}{\arrivedN{1}}
    \ArcL{8}{2}{\arrivedN{0}}
    
    \ArcR{1}{2}{\takeOffEnd}
    \ArcR{3}{0}{\landEnd}
    
    \ArcR[.1]{17}{5}{\takeOffEnd}
    \ArcR{18}{16}{\landEnd}
    \ArcR[.1]{20}{7}{\takeOffEnd}
    \ArcR{21}{19}{\landEnd}
    
%     \ArcL{B}{C}{\arrivedN{4}}
%     \ArcL{D}{E}{\arrivedN{5}}
%     \ArcL{G}{C}{\arrivedN{4}}
%     \ArcL{F}{A}{\arrivedN{3}}
   
    \ArcR[.1]{11}{2}{\arrivedN{0}}
    \ArcR[.1]{10}{A}{\arrivedN{3}}
    \ArcR[.1]{13}{5}{\arrivedN{1}}
    \ArcR[.1]{12}{C}{\arrivedN{4}}
    \ArcR[.1]{15}{7}{\arrivedN{2}}
    \ArcR[.1]{14}{E}{\arrivedN{5}}
      
      
     \fontsize{30pt}{30pt}\selectfont
     \rput[t]{0}(0,-4){$...$}
     \rput[t]{0}(4,-4){$...$}
     \rput[t]{0}(8,-4){$...$}
    \end{VCPicture}
}% \MediumPicture 
 

==> src/lts/controller.tex <==
\TinyPicture
%   \ShowFrame \ShowGrid
\VCDraw{ %
    \begin{VCPicture}{(-1,-1.4)(19,1.8)}
%    \SetEdgeLabelScale{1.2}
    \State[0]{(1,-0.8)}{0}
    \State[1]{(1,0.8)}{1}
    \State[2]{(4,0.8)}{2}
    \State[3]{(6,0.8)}{3}
    \State[4]{(8,0.8)}{4}
    \State[5]{(10,0.8)}{5}
    \State[6]{(12,0.8)}{6}
    \State[7]{(14,0.8)}{7}
    \State[8]{(17,0.8)}{8}
    \State[9]{(17,-0.8)}{9}
    \State[10]{(14,-0.8)}{10}
    \State[11]{(12,-0.8)}{11}
    \State[12]{(10,-0.8)}{12}
    \State[13]{(8,-0.8)}{13}
    \State[14]{(6,-0.8)}{14}
    \State[15]{(4,-0.8)}{15}
    \Initial[w]{0}


    \ChgEdgeLineStyle{dashed} %\EdgeLineDouble 
        \ArcL{0}{1}{\takeOff}
        \ArcL{2}{3}{\goN{1}}
        \ArcL{14}{3}{\goN{1}}
        \ArcL{4}{5}{\goN{0}}
        \ArcL{6}{11}{\goN{1}}
        \ArcL{6}{7}{\land}
        \ArcL{8}{9}{\takeOff}
        \ArcL{10}{11}{\goN{1}}
        \ArcL{12}{13}{\goN{2}}
        
        \ArcL{14}{15}{\land}
    \RstEdgeLineStyle %\EdgeLineSimple 


%\SetArcAngle{45} %% int (degree)
%\SetLArcAngle{45} %% int (degree)
%\SetArcCurvature{0} %% float
%\SetArcOffset{1pt} %% length

    \ArcL{1}{2}{\takeOffEnd}
    \ArcL{3}{4}{\arrivedN{1}}
    \ArcL{5}{6}{\arrivedN{0}}
    \ArcL{7}{8}{\landEnd}
    \ArcL{9}{10}{\takeOffEnd}
    \ArcL{11}{12}{\arrivedN{1}}
    \ArcL{13}{14}{\arrivedN{2}}
    
    \ArcL{15}{0}{\landEnd}
         
        
    \end{VCPicture}
}% \MediumPicture 


%
%\TinyPicture
% %\ShowFrame \ShowGrid
%\VCDraw{ %
%    \begin{VCPicture}{(0,-1)(5,2)}
%%    \SetEdgeLabelScale{1.2}
%    \State[0]{(0,0)}{0}
%    \State[1]{(4.2,0)}{1}
%    \Initial[n]{0}
%
%    \ChgEdgeLineStyle{dashed} %\EdgeLineDouble 
%    \EdgeR[.5]{0}{1}{\inP}
%    \RstEdgeLineStyle %\EdgeLineSimple 
%
%  %  \LArcL{1}{0}{\yesNemoCurrent}
%   % \LArcR{1}{0}{\noNemoCurrent}
%    \LArcR[.6]{1}{0}{\yinP}
%    \LArcL{1}{0}{\ninP}
%    \end{VCPicture}
%}% \MediumPicture 

==> src/lts/discretization.tex <==
\TinyPicture
%  \ShowFrame \ShowGrid
\VCDraw{ %
    \begin{VCPicture}{(-1.5,-5.3)(9.5,2.4)}
%    \SetEdgeLabelScale{1.2}
    \State[0]{(0,0)}{0}
    \State[1]{(2,0.5)}{1}
    \State[2]{(4,0)}{2}
    \State[3]{(6,0.5)}{3}
    \State[4]{(8,0)}{4}
    \State[5]{(2,-0.5)}{5}
    \State[6]{(6,-0.5)}{6}
    
    \State[7]{(0,-4)}{7}
    \State[8]{(2,-3.5)}{8}
    \State[9]{(4,-4)}{9}
    \State[10]{(6,-3.5)}{10}
    \State[11]{(8,-4)}{11}
    \State[12]{(2,-4.5)}{12}
    \State[13]{(6,-4.5)}{13}
    
    \State[14]{(-0.5,-2)}{14}
    \State[15]{(0.5,-2)}{15}
    \State[16]{(3.5,-2)}{16}
    \State[17]{(4.5,-2)}{17}
    \State[18]{(7.5,-2)}{18}
    \State[19]{(8.5,-2)}{19}
    \Initial[w]{0}


    \ChgEdgeLineStyle{dashed} %\EdgeLineDouble 
        \ArcL{0}{1}{\goN{1}}
        \ArcL{2}{3}{\goN{2}}
        \ArcL[.7]{4}{6}{\goN{1}}
        \ArcL[.7]{2}{5}{\goN{0}}
        
        \ArcL[.7]{7}{8}{\goN{4}}
        \ArcL[.7]{9}{10}{\goN{5}}
        \ArcL{11}{13}{\goN{4}}
        \ArcL{9}{12}{\goN{3}}
        
        \ArcR[.9]{7}{15}{\goN{0}}
        \ArcR[.9]{0}{14}{\goN{3}}
        \ArcR[.9]{9}{17}{\goN{1}}
        \ArcR[.9]{2}{16}{\goN{4}}
        \ArcR[.9]{11}{19}{\goN{2}}
        \ArcR[.9]{4}{18}{\goN{5}}
        
    \RstEdgeLineStyle %\EdgeLineSimple 


%\SetArcAngle{45} %% int (degree)
%\SetLArcAngle{45} %% int (degree)
%\SetArcCurvature{0} %% float
%\SetArcOffset{1pt} %% length

    \ArcL{1}{2}{\arrivedN{1}}
    \ArcL{3}{4}{\arrivedN{2}}
    \ArcL{6}{2}{\arrivedN{1}}
    \ArcL{5}{0}{\arrivedN{0}}
    
    \ArcL{8}{9}{\arrivedN{4}}
    \ArcL{10}{11}{\arrivedN{5}}
    \ArcL{13}{9}{\arrivedN{4}}
    \ArcL{12}{7}{\arrivedN{3}}
   
    \ArcR[.1]{15}{0}{\arrivedN{0}}
    \ArcR[.1]{14}{7}{\arrivedN{3}}
    \ArcR[.1]{17}{2}{\arrivedN{1}}
    \ArcR[.1]{16}{9}{\arrivedN{4}}
    \ArcR[.1]{19}{4}{\arrivedN{2}}
    \ArcR[.1]{18}{11}{\arrivedN{5}}
         
        
    \end{VCPicture}
}% \MediumPicture 
 

==> src/lts/discretizationChange.tex <==
\TinyPicture
%  \ShowFrame \ShowGrid
\VCDraw{ %
    \begin{VCPicture}{(2,-4.8)(17.1,5.1)}
%    \SetEdgeLabelScale{1.2}

   \HideState
    \State[0]{(0,0)}{0}
    \State[1]{(2,0.5)}{1}
    \State[5]{(2,-0.5)}{5}
    \State[7]{(0,-4)}{7}
    \State[8]{(2,-3.5)}{8}
    \State[12]{(2,-4.5)}{12}
    \State[14]{(-0.5,-2)}{14}
    \State[15]{(0.5,-2)}{15}
    \ShowState
    
    
    \State[2]{(4,0)}{2}
    \State[3]{(6,0.5)}{3}
    \State[4]{(8,0)}{4}
    \State[6]{(6,-0.5)}{6}
    
    \State[9]{(4,-4)}{9}
    \State[10]{(6,-3.5)}{10}
    \State[11]{(8,-4)}{11}
    \State[13]{(6,-4.5)}{13}
    
    \State[16]{(3.5,-2)}{16}
    \State[17]{(4.5,-2)}{17}
    \State[18]{(7.5,-2.3)}{18}
    \State[19]{(8.5,-1.7)}{19}
%     \Initial[w]{0}


    
   \HideState
    \State[22]{(16.5,4)}{22}
    \State[29]{(16.5,0)}{29}
    \State[31]{(16.5,-4)}{31}
    \State[36]{(16,2)}{36}
    \State[37]{(17,2)}{37}
    \State[38]{(16,-2)}{38}
    \State[39]{(17,-2)}{39}
    \ShowState

    \State[20]{(12.5,4)}{20}
    \State[21]{(14.5,4.5)}{21}
    \State[25]{(14.5,3.5)}{25}
    \State[27]{(12.5,0)}{27}
    \State[28]{(14.5,0.5)}{28}
    \State[32]{(14.5,-0.5)}{32}
    \State[34]{(12,2)}{34}
    \State[35]{(13,2)}{35}
    
    
    \State[23]{(12,-2.3)}{23}
    \State[24]{(12.5,-4)}{24}
    \State[26]{(13,-1.7)}{26}
    
    \State[30]{(14.5,-3.5)}{30}
    \State[33]{(14.5,-4.5)}{33}
    
    

    \ChgEdgeLineStyle{dashed} %\EdgeLineDouble 
	
        \ArcL{4}{27}{\textbf{\reconfigure}}
        \ArcR[.6]{18}{23}{\textbf{\reconfigure}}
        \ArcR{11}{24}{\textbf{\reconfigure}}
        \ArcL[.4]{19}{26}{\textbf{\reconfigure}}
    
%         \ArcL{0}{1}{\goN{1}}
        \ArcL{2}{3}{\goN{2}}
        \ArcL[.7]{4}{6}{\goN{1}}
        \ArcL[.7]{2}{5}{\goN{0}}
        
%         \ArcL[.7]{7}{8}{\goN{4}}
        \ArcL[.8]{9}{10}{\goN{5}}
        \ArcL{11}{13}{\goN{4}}
        \ArcL{9}{12}{\goN{3}}
        
%         \ArcR[.9]{7}{15}{\goN{0}}
%         \ArcR[.9]{0}{14}{\goN{3}}
        \ArcR[.9]{9}{17}{\goN{1}}
        \ArcR[.9]{2}{16}{\goN{4}}
        \ArcR[.9]{11}{19}{\goN{2}}
        \ArcR[.9]{4}{18}{\goN{5}}
        
        
        \ArcL[.25]{20}{21}{\goN{7}}
        \ArcR[.9]{24}{26}{\goN{2}}
        \ArcL{22}{25}{\goN{6}}
        
        \ArcL[.8]{27}{28}{\goN{8}}
%         \ArcL[.8]{29}{39}{\goN{5}}
        \ArcL{31}{33}{\goN{5}}
        \ArcL{29}{32}{\goN{2}}
        
        \ArcR[.9]{27}{35}{\goN{6}}
        \ArcR[.9]{20}{34}{\goN{2}}
        \ArcR[.9]{27}{23}{\goN{5}}
%         \ArcR[.9]{22}{36}{\goN{4}}
%         \ArcR[.9]{31}{39}{\goN{2}}
        \ArcL[.8]{24}{30}{\goN{9}}
        
    \RstEdgeLineStyle %\EdgeLineSimple 


%\SetArcAngle{45} %% int (degree)
%\SetLArcAngle{45} %% int (degree)
%\SetArcCurvature{0} %% float
%\SetArcOffset{1pt} %% length

    \ArcL{1}{2}{\arrivedN{1}}
    \ArcL{3}{4}{\arrivedN{2}}
    \ArcL{6}{2}{\arrivedN{1}}
%     \ArcL{5}{0}{\arrivedN{0}}
    
    \ArcL{8}{9}{\arrivedN{4}}
    \ArcL{10}{11}{\arrivedN{5}}
    \ArcL{13}{9}{\arrivedN{4}}
%     \ArcL{12}{7}{\arrivedN{3}}
   
%     \ArcR[.1]{15}{0}{\arrivedN{0}}
%     \ArcR[.1]{14}{7}{\arrivedN{3}}
    \ArcR[.1]{17}{2}{\arrivedN{1}}
    \ArcR[.1]{16}{9}{\arrivedN{4}}
    \ArcR[.7]{19}{4}{\arrivedN{2}}
    \ArcR[.05]{18}{11}{\arrivedN{5}}
    
%     ---

    \ArcL{21}{22}{\arrivedN{7}}
    \ArcR[.7]{23}{24}{\arrivedN{5}}
    \ArcR[.05]{26}{27}{\arrivedN{2}}
    \ArcL{25}{20}{\arrivedN{6}}
    
    \ArcL{28}{29}{\arrivedN{8}}
    \ArcL{30}{31}{\arrivedN{9}}
    \ArcL{33}{24}{\arrivedN{5}}
    \ArcL{32}{27}{\arrivedN{2}}
   
    \ArcR[.1]{35}{20}{\arrivedN{6}}
    \ArcR[.1]{34}{27}{\arrivedN{2}}
%     \ArcR[.1]{37}{22}{\arrivedN{1}}
%     \ArcR[.1]{36}{29}{\arrivedN{4}}
%     \ArcR[.7]{39}{24}{\arrivedN{2}}
%     \ArcR[.05]{38}{31}{\arrivedN{5}}
         
        
     \fontsize{30pt}{30pt}\selectfont
     \rput[t]{0}(1.8,0.5){$...$}
     \rput[t]{0}(1.8,-0.5){$...$}
     \rput[t]{0}(1.8,-3.5){$...$}
     \rput[t]{0}(1.8,-4.5){$...$}
     
     \rput[t]{0}(16.7,4){$...$}
     \rput[t]{0}(16.7,0){$...$}
     \rput[t]{0}(16.7,-4){$...$}
     
     \fontsize{20pt}{20pt}\selectfont
     \rput[t]{0}(5,2){\textit{Old Workspace}}
     \rput[t]{0}(9.5,4.6){\textit{New Workspace}}
     
    \end{VCPicture}
}% \MediumPicture 
 

==> src/morph.tex <==
\section{Architecture Overview} \label{sec:morph}


\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{src/img/morphabreviado.eps}


\caption{Architecture Overview}
\label{fig:archoverview}
\end{figure}

%\subsection{Architectural Overview}
Figure~\ref{fig:archoverview} presents an abstract view of the UAV architecture. 
To facilitate traceability, we will use an \morph{alternative 
font}, when referring to elements in the figure.

Users interact with the system via the \morphControlPanel. In the panel they write 
missions 
specifications and provide any new software modules for the UAV. The panel is also used to 
monitor the mission by visualising \morphTelemetry data transmitted by the \morphVehicle. 
The specifications are consumed by the \morphSynthesiser that outputs a discrete 
event 
controller in the form of an LTS to the \morphCtrlManagment layer. The latter 
is 
mainly in charge of performing a safe hot-swap of the controller being run in the 
\morphEnactor  layer with a new controller. 

The \morphEnactor layer runs the controller, sending controlled \morphCommands to and 
receiving monitored \morphEvents from the \morphHybridControl. The 
\morphHybridControl layer is 
in 
charge of converting discrete events and commands into ones that predicate over continuous 
values. For instance, it knows that when it  receives a command \goN{4}, number $4$ 
corresponds to a circular area of \SI{50}{\meter} diameter and centred at 
\SI{48.8566}{\degree}$N$ and \SI{2.3522}{\degree}$E$. Information on discretization 
of the continuous 
regions is received from the \morphControlPanel. The \morphHybridControl layer
also 
generates the intermediate \textit{waypoints} that 
need to be followed to reach that the target area. These waypoints depend on the 
manoeuvrability of the \morphVehicle and are the input to the various 
\morphFeedback that compute low level actuator commands such as thrust and rudder 
position. This layer also performs the conversion of telemetry data received 
via \morphSensors such as battery level or current location to a discretized 
events \lowBat and \arrivedN{4}. Other capabilities (e.g., camera control) may be 
accessed via the vehicle's \morphActuators.

 
 The \morphHybridControl layer also receives software modules from the 
 \morphControlPanel and is responsible for, having received a \reconfigure command 
 from the 
 \morphEnactor layer, binding them into the architecture so they can be used to 
 execute new  commands or produce new events. 



==> src/motivation.tex <==
\begin{figure*}
% \begin{subfigure} {0.18\linewidth}
% \centering
% \includegraphics[width=0.60\linewidth]{src/img/discretizacion}
% \caption{}
% \label{fig:regiondisc}
% \end{subfigure}
% ~
\begin{subfigure} {0.25\linewidth}
\centering
\input{src/lts/discretization}
\caption{}
\label{fig:discretization}
\end{subfigure}
~
\begin{subfigure} {0.16\linewidth}
\centering
\input{src/lts/capabilities}
\caption{}
\label{fig:capabilities}
\end{subfigure}
~
\begin{subfigure} {0.34\linewidth}
\centering
\input{src/lts/composition}
\caption{}
\label{fig:composition}
\end{subfigure}
\caption{(a) Grid-based discretization of. (b) Movement restrictions. 
(c) UAV capabilities. (d) Parallel composition (snippet).}
\label{fig:LTS}
\end{figure*}

\begin{comment}

\section{Motivating Use Case} \label{sec:motivation}

%\emph{\textbf{\missiondeg: }} Consider a UAV that is covering an area for 
%collecting data (e.g., mapping purposes). Unexpectedly, the battery consumption 
%rate is observed to be significantly higher than expected. The cause for the 
%increased 
%consumption rate might include unexpected high-winds, a faulty battery, or 
%malfunctioning 
%rudder servos. The detection of the unexpected battery consumption rate may be a 
%runtime 
%monitor that expects consumption to follow some model or a human observing a 
%control panel 
%on a ground control station. As a result, and after some manual diagnosis, a new 
%mission 
%may be specified. The mission might reduce the area to be covered based on what 
%has been 
%already covered, coverage priorities or the direction of the wind. The mission 
%specification would then be used to synthesise a new controller and uploaded onto 
%the UAV 
%where it would replace the current mission controller.

%\emph{\textbf{\rescue: }} 
Consider a UAV that is performing a patrol mission, flying at a high 
altitude between series of patrol points, recording the ground with a camera to 
relay a low-res movie through a low-bandwidth channel back to a control centre. While in 
mission, a report comes into the control centre that a person, known to be 
wearing a red jacket, has gone missing near the patrol area. A user then specifies a new 
mission for the UAV that involves systematically searching the area at low altitude using 
a red-sensor detection filter on high-res photos, landing on detection. The user 
prepares for upload the corresponding image processing module and specifies a number of 
key mission transition requirements: The module cannot be bound into the software while 
the camera is in use, the camera must be realigned to point downwards 
before the new mission is started. 

The architecture that we present allows for  the  system to automatically produce a 
controller that plays a strategy guaranteed to satisfy the user requirements. In this 
case, it involves first stopping the current mission, then realigning the camera, setting  
it  in high-res mode, setting the new altitude, binding the new software module, and 
then, only when the new altitude is reached, starting the new mission.
% in which at all 
% appropriate  locations are covered, taking  a picture and processing it at each location. 
Having computed the controller the system then uploads it, together with the new 
software module, and replaces  the currently executing controller with the new one. 
The new controller does the rest, effectively switching missions in-flight.

%
%\emph{\textbf{\goalchange: }} Consider a UAV typical patrol mission as 
%described in [22] for surveillance of two areas. To restrict the movement area of 
%the UAV the user imposes an area \region{\nfold} as a no-fly zone (i.e., avoidance 
%area), allowing other vehicles or humans to work in this region. Assume now that 
%the 
%goals for the UAV mission change dramatically, for instance, the currently flown 
%area 
%needs to be closed for maintenance. Instead of aborting the current mission and 
%re-synthesising a new one from scratch, the user specifies the two new areas to be 
%patrolled and aims to upload the new plan into the UAV to minimise the system's 
%downtime. 
%However, since the old flying area will be closed for maintenance, the user adds 
%another 
%no-fly zone \region{\nfnew}. However, updating the current plan with the new one 
%is not 
%a trivial task, as the regions \region{\nfold} and \region{\nfnew} are mutually 
%exclusive, meaning there is no safe place to change from the old plan into the new 
%one 
%without violating one of both specifications. 


\end{comment}

==> src/motivationnew.tex <==



\section{Assured Robot Adaptation \& Related Work} \label{sec:relwork}

We begin by identifying the requirements that must be met for an 
\textit{implementation of runtime assured mobile robot mission adaptation}:

\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
 \item \textbf{Runtime} adaptation requires updating the system's mission plan while 
 it is running~\cite{ModelRuntime}.
 \item \textbf{Assured} adaptation means that the technique used is founded on formal 
methods and as such provides guarantees of correctness. Correct dynamic software update 
has been studied extensively. However, it mostly  assumes that either there is no 
specification change and hence the same behaviour (minus bugs to be fixed) is expected 
(e.g.,~\cite{Hosek:2013:SSU:2486788.2486869}), or the specification is generic 
(e.g.,~\cite{DSURelaxedConsistencyModel,journals/tse/GuptaJB96,
Kramer:1990:EPP:93658.93672,Banno10}).
 \item The use of \textbf{mobile robots} involves having a mission specification language 
that allows to express the typical robotic applications. The work in~\cite{Menghi19} 
shows many robotic mission patterns that are common in the literature, expressed as LTL.
 \item To achieve \textbf{adaptation}, the update strategy must include a reconfiguration 
mechanism to allow introducing new capabilities into the robot or model new behaviours 
and interactions of the robot and its environment. \sz{Agregar citas}
 \item Another key concept in \textbf{adaptation} is the need for user-specified update 
properties as recognised by~\cite{Baresi:2010:DBD:1882362.1882367, 
Hayden:2012:SVC:2189314.2189336,Ghezzi2012,LaManna2013,Zhang:ICSE2006}. This means that 
an expert user may want to specify when or how adaptation from the old to the new mission 
can take place.
 \item \textbf{Implementation} of an assured adaptation system will require an 
architecture that allows to update plans and reconfiguration at runtime. \sz{Faltan citas 
y related work}
\end{enumerate}

The software engineering toolbox has many different techniques, ranging from 
requirements techniques to programming language constructs, that allow 
engineering systems that behave correctly under exceptional circumstances. To 
mention a few, goal modelling  allows assessing unstable requirements and eliciting  
 alternatives (e.g.,~\cite{vanLamsweerde01}), risk and safety analysis allows 
 detecting corner  cases that a design does not address properly 
 (e.g.~\cite{Lev95}), 
 exception  handling (e.g.,~\cite{LISP}) and fault tolerance 
 mechanisms~\cite{lamport1998the} to support catching, masking and degrading
 behaviour gracefully.
However, most of these techniques require devising upfront, before deployment, about what 
exceptional behaviour might occur and how it should be handled. 

We found no technique and implementation in the literature that would account for all the 
different requirements we described earlier. Despite this, we did find a number of 
elements that we propose to combine to achieve our goal adaptation system, namely: 
Dynamic Controller Update, hybrid controllers and MORPH reference architecture.

\textbf{Dynamic Controller Update} (DCU) promises \textit{runtime assured mission 
adaptation} (requirements $1$ and $2$) for systems that use high-level \textit{Discrete 
Event Controllers} for their mission plans, including system reconfiguration at an 
abstract level and user supplied transition requirements (requirement $4$ and $5$). 
However, the applicability of the DCU technique in real-life robot systems is yet to be 
studied. In Section~\ref{sec:dcu4robots} we will describe what modification must be made 
to the basics of the formulation of DCU to allow generating missions and update plans for 
\textit{mobile robots} (requirement 3) and how to model these robot problems in its 
formulation.

Recent research~\cite{Gazit08} has shown in mobile robot systems that the use of 
\textbf{Hybrid Controllers} provides a clear architecture and interface 
between discrete plans produced from controller synthesis and low-level feedback 
controllers, sensors and actuators from the robot. This approach is useful to implement 
previously synthesised \textit{Discrete Event Controllers}~\cite{Iterator}, 
but it includes no mechanisms to provide mission adaptation. We propose to extend hybrid 
controller architectures to include elements from the \textbf{MORPH reference 
architecture}~\cite{MORPH15}, which proposes a more complex structure in which 
structural and behavioural adaptation are managed in an independent but coordinated 
fashion (requirement 6). Moreover, no validation of this concept has been published. We 
will explain this extension to support adaptation in Section~\ref{sec:morphhybrid}.


==> src/preliminaries.tex <==
\section{Specification, Synthesis and Mission Updates}
\label{sec:Preliminaries}

Before discussing the architecture, we must introduce background on how UAV missions 
are specified and what it 
means for a discrete event controller to be synthesised from them. We do not focus on the 
formal aspects of specifications and synthesis algorithms. 
Instead we focus on how missions that are executed in a continuous variable 
space (e.g., geographical regions, sensor data, actuator inputs) are abstracted into 
discrete events 
and finite state spaces. Conveying the level of abstraction that is used is important to 
understand how the architecture is partitioned. A full formal treatment discretization 
of 
missions can be found in~\cite{Fainekos05}, for synthesis algorithms refer 
to~\cite{LTLMoP} for 
example. 
We specifically use the approach formalised in~\cite{Nahabedian-TSE}. 

We use the a simple scenario to exemplify main concepts.

\example{
Consider a typical UAV patrol mission as described in~\cite{Menghi19} for surveillance of 
two areas. To restrict the movement area of the UAV the user imposes an area 
\region{\nfold} as a no-fly zone allowing other vehicles or humans to work in this 
region.}

\subsection{Discrete Events}

A common strategy for reasoning about robot behaviour is to abstract the continuous 
physical world in which they operate~\cite{Castro15, Belta07, Paull13}. 
This involves discretizing the physical space where it moves and the robot sensor and 
actuator capabilities. 
%For an UAV moving in a continuous region, certain abstractions must be made to 
%obtain 
%a set of LTS that represent the system. 

\example{We discretize the continuous workspace of the UAV 
using a grid-based strategy  as in, for instance,~\cite{Livingston13, 
Wei18, 
Kundu19}. We number the cells in the discretization in a linear manner (see 
Figure~\ref{fig:regiondisc}). The UAV's capabilities can be abstracted using thresholds 
and 
control 
modes~\cite{Atlas}, and event pairs (e.g., \takeOff/\takeOffEnd) to 
mark 
the beginning and end of the control modes.

Controlled and monitored events may refer to discretization as in \goN{5} and 
\arrivedN{5} which model issuing the command to go to cell $5$ and the event of 
reaching it. We refer to this type of 
abstraction (e.g.,~\cite{Gazit09,Gazit08}) as Explicit-Location Planning because events 
refer explicitly to discrete locations.
}


\subsection{Labelled Transition Systems}

Labelled Transition Systems (LTS)~\cite{Keller76} support compositional
modelling of reactive systems. They describe observable system behaviour by 
means of transitions labelled with event names. We distinguish between controlled 
events (or actions/commands) and uncontrolled or monitored events. We 
use dashed transitions for controlled actions and continuous lines for uncontrolled 
events.

\example{In
Figure~\ref{fig:capabilities} we show LTS modelling the intended behaviour of a UAV 
moving 
in a discrete area. Initially (state $0$), the UAV may be commanded to \takeOff and 
as a result an event confirming successful termination of take-off will occur 
(\takeOffEnd). Once flying, a command to \go to a cell may be issued however 
new \go commands cannotwill be issued until an \arrived has been received. 
Figure~\ref{fig:discretization} describes movement within a discretized 
space restricting it only to adjacent cells as determined by 
Figure~\ref{fig:regiondisc}. Note that the LTS also models that the UAV is starting in 
cell $0$.

Note that an LTS (e.g.,~\ref{fig:capabilities}) can model constraints over controlled 
actions 
(e.g., \go  can only be issued while flying) and also \textit{assumptions} 
over monitored events (e.g.,  \arrived will be received after a \go 
command but not necessarily for the same cell as requested).}

The \textit{traces} of an LTS are all the sequences of events that can be 
formed by following transitions from the initial LTS state. 

%
%\begin{definition}(\emph{Labelled Transition System}) \label{def:LTS}
%A \emph{Labelled Transition System} (LTS)  $E$ is a tuple $(S_E,$ $A_E,$ $\Delta_E,$ 
%$e_0)$,  where 
%$S_E$ is a finite set of states, $A_E\subseteq \emph{Act}$ is its {\em communicating 
%alphabet}, 
%$\emph{Act}$ is the universe of all observable events, $\Delta_E \subseteq (S_E 
%\times A_E \times 
%S_E)$ is a transition relation, and $s_0 \in S_E$ 
%is the initial state.
%We say that $E$ is deterministic if $(e,\ell,e') \in \Delta_E$ and $(e,\ell,e'') \in 
%\Delta_E$, 
%then, $\! e'\!=\!e''\!$, and is deadlock-free if for all $e \in S$ there exists $(e,\ell,e') 
%\in 
%\Delta_E$. 
%\end{definition}

%\begin{notation}
%Let $E$ be an LTS, for a state $e \in S_E$ , we denote $\Delta_E(e)=\{\ell~|~(e,\ell,e') 
%\in 
%\Delta_E \}$.
%\end{notation}
%
%\begin{notation}
%Let $E$ be an LTS, for a state $e\in S_E$, we denote changing the initial state of $E$ 
%from $s_0$ 
%to $e$ as $E(e)$.
%\end{notation}

%\begin{notation}
%Let $E$ be an LTS, $\ell$ be a label in the alphabet of $E$, we denote by $e \xrightarrow[E]{\ell} 
%\dot{e}$ to the transition $(e,\ell,\dot{e})$ $\in$ $\Delta_E$.
%\end{notation}

%\begin{definition}(\emph{Trace}) \label{def:trace}
%A trace of an LTS $E$ is a sequence of labels $\pi=\ell_0, \ell_1,\dots$, for which 
%there exists a 
%sequence of states $s_0,s_1,\dots$ such that $s_0$ is the initial state of $E$ and 
%$\forall i \geq 
%0 \cdot \ell_{i} \in \Delta_E(s_i)$.
%We denote by $\pi \in E$ a trace on $E$ and by $\ell \in$ $\pi$ a label in a trace 
%$\pi$.
%\end{definition}

%We introduce the following equivalence relations between LTS.
%
%\begin{definition}(\emph{Isomorphism}) \label{def:isomorphism}
%Let $E$ $=$ $(S_E,$ $A,$ $\Delta_E,$ $s_E)$ and $M$ $=$ $(S_M,$ $A,$ 
%$\Delta_M,$ $s_M)$ be LTS.
%An isomophism is a bijection $f:S_E \rightarrow S_M$ that preserves transitions:
%
%\begin{center}
%$(q,\ell,q') \in \Delta_E$ \;\; if and only if \;\; $(f(q),\ell,f(q')) \in \Delta_M$\\
%\end{center}
%for all $q, q' \in S_E$. If there exists an isomorphism between 
%$E$ and $M$, then we say that $E$ and $M$ are isomorphic, denoted $E = M$.
%\end{definition}
%
%\begin{definition}(\emph{Bisimulation}) \label{def:bisimulation}
%Let $\mathcal{P}$ be the universe of all LTS. A binary relation $\mathcal{R} 
%\subseteq$ 
%$\mathcal{P}$ $\times$ $\mathcal{P}$ is a bisimulation if and only if whenever 
%$(P,Q) \in 
%\mathcal{R}$ then for each $a \in Act$ the following hold:
%
%\begin{itemize}[leftmargin=*]
%\item if $(P \xrightarrow{a} P')$, then, $(\exists Q' \cdot Q \xrightarrow{a} Q' 
%\wedge (P',Q') 
%\in \mathcal{R})$
%\item if $(Q \xrightarrow{a} Q')$, then, $(\exists P' \cdot P \xrightarrow{a} P' 
%\wedge (P',Q') 
%\in \mathcal{R})$
%\end{itemize}
%where $X \xrightarrow{x} X'$ denotes that the LTS $X$ can execute $x$ reaching a 
%state $x'$ and 
%$X' = X(x')$. We denote by $P \sim Q$ that $P$ and $Q$ are bisimilar.
%\end{definition}

Complex behaviour models can be built compositionally using \textit{parallel 
composition} %~\cite{magee06}. 
Given two LTS $A$ and $B$, their parallel composition 
($A\|B$) is an 
LTS that represents $A$ and $B$ executing asynchronously in parallel but 
synchronising on shared events. This means that, for instance, composition does not 
allow $A$ to progress along a 
transition labelled $\ell$ if $\ell$ is in the scope of $B$ and $B$ does not perform 
$\ell$ simultaneously. Composition can be thought of as the conjunction of the 
assumptions and constraints.

\example{Figure~\ref{fig:composition} shows part of the LTS resulting from the 
composition of 
Figures~\ref{fig:discretization} and \ref{fig:capabilities}.  In state $0$, 
\takeOff can occur because in it enables in
state $0$ of LTS \ref{fig:capabilities} and out of scope of 
LTS 
\ref{fig:discretization}. State $2$ of the composition represents when LTS 
\ref{fig:discretization} is 
in 
 $0$ and LTS \ref{fig:capabilities} 
is in $2$. Here, despite LTS \ref{fig:capabilities} enabling action $\goN{5}$ in 
state $2$, the 
composition does not 
allow such action because $\goN{5}$ is in the scope of \ref{fig:discretization} but not 
enabled in LTS \ref{fig:discretization}'s 
state $0$. 
}


%
%We formalise the parallel composition as follows.
%
%\begin{definition}(\emph{Parallel Composition}) \label{def:parallelComposition} 
%The parallel composition $E\|C$ of two LTS $E = (S_E, A_E, \Delta_E, e_0)$ and 
%$C = (S_C, A_C, \Delta_C, c_0)$ is an LTS $( S_E \times S_C, A_E \cup A_C, 
%\Delta_{\|},(e_0,c_0))$ such that $\Delta_{\|}$ is the smallest relation that 
%satisfies the rules below:
%
%\begin{center} \begin{tabular}{c}
%    $\!  \dfrac{(e,\ell,e') \in \Delta_E}
%            {((e,c),\ell,(e',c)) \in \Delta_{\|}} \, 
%            { \ell \, \notin \, A_C}$
%\\
%\\
%    $\!  \dfrac{(c,\ell,c')\in \Delta_C} 
%            {((e,c),\ell,(e,c'))\in \Delta_{\|}} \, 
%            {\ell \, \notin \, A_E}$
%    \\
%    \\
%
%    $\! \dfrac{(e,\ell,e') \in \Delta_E, \ (c,\ell,c') \in \Delta_C}  
%        {((e,c),\ell,(e',c'))\in \Delta_{\|}} \, 
%        {\ell \, \in \, A_E\cap A_C }$
%   
%\end{tabular} 
%\end{center}
%\end{definition}
%
%The relabelling operation defines an LTS by relabelling or removing transitions from 
%another LTS. 
%It does so by either removing a transition when its label is not defined in the 
%relabelling 
%function, or by changing the label according to the relabelling function.
%
%\begin{definition}\emph{(Relabelling operator)} \label{def:relabelling}
%Let $E = (S_E, A_E,$ $\Delta_E, e_0)$ be an LTS and $f:A_E \rightarrow \emph{Act}$ 
%be an injective partial function.
%The relabelling operation $[E]_f$ is an LTS $(S_E, A', \Delta_f, 
%e_0)$, where $\Delta_f$ is the smallest relation that satisfies the rule below:
%\begin{center} 
%	\begin{tabular}{lcl}
%	    $\!  \dfrac{(e,\ell,e') \; \in \; \Delta_E}
%	    {(e,f(\ell),e') \; \in \; \Delta_{f}} 
%	    \, {}$ %&
%%	    $\!  \frac{(e, \ell, e') \; \in \; \Delta_E} 
%%	    {(e,\ell,e') \; \not\in \; \Delta_{f}}
%%	    \, {\scriptstyle \ell \, \not\in \, Dom(f)}$
%	\end{tabular} 
%\end{center}
%\end{definition}

%\begin{property}\label{prop:relabel}
%Let $E, B$ be deterministic LTS, and $f: Act \rightarrow Act$ be a partial injective 
%function, 
%then, the 
%following equivalence holds: $[E\|B]_f \sim [E]_f \| [B]_f$ 
%\end{property}

%\begin{proof}[Proof of Property~\ref{prop:relabel}]
%We postulate the binary relation $=$ as a bisimulation. Then, for every state $(e,b)$ the following 
%holds.
%
%\vspace{1em}
%\noindent
%\begin{tabular}{rclc}
%$(e,b) \xrightarrow[{[}E\|B{]}_f]{f(\ell)} (e',b')$ & iff & $(e,b) \xrightarrow[E\|B]{\ell} 
%(e',b')$ 
%& iff \\
%$e \xrightarrow[E]{\ell} e'$ or $b \xrightarrow[B]{\ell} b'$ & iff &
%$e \xrightarrow[{[}E{]}_f]{f(\ell)} e'$ or $b \xrightarrow[{[}B{]}_f]{f(\ell)} b'$ & iff \\ 
%\multicolumn{4}{c}{$(e,b) \xrightarrow[{[}E{]}_f\|{[}B{]}_f]{f(\ell)} (e',b')$}
%\end{tabular}
%
%As $f$ is an injective function, it is not possible to generate a non-deterministic LTS from 
%relabelling.
%\end{proof}
%
%We introduce an interrupt handler operation that defines the sequential execution of 
%two LTS where 
%the switch from one LTS to the other is triggered by an event ($\alpha$).
%
%\begin{definition}\emph{(Interrupt handler)}  \label{def:lightning}
%Let $E$ $=$ $(S_E, A_E, \Delta_E, e_0)$ and $N$ $=$ $(S_N, A_N, \Delta_N, n_0)$ be 
%LTS, 
%$H$ be an interrupt handler relation such that $H \subseteq (S_E \times S_N)$, and
%$\alpha$ be an interrupt event such that $\alpha \not\in (A_E \cup A_N)$,.
%
%The interrupt handler $E \lig{H}{\alpha}N$ is an LTS 
%defined as $(S_E \cup S_N, A_E \cup A_N \cup \{\alpha\}, \Delta_{\lightning}, 
%e_0)$, where $\Delta_{\lightning}$ is the smallest relation that satisfies the 
%rules below:
%\\
%\begin{center} 
%	\begin{tabular}{lr}
%	    $\!  \dfrac{(e,\ell,e') \; \in \; \Delta_E}
%	    {(e,\ell,e') \; \in \; \Delta_{\lightning}}$
%	    &
%   	    $\! \dfrac{(n,\ell,n') \; \in \; \Delta_N}  
%        {(n,\ell,n') \; \in \; \Delta_{\lightning}}$ 
%\\
%\\		
%		\multicolumn{2}{c}{
%    	$\!  \dfrac{} 
%	    {(e,\alpha,n) \; \in \; \Delta_{\lightning}}
%	    \, {(e,n) \, \in \, H}$
%	    }
%	\end{tabular} 
%\end{center}
%\end{definition}

%\begin{property} \label{prop:lig}
%Let $A, B, C$ and $D$ be LTS,
%$H$ and $K$ be interrupt handlers relations defined for each state of $A$ and $K$ respectively,
%$\ell$ be an interrupt event,
%then, the following equivalence holds:
%\begin{equation*}
%P = ( (A \;\lig{H}{\alpha}\; B) \;\|\; (C \;\lig{K}{\alpha}\; D) ) \;\;\; \sim \;\;\; (A\|C) 
%\;\lig{R}{\alpha} \; (B\|D) = Q
%\end{equation*}
%where $R$ is an interrupt handler such that $((a,c),(b,d)) \in R$ iff $(a,b) \in H$ and $(c,d) 
%\in 
%K$. 
%\end{property}
%

%\begin{property} \label{prop:lig}
%Let $A, B, C$ and $D$ be LTS, 
%$H$ and $K$ be interrupt handlers relations and
%$\ell$ be an iterrupt event,
%then, the following equivalence holds:
%\begin{equation*}
%(A \;\lig{H}{\alpha}\; B) \;||\; (C \;\lig{K}{\alpha}\; D) \sim ( (A||C) \;\lig{H'}{\alpha}\; 
%B) 
%\;||\; (( A||C)\; \lig{K'}{\alpha}\; D)
%\end{equation*}
%where 
%$((a,c),b) \in H'$ iff $(a,b) \in H$, and,
%$((a,c),d) \in K'$ iff $(c,d) \in K$.
%\end{property}

%\begin{proof}[Proof of Property~\ref{prop:lig}]
%	We postulate the binary relation $\mathcal{R}$ such that for all $(a,c) \in A\|C$, $(a,c) 
%	\mathcal{R} (ab,cd)$ where $(ab,cd)$ are states before $\alpha$ in $P$. 
%	For all $(b,d) \in B\|D$, $\mathcal{R}$ is the relation $=$.
%	
%	\noindent
%	\begin{tabular}{rcll}
%		%\multicolumn{2}{c}{$(ab_0,cd_0) \sim$ $(a_0,c_0)$} & \multicolumn{2}{c}{$(ab_0,cd_0)$, 
%		%$(a_0,c_0)$ 
%		%initial states.}\\
%		$a \xrightarrow{\ell} a'$ or $c \xrightarrow{\ell} c'$ & iff & $(a,c) 
%		\xrightarrow{\ell} (a',c')$ & $\ell \neq \alpha$\\
%		& & $(a,c) \xrightarrow{\ell} (a',c')$ &\\
%		$a \xrightarrow{\alpha} H(a)$ and $c \xrightarrow{\alpha} K(c)$ & iff & 
%		\multicolumn{2}{l}{$(a,c)  \xrightarrow{\alpha} H'(a,c)$}\\
%		& & \multicolumn{2}{l}{$(a,c)  \xrightarrow{\alpha} K'(a,c)$}\\
%	\end{tabular}
%When transitioning through $\alpha$ both LTS reach bisimilar states because interrupt handler 
%relations $H'$ and $K'$ were defined to do so.
%\end{proof}


%\sz{\textbf{Empiezo a introducir LTS para misiones:}} \\



\subsection{Linear Temporal Logic}
\label{sec:fltl}

Linear Temporal Logic (LTL) is often used to describe behaviour 
requirements (e.g.,~\cite{vanLamsweerde01}). 
We use LTL of fluents as it provides a uniform framework for specifying state-based 
temporal properties in event-based models~\cite{gianna03}. 
%FLTL~\cite{gianna03} is a linear-time temporal logic for reasoning about fluents. 
A \emph{fluent} \formatFluent{fl} is defined by  a set of events that make it 
true ($Set_\top$), a set of events 
that make it false ($Set_\bot$) and an initial value ($v$) true ($\top$) or false 
($\bot$): $\formatFluent{fl} = \langle Set_\top, Set_\bot, v \rangle$. 

We may use an 
event label \event for the fluent defined as $\formatFluent{fl} = \langle
\set{\event}, \Lambda \setminus \set{\event}, \bot \rangle$, where $\Lambda$ denotes all 
the rest of the events. Thus, the fluent \event is only 
true just after the occurrence of the action \event.


\example{To define the fluents for  the  UAV mission requirements, we assume the 
patrol areas 
are cells 0 and 2 of Figure~\ref{fig:regiondisc}, and the no-fly region \region{\nfold} 
includes 
cells 3, 4 and 5, i.e., the bottom row. We define the following fluents (where $\Sigma = 
\set{\arrivedN{i} 
\cdot 0 \leq i \leq 
5})$: $\arrivedfl{0} = \langle \set{\arrivedN{0}} , \Sigma \backslash \set{\arrivedN{0}} 
, \top \rangle$, $\arrivedfl{2} = \langle \set{\arrivedN{2}} , \Sigma \backslash 
\set{\arrivedN{2}} , \bot \rangle$ and $\arrivedfl{\region{\nfold}} = \langle 
\set{\arrivedN{3},\arrivedN{4},\arrivedN{5}}, \Sigma \backslash 
\set{\arrivedN{3},\arrivedN{4},\arrivedN{5}} , \bot \rangle$.

Fluent \arrivedfl{0}, for instance, is initially true as the UAV starts at cell $0$ and 
becomes true 
every time event $\arrivedN{0}$ occurs, but becomes false every time any other 
\arrived event occurs. 
}

An FLTL formula is defined inductively using the standard Boolean connectives and 
temporal operators with their usual meaning: $\mathbf{X}$~(next), 
$\mathbf{U}$~(strong until)
, $\F$~(eventually) 
, $\Gl$~(always) 
, and $\mathbf{W}$~(weak until).
LTL satisfaction is defined with respect to a trace and can be extended 
to LTS if all the LTS traces satisfy the formula. 

\example{
The UAV mission goal can be written as:
%\begin{equation} \label{eqn:specpatrol}
$ \left(\Gl \F \arrivedfl{0} \wedge \Gl \F \arrivedfl{2} \right)$ $\wedge$ $\left( \Gl 
 \neg 
\arrivedfl{\region{\nfold}} \right)$.
%\end{equation}
 That is, be at cells $0$ and $2$ infinitely often and never be within the 
\region{\nfold} region.        
}



% of sets and a Boolean value: $\formatFluent{f} =$ 
%$\langle I, T, 
%Init\rangle$
%, where $\formatFluent{f}.I$ is the set of initiating actions, 
%$\formatFluent{f}.T$ is a set of terminating actions 
%and $\formatFluent{f}.I \cap \formatFluent{f}.T = \emptyset$.
%A fluent may be initially \emph{true} or \emph{false} as indicated by the 
%$\formatFluent{f}.Init$. 
%Note that, every action $\ell \in \emph{Act}$ induces a fluent, namely $\dot{\ell} =$ 
%$\langle$ 
%$\ell,$ $\emph{Act}$ $\backslash$ $\{\ell\},$ $\bot \rangle$.
%Finally, the alphabet of a fluent is the union of its terminating and initiating actions.

%Let $\mathcal{F}$ be the set of all possible fluents and $d$ be a fluent definition 
%function $d: 
%\mathcal{F} 
%\rightarrow \langle I,T,Init\rangle$.
%
%\begin{center}
%$\varphi ::= f \mid \neg \varphi \mid \varphi \vee \psi \mid \mathbf{X}\varphi \mid 
%\varphi 
%\mathbf{U} \psi$,
%\end{center}
%
%where $f \in \mathcal{F}$.
%We define $\varphi \wedge \psi$ as $\neg \varphi \vee \neg \psi$, 
%as $\top \mathbf{U} \varphi $, 
%as $\neg \F \neg \varphi$, and 
%as $\varphi \mathbf{U} \psi \vee \Gl \varphi$.
%
%Let $\Pi$ be the set of infinite traces over $\emph{Act}$.
%The trace $\pi=\ell_0,\ell_1,\ldots$ satisfies a fluent $f$ for a fluent
%definition $d$ at position $i$, denoted $\pi,i \modelsF{d} f$, if and only if, one of the 
%following
%conditions holds:
%
%\begin{itemize}[label = {\small$\blacktriangleright$}, leftmargin=*]
%\item $d(f).Init \wedge (\forall j \in \mathbb{N} \cdot 0 \leq j \leq i 
%\Rightarrow \ell_j \notin 
%d(f).T)$
%\item $\exists j \in \mathbb{N} \cdot (j \leq i \wedge \ell_j \in d(f).I)$ 
%$\wedge$
%
%\noindent	$\qquad\qquad\qquad\qquad(\forall k \in \mathbb{N} \cdot j < k \leq i 
%\Rightarrow \ell_k 
%\notin 
%	d(f).T)$
%\end{itemize}
%
%In other words, a fluent holds at position $i$ if and only if it
%holds initially or some initiating action has occurred, but no
%terminating action has since then occurred.
%
%Given an infinite trace $\pi$, the satisfaction of a formula $\varphi$
%at position $i$ for a fluent definition $d$, denoted $\pi,i\modelsF{d}\varphi$, is 
%defined as shown 
%in
%Figure~\ref{fig:satisfactionop}.  We say that $\varphi$ holds in
%$\pi$ for a fluent definition $d$, denoted $\pi\modelsF{d}\varphi$, if 
%$\pi,0\modelsF{d}\varphi$.
%
%To support combined reasoning over two specifications (the old and new) that may 
%have different 
%scopes (i.e. refer to different sets of events) we introduce a fluent definition 
%extension and a 
%related property.
%
%\begin{figure}[t]
%$$\begin{array}{lcl}
%%\pi,i \modelsF{d} f &\triangleq & \pi,i \modelsF{d} f  \\
%\pi,i \modelsF{d} \neg \varphi & \triangleq & \pi,i \not \modelsF{d} \varphi \\
%\pi,i \modelsF{d} \varphi \vee \psi &\triangleq& (\pi,i\modelsF{d} \varphi) \vee (\pi,i 
%\modelsF{d} 
%\psi) \\
%\pi,i \modelsF{d} \mathbf{X} \varphi &\triangleq & \pi,i+1 \modelsF{d} \varphi \\
%\pi,i \modelsF{d} \varphi \mathbf{U} \psi &\triangleq&\exists j \geq i \cdot \pi,j 
%\modelsF{d} \psi 
%\quad \wedge \\
%& & \qquad \quad \forall \mbox{ }i \leq k < j \cdot \pi,k \modelsF{d} \varphi\\
%\end{array}$$
%\caption{Semantics for the satisfaction operator.}
%\label{fig:satisfactionop}
%\end{figure}
%

%
%\begin{definition}\label{def:fluentDefinitionExtension} \emph{(Fluent definitions 
%extension)}
%Let $d$ and $d'$ be fluent definitions over $\Sigma$ and $\Sigma'$ respectively,  
%$d_e$ is a fluent definition extension of $d$ and $d'$, if and only if,
%the following conditions hold:
%
%
%\begin{itemize}[label = {\small$\blacktriangleright$}, leftmargin=*]
%\item $\forall$ $(f_e,$ $\langle I_e,T_e,Init_e \rangle)$ $\in d_e$, $\exists$ 
%$(f,\langle I,T,Init 
%\rangle)$ $\in d$
%such that $I_e =$ $I$ $\cup$ $\dot{I}$ and $T_e$ $=$ $T \cup \dot{T}$ 
%where $\dot{I}$ $\subseteq$ $(\Sigma'$ $\setminus$ $\Sigma)$ and  $\dot{T}$ 
%$\subseteq$ $(\Sigma'$ 
%$\setminus$ $\Sigma)$.
%\item $\forall$ $(f, \langle I,T,Init \rangle)$ $\in d$, $\exists$ $(f_e,\langle 
%I_e,T_e,Init_e 
%\rangle)$ $\in d_e$
%such that $I_e$ $=$ $I$  $\cup$ $\dot{I}$ and $T_e$ $=$ $T$ $\cup$ $\dot{T}$ 
%where $\dot{I}$ $\subseteq$ $(\Sigma'$ $\setminus$ $\Sigma)$ and $\dot{T}$ 
%$\subseteq$ $(\Sigma'$ 
%$\setminus$ $\Sigma)$.
%
%\item $\forall$ $(f_e,\langle I_e,T_e,Init_e \rangle)$ $\in d_e$, $\exists$ 
%$(f',\langle 
%I',T',Init' \rangle)$ $\in d'$
%such that $I_e =$ $I'$ $\cup$ $\dot{I}$ and $T_e$ $=$ $T' \cup \dot{T}$ 
%where $\dot{I}$ $\subseteq$ $(\Sigma$ $\setminus$ $\Sigma')$ and  $\dot{T}$ 
%$\subseteq$ $(\Sigma$ 
%$\setminus$ $\Sigma')$.
%\item $\forall$ $(f',\langle I',T',Init' \rangle)$ $\in d'$, $\exists$ $(f_e,\langle 
%I_e,T_e,Init_e \rangle)$ $\in d_e$
%such that $I_e$ $=$ $I'$  $\cup$ $\dot{I}$ and $T_e$ $=$ $T'$ $\cup$ $\dot{T}$ 
%where $\dot{I}$ $\subseteq$ $(\Sigma$ $\setminus$ $\Sigma')$ and $\dot{T}$ 
%$\subseteq$ $(\Sigma$ 
%$\setminus$ $\Sigma')$.
%
%\end{itemize}
%
%\end{definition}

\subsection{Discrete Event Controller Synthesis} \label{sec:ltscontrol}

A Discrete Event Controller Synthesis problem can be described as follows: Given an 
LTS $E$ that describes 
assumptions and requirements of the environment based on a partition of controllable 
and uncontrollable events, and given an LTL formula $\varphi$ representing the 
system goal, find a controller $C$ in the form of an LTS such that $C \| E$ satisfies 
$\varphi$ and never deadlocks, and in addition $C$ never restricts the occurrence of 
uncontrollable events in $E$ (c.f., \textit{legality}~\cite{alfaro01}). 

In other words, the problem is to find an LTS that can monitor uncontrolled events 
(never blocking their occurrence) and decide when to perform controlled events  such 
that for any trace in $E$, the controller with always 
achieve $\varphi$ and never deadlock. 

%
%\begin{definition}[LTS Control~{\rm \cite{dippolito13}}] \label{def:lts-control}
%Let $E = (S_E,$ $ A_E, \Delta_E, e_0)$ be an environment model in the form of an LTS,
%$A \subseteq  A_E$ be a set of controllable actions,
%$\unc{A} \subseteq  A_E$ be a set of uncontrollable actions,
%$G$ be a controller goal in the form of an FLTL property,
%and $d$ a fluent definition. 
%A solution for the LTS control problem with specification $\mathcal{E}$ $=$ $(E, G, 
%d, 
%A, 
%\unc{A})$ is an LTS $C$ $=$ $(S_C,A_E,\Delta_C,c_0)$ such that 
%$C$ is a legal LTS for $E$ with respect to $(A,\unc{A})$, $E\|C$ is deadlock free, and 
%$E\|C 
%\modelsF{d} G$.  
%\end{definition}




%The notion of legality (based on Interface 
%Automata~\cite{DBLP:conf/sigsoft/AlfaroH01}) 
%allows modelling controllability and monitorability of events. \sz{Propuesta: In the 
%LTS 
%in Figure~\ref{fig:composition}, controllable/uncontrollable actions are shown as 
%dotted/continuous lines. This LTS represents all the possible combinations of actions
%that can happen in the modelled system. We will refer to these type of LTS that result 
%from the parallel composition of all the modelled LTS as the \emph{environment}}. 
%A legal LTS cannot block the occurrence of events that it does not control and cannot 
%attempt 
%actions that it controls but its environment can not accept.
%
%\begin{definition} \label{def:Legal} \emph{(Legal LTS)}
%Let $P = (S_P, A_P$, $\Delta_P$,$p_0)$ and $Q = (S_Q,A_Q,\Delta_Q, q_0)$ be LTS,
%$C \subseteq (A_P \cup A_Q)$ be a set of events that $P$ does control and 
%$U \subseteq (A_P \cup A_Q)$ be a set of events that $P$ does not control.
%
%We say that $P$ is a legal LTS for $Q$ with respect to $(C,U)$ if 
%$\forall$ $(p,q) \in S_{P\|Q}$, $p$ and $q$ are legal in the following sense: 
%\begin{itemize}[leftmargin=*]
%\item $(\Delta_P(p) \cap U)$ $=$ $(\Delta_{Q}(q)\cap U)$, and
%\item $(\Delta_P(p) \cap C)$ $\subseteq$ $(\Delta_Q(q) \cap C)$. 
%\end{itemize}    
%\end{definition}
%
%Note that we adopt a slightly stronger notion than that 
%of~\cite{DBLP:conf/sigsoft/AlfaroH01}.
%Here, we request the $P$ not to be more robust (i.e. accept more uncontrollable 
%events) than $Q$ can exhibit.

\begin{figure}[b]
 \centering
 \input{src/lts/controller}
 \caption{LTS representation of a synthesised controller that satisfies $ \left(\Gl \F 
\arrivedfl{0} \wedge \Gl \F \arrivedfl{2} \right)$ $\wedge$ $\left( \Gl 
 \neg \arrivedfl{\region{\nfold}} \right)$.} 
\label{fig:controller}
\end{figure}

In general, synthesis of LTL is 2EXPTIME complete~\cite{pnueli89a}. Nevertheless, 
restriction on LTL have been studied and found to be solvable with lower 
complexity bounds. Notably, safety and \gr liveness 
properties can be solved in polynomial time~\cite{piterman06}. \gr properties are of the 
form $\bigwedge_{i=1}^n \Gl\F \assume_i$ $\implies$ $\bigwedge_{j=1}^m \Gl\F 
\guarantee_j$ where $\assume_i$ and $\guarantee_j$ are Boolean combinations of fluents 
that refer to assumptions and goals, respectively.

%An algorithm for solving LTS control problems for 
%safety and \gr properties is presented in~\cite{dippolito13}. 
%MTSA~\cite{MTSA,MTSAweb} implements it in addition to other 
%control problems (e.g.,~\cite{DBLP:journals/tosem/FischbeinDBCU12,dippolito11,
%DBLP:journals/tse/CiolekBDPU17}).


%It is defined as
%follows:
%
%\begin{definition}\label{def:sgr-lts-control}\emph{(\sgr LTS Control)}
%An LTS control problem $\mathcal{L}=\langle E, H, L_c\rangle$ is
%\sgr if $E$ is deterministic, and $H=\set{(\emptyset, I), (As, G)}$,
%where $I = \Gl \invariant$, $As=\bigwedge_{i=1}^n \Gl\F \assume_i$, $G
%= \bigwedge_{j=1}^m \Gl\F \guarantee_j$, and $\invariant$, $\assume_i$
%and $\guarantee_j$ are Boolean combinations of fluents.
%\end{definition}


\example{In Figure~\ref{fig:controller} we depict
the controller obtained by solving the 
control problem for an environment as in Figure~\ref{fig:composition}, the safety 
property  
$\Gl \neg \arrivedfl{\region{\nfold}}$ and the \gr property \linebreak
$\Gl \F \arrivedfl{0} \wedge \Gl \F \arrivedfl{2}$. Note that in state $14$, the 
controller may opt between landing or going to cell $1$. A more realistic model 
would consider battery levels and land accordingly. In this simple example, to 
avoid unnecessary 
landing we can add the following LTL property: $\Gl \neg \formatFluent{Land}$, 
where $\formatFluent{Land} = \langle \set{\land}, \set{\takeOff}, \bot \rangle$.
}
 


Consider a UAV system with an API that provides methods for all controllable events 
and produces all monitorable events of a controller $C$ that was synthesised for an 
environment $E$ and goal 
$\varphi$. Consider a module that \textit{enacts} $C$ by subscribing to the UAV 
events, monitoring them and calling API methods 
according to $C$. Enacting $C$ is guaranteed to achieve $\varphi$ as long as the 
UAV's observable 
behaviour is consistent with $E$.

%\begin{property}\label{prop:controller-bisimilar}
%Let $C$ be solution for the LTS control problem with specification $\mathcal{E}$ $=$ $(E, G, d, 
%A, \overline{A})$, then, $E\|C$ $\sim$ $C$.
%\end{property}

%\begin{proof}[Proof of Property~\ref{prop:controller-bisimilar}]
%The binary relation $\mathcal{R}$ such that for all $(e,c) \in E\|C$, $(e,c)\; \mathcal{R}\; c$ 
%is a bisimulation.
%
%Note that $C$ and $E$ share the same alphabet, and therefore, every transition of $E\|C$ is a 
%transition in $C$ because of the third rule of parallel composition. 
%In addition, as $C$ is a legal LTS for $E$, then, $C$ is a cut of $E$. (i.e. $C$ has less 
%behavior than $E$).
%Then, $(e,c) \xrightarrow[E\|C]{\ell} (e',c')$ iff 
%$c$ $\xrightarrow[C]{\ell} c'$ and $(e',c')\;$ $\mathcal{R}\;$ $c'$.


==> src/relatedwork.tex <==
\section{Discussion and Related Work}
\label{sec:discussion}


    The software engineering toolbox has many different techniques, ranging from 
 requirements techniques to programming language constructs, that allow 
 engineering systems that behave correctly under exceptional circumstances. To 
 mention a few, 
 goal modelling  allows assessing unstable requirements and eliciting  
 alternatives (e.g.,~\cite{vanLamsweerde01}), risk and safety analysis allows 
 detecting corner  cases that a design does not address properly 
 (e.g.~\cite{Lev95}), 
 exception  handling (e.g.,~\cite{LISP}) and fault tolerance 
 mechanisms~\cite{lamport1998the} to support catching, masking and degrading
 behaviour gracefully.
Most of these techniques require devising upfront, before deployment, about what 
exceptional behaviour might occur and how it should be handled. This paper 
proposes an architecture to provide better support when exceptional 
circumstances 
that were not considered before runtime occur. It takes a human-in-the-loop 
perspective and provides users with a high-level language and synthesis 
mechanisms to reduce the time it takes to change UAV missions at fly-time. 
  
This paper uses discrete event controller synthesis to ensure correct mission 
adaptation and as such builds on a large 
corpus of knowledge developed by the supervisory control~\cite{ramadge89}, 
reactive 
synthesis~\cite{pnueli89a} and automatic planning~\cite{Fikes:1971:SNA}
communities. We build in particular on advances in tractability developed by 
Piterman et. al~\cite{piterman06} for GR(1) temporal logic formulas. 

We build on the notion of model at runtime~\cite{ModelRuntime} both in the 
controllers being enacted, exception mechanisms, and the knowledge repository. 
We also build on the idea that involving humans in adaptation can add adaptability 
by having them act as  sophisticated  sensors and decision-makers or system-level 
effectors~\cite{Reasoning,Coupling,Guo18}. We believe the possibility of writing 
high-level mission goals and transition requirements, exploring model based 
solutions using tools like such as~\cite{MTSA,RATSY} and then deploying them as in 
this 
work, facilitates human-in-the-loop adaptation. 

Synthesis of discrete events controllers is increasingly being used by the robotics 
community to produce guaranteed-by-construction reactive plans that command 
robots~\cite{Gazit09,Atlas,Jing17,LTLMoP}. These approaches 
conceive synthesis mostly at development time. In~\cite{Guo18}  short-term 
reachability tasks can be added (and synthesised) at runtime, but the original goal 
remains fixed. 
%Central to our architecture is the possibility of runtime synthesis and 
%assured deployment even with massive specification changes. 
Synthesis has also been used 
%in the software engineering community, also
 at 
development time to produce glue code, 
adapters and mediators 
(e.g.,~\cite{Connectors,Issarny2011,Greenyer:2013:ISC:2491411.2491445,Pelliccione:2008:AAC:1454787.1454980}).
 It has also been been explored at runtime to  
support structural  reconfiguration of systems 
(e.g.,~\cite{Tajalli2010,arshad,seams08}).

Correct dynamic software update has been studied extensively. However, it 
mostly  assumes that either there is no specification change and hence the same behaviour 
(minus bugs to be fixed) is expected (e.g.,~\cite{Hosek:2013:SSU:2486788.2486869}), or 
the specification is generic 
(e.g.,~\cite{DSURelaxedConsistencyModel,journals/tse/GuptaJB96,Kramer:1990:EPP:93658.93672,Banno10}).
 The need for user-specified update properties has been recognised
 by many (e.g.,~\cite{Baresi:2010:DBD:1882362.1882367,
 Hayden:2012:SVC:2189314.2189336,Ghezzi2012,LaManna2013,Zhang:ICSE2006}).
 Some automated solutions to compute solutions 
 (e.g.,~\cite{Ghezzi2012,LaManna2013}) exists. Also, \cite{MAPEKTemplates} presents a 
 template based approach to reason about adaptations correctness.
Refer to~\cite{Nahabedian-TSE} 
for an explanation 
on how  controller update as defined herein builds upon and generalises  
 these works. 
  
  
  The notion of applying discrete event controller synthesis at runtime to support 
  adaptation was proposed in~\cite{MORPH15}. The MORPH reference architecture 
  proposes a more complex structure in which structural and behavioural adaptation 
  are managed in an independent but coordinated fashion. However, no validation of 
  this concept has been published. In a sense, the work presented here provides 
  experimental support to some of the ideas proposed in~\cite{MORPH15}.
 
 We believe experimental results provide some evidence that runtime synthesis can 
 be used to support mission adaptation in real UAV systems. Of course, there are 
 threats to validity. The main one being that experimental results may not generalise 
 to all UAV setups and vehicle configurations. Certainly, one limitation is that 
 synthesis is being applied to a single UAV. Many missions of interest in this domain 
 are multi-vehicle\cite{Cabreira19}. One potential limitation of the approach is that 
 discrete event controller synthesis may not scale to large missions. However, 
 techniques such as Iterator-Based  Planning~\cite{Iterator} have shown that 
 missions for hundreds of thousands of discrete locations are tractable. 
 
 
Complementary to discrete event controllers is the control of continuous variable 
dynamic systems, on which hybrid control systems rely for 
motion~\cite{Belta07,Gazit08}. This type of control is gaining increased attention in the 
adaptive systems~\cite{ControlAdaptive} 
community.
  
Our software architecture is inspired by MORPH~\cite{MORPH15}, the 3 layered 
architecture for robots~\cite{GAT} and 
self-managed systems~\cite{Kramer:2007:SSA:1253532.1254723}. and the MAPE-K 
architecture~\cite{MAPEK}. 
There has been significant work on architectures for robots and adaptive systems 
(e.g.,~\cite{Rainbow,Tajalli2010,HAFLOOP,MegaModels,DistArch,AMOUI20122720,MetaAdaptation,
MOSAICO}),
 see~\cite{DBLP:journals/jss/AhmadB16} 
for a systematic study. To the best of our 
knowledge this is the first one to implement assured adaptation at the mission level 
without constraining a priori what mission adaptations are allowed. 
% Noteworthy is~\cite{DistArch} where a fixed mission goal is achieved distributedly 
%and where local plans can be replanned. Also, in\cite{HAFLOOP} meta-adaptation 
%strategies are proposed and can be applied at runtime. n other 
%words, rather than focusing on adapting the managed system, it looks at adapting 
%the elements of the adaptation framework itself, i.e., the components involved in the 
%MAPE-K loop. 
%In~\cite{AMOUI20122720} a model-based architectural approach to 
%adaptation is presented, with much similitude to this work, however support for 
%automated synthesis of correct mission adaptation is not covered. 

%Herein, we  exploited to a limited extent what can be inferred and stored in 
%the knowledge repository about the systems current behaviour and structure. In 
%this 
%sense, the work is complementary to approaches to reflection \cite{reflection} and 
%self-awareness (e.g.,~\cite{SelfAwareness}).

%  However,  many of these techniques involve detecting exceptional circumstances 
%   at 
%   development time to build responses into the system so it can respond adequately 
%   at runtime. Research on self-adaptation focuses augmenting the spectrum of 
%   unexpected circumstances systems can handle, improving their behaviour in 
%   response to those events, and reducing the need and extent to which these 
%   situations can occur at development time. For 
%   example,~\cite{MetaAdaptation,MOSAICO} 
%   support runtime adaptation but based on a constrained set of pre-conceived
%    adaptations.
%  \\
  


%  
%  @INPROCEEDINGS{Doherty04adistributed,
%      author = {P. Doherty and P. Haslum and F. Heintz and T. Merz and P. Nyblom and T. 
%Persson and B. Wingman},
%      title = {A distributed architecture for autonomous unmanned aerial vehicle 
%experimentation},
%      booktitle = {In Proceedings of the 7th International Symposium on Distributed 
%Autonomous Robotic Systems},
%      year = {2004},
%      pages = {221--230}
%  }
%    
    
     %  [19] T. Baier, M. Huser, D. Westhoff, and J. Zhang, “A flexible software architecture 
     %  for multi-modal service robots,” in Multiconference on Computational 
     %Engineering 
     %  in Systems Applications, 2006.]
     
    
    
 
 

